Fair Energy Allocation in Risk-aware Energy Communities

This work introduces a decentralized mechanism for the fair and efficient allocation of limited renewable energy sources among consumers in an energy community. In the proposed non-cooperative game, the self-interested community members independently decide whether to compete or not for access to RESs during peak hours and shift their loads analogously. In the peak hours, a proportional allocation (PA) policy is used to allocate the limited RESs among the competitors. The existence of a Nash equilibrium (NE) or dominant strategies in this non-cooperative game is shown, and closed-form expressions of the renewable energy demand and social cost are derived. Moreover, a decentralized algorithm for choosing consumers' strategies that lie on NE states is designed. The work shows that the risk attitude of the consumers can have a significant impact on the deviation of the induced social cost from the optimal. Besides, the proposed decentralized mechanism with the PA policy is shown to attain a much lower social cost than one using the naive equal sharing policy.

==> old/Equal_sharing/uncoordinated_ES.tex <==


\subsection{Equal Sharing}\label{sec:eq_sharing_eq_extra_demand}
The analysis of the mixed strategy equilibrium probabilities for the ES policy coincides with the one for the PA policy (Section \ref{sec:prop_alloc_eq_extra_demand}) for all cases, except for Cases $2$ and $4$. For the sake of concision, this analysis is detailed below only for those cases.

\subsubsection*{\textbf{Case $2$}} 
\hspace{10pt}
\vspace{5pt}

\textbf{Sub-case $2(a)$:} A mixed strategy equilibrium exists if and only if, for any consumers' types  $\vartheta_i \in \Theta$ and $ \vartheta_j \in \Theta \setminus \{\vartheta_i\}$, with energy profiles $E_{\vartheta_i} \neq E_{\vartheta_j}$, it holds that
\small
\begin{align}\label{eq:relation_E_0_E_1_es_ne_extra_demand}
(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i} =(\gamma-\epsilon_{\vartheta_j}\beta)E_{\vartheta_j}.
\end{align}
\normalsize
This condition is derived by equalizing the right-hand sides of Eqs. \eqref{eq:eq_sharing_energy} and \eqref{eq:conditionEQ_extra_demand}, for $\vartheta_i \in \Theta$ and $\vartheta_j \in \Theta \setminus \{\vartheta_i\}$ and obtaining:
\begin{small}
\begin{align}
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1= \sum_{ {\vartheta_\ell}\in \Theta} r_{\vartheta_\ell} (N-1) p^{ES,NE}_{RES,\vartheta_\ell},\label{eq:probrelationes1}\\
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)E_{\vartheta_j}}-1= \sum_{ {\vartheta_\ell}\in \Theta} r_{\vartheta_\ell} (N-1) p^{ES,NE}_{RES,\vartheta_\ell}.\label{eq:probrelationes2}
\end{align} 
\end{small}
As the right hand-sides of Eqs. \eqref{eq:probrelationes1}-\eqref{eq:probrelationes2} are equal, it derives that:
\begin{align}
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1= 
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)E_{\vartheta_j}}-1,
\end{align} 
which straightforwardly leads to Eq. \eqref{eq:relation_E_0_E_1_es_ne_extra_demand}. 

 %\emph{The energy demand profiles satisfy  $E_{\vartheta_i } \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i }\beta)}$,  for all $\vartheta_i \in \Theta$.} %or $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gam
As a result, the competing probabilities, $p^{ES,NE}_{RES,{\vartheta_i }}$, for all $ \vartheta_i \in \Theta$ that lead to equilibrium states lie in the following range,
\footnotesize
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1-
  \sum_{{\vartheta_j}\in \Theta \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1\right]\frac{1}{r_{\vartheta_i}(N-1)}\right\}
    \Biggr].
    \label{eq:prop_alloc_eq_bounds_0_extra_demand}
\end{align}
\normalsize
Similarly to the PA policy, this range is derived using Eq. \eqref{eq:probrelationes1}.

\begin{remark}
Note that, similarly to the PA policy, from the condition of Eq. \eqref{eq:relation_E_0_E_1_es_ne_extra_demand}, the existence of NE is possible if and only if $\epsilon_0<\epsilon_1<\epsilon_2<..<\epsilon_{M-1}$. 
\end{remark}
\vspace{5pt}

%Then, we take extreme values of the other probabilities as before. 
%Note that the probabilities $p^{PA,NE}_{RES,\vartheta_i}$ should be chosen in the range \eqref{eq:prop_alloc_eq_bounds_0_extra_demand}, but, also under the constraint of \eqref{eq:probrelationes1}.


\textbf{Sub-case $2(b)$:} In this case, the analysis is identical to the one for the PA policy, in Section \ref{sec:prop_alloc_eq_extra_demand}. 
\vspace{5pt}
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%  p^{PA,NE}_{RES,1}
%  \in
%   \notag\\\Biggl[ max\left(0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{1}\beta)}-E_1-r(N-1)E_0\right]\frac{1}{(1-r)(N-1)E_1}\right),
%   \notag\\
%     min\left(1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{1}\beta)}-E_1\right]\frac{1}{(1-r)(N-1)E_1}\right)
%    \Biggr].
%    \label{eq:prop_alloc_eq_bounds_1_extra_demand}
%\end{align}
%\normalsize


%The rest content of Sub-case (a) remains the same with Section \ref{sec:prop_alloc_eq_extra_demand}. 
%The expected aggregated demand for any $\vartheta_i \in \Theta$ is equal to,
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%& D^{PA,NE}=\nonumber \\ & \min\{N  \sum_{\vartheta_j \in \Theta} r_{\vartheta_j }E_{\vartheta_j}, \max\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1\right]\frac{N}{(N-1)},0\}\}.
%    \label{eq:demand1}
%\end{align}
%\normalsize
%If $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$  for all $\vartheta_i \in \Theta$, it is dominant strategy for all consumers to defer from competing for $RES$, namely, $\upsilon_{RES, \vartheta_i}(p)>\upsilon_{nonRES, \vartheta_i}(p)$, $\forall p$ and $\forall i\in \mathcal{N}$. To show this, assume that $\vartheta_i=0$ and the allocated energy is $E'$. Then, in a large population regime $\upsilon_{RES, 0}(p)= E'  c_{RES}+(E_0-E') \gamma  c_{RES}$ and 
%$\upsilon_{nonRES, 0}(p)= \epsilon_0 E_0 \beta c_{RES}$. The inequality $\upsilon_{RES,0}(p)>\upsilon_{nonRES, 0}(p)$ is then equivalent to the inequality $E_0 >E' \frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ which is true by assumption and by the fact that the allocated energy $E'$ will be less than the available energy $\mathcal{ER}$. The same can be shown for the other $\vartheta_i\in \Theta$. Obviously, in this case, $D^{PA,NE}=0$.

\textbf{Sub-case $2(c)$:} %In this Sub-case Eq. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} is not true.
For consumers' types in the set $\Sigma_1$, the analysis is identical to the one for the PA policy, in Section \ref{sec:prop_alloc_eq_extra_demand}.

For consumers' types in the set $\Sigma_2$, the mixed strategy NE is determined under the condition of Eq. \eqref{eq:relation_E_0_E_1_es_ne_extra_demand} involving only those consumers' types in $\Sigma_2$. 

Therefore, the competing probabilities $p^{ES,NE}_{RES,\vartheta_i}$ for all $\vartheta_i\in \Sigma_2$ that lead to equilibrium states lie in the range:%the particular conditions on pricing and energy demand levels and provided by 
%
%
%if their energy demand $E_{\vartheta_j}$ equals the threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$, then the competing probability is 
\footnotesize
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{\vartheta_j\in \Sigma_2 \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_i}\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}\right]\frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_es_bounds_0_extra_demandnew}
\end{align}
\normalsize
By analogy with the analysis for the PA policy, this range is derived by writing Eq. \eqref{eq:probrelationes1} for consumers in $\Sigma_2$, which gives:
 $$\sum_{\vartheta_l\in \Sigma_2} p^{ES,NE}_{RES,\vartheta_l} r_{\vartheta_l }(N-1)=\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1$$.
 Then, \eqref{eq:prop_alloc_es_bounds_0_extra_demandnew} is derived by multiplying both sides of this equation with $E_{\vartheta_i}$ and taking the upper and lower bounds of the probabilities for all other consumers except $\theta_i \in \Sigma_2$.

\subsubsection*{\textbf{Case $4$}} 
For the consumers' types in the set $\Sigma_1$, the analysis is identical to the one for the PA policy, in Section \ref{sec:prop_alloc_eq_extra_demand}.

For the consumers' types in the set $\Sigma_2$, the mixed strategy NE is determined under condition \eqref{eq:relation_E_0_E_1_es_ne_extra_demand} involving only the those consumers' types in $\Sigma_2$. Besides, for consumers' types $\vartheta_i \in \Sigma_2$, the competing probabilities $p^{ES,NE}_{RES,\vartheta_i}$ that lead to equilibrium states lie in the range:
\small
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{\vartheta_j\in \Theta \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_i}\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}- \right. \right. \nonumber \\ & \left. \left.
  \sum_{\vartheta_j\in \Sigma_1\setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_i}\right]\frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_eq_bounds_0_extra_demandnew55}
\end{align}
\normalsize
This result is derived similarly to Eq. \eqref{eq:prop_alloc_es_bounds_0_extra_demandnew}, but considering that all consumers' types $\vartheta_i \in \Sigma_1$ compete for $RES$, i.e., that their competing probabilities that lead to equilibrium states are equal to $p^{ES,NE}_{RES,\vartheta_i}=1$.%, i.e., by equalizing the right-hand sides of Eqs. (\ref{eq:eq_sharing_energy}) and (\ref{eq:conditionEQ_extra_demand}) and considering that consumers with energy profile in $\Sigma_1$ compete for $RES$, i.e., $p^{ES,NE}_{RES,\vartheta_i}=1,~ \forall \vartheta_i \in \Sigma_1 $.% Then, we obtain the equality $\sum_{\vartheta_j\in \Sigma_2} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }(N-1)+\sum_{\vartheta_j\in \Sigma_1} r_{\vartheta_j }(N-1)=\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1$, and  Eq. \eqref{eq:prop_alloc_eq_bounds_0_extra_demandnew55} derives if multiplying both sides with $E_{\vartheta_i}$ and taking extreme values of the probabilities. %Note that based on Eq. \eqref{eq:equal_sharing_eq_j_extra_demand2}, if $E_{\vartheta_j}$ is strictly lower than $thr_d=\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}rse^{PA}_{\vartheta_j}(.)$ then the dominant strategy is to compete for $RES$, else if $E_{\vartheta_j}> th_d$ the dominant strategy is to defer from competing for $RES$.




%with $E_0 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$. Otherwise, if $E_0 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$, it is dominant strategy for all consumers to defer from competing for $RES$, namely $c_{i}^{(\cdot)}(RES,p)>c_{i}^{(\cdot)}(nonRES,p)$, $\forall p$ and $\forall i\in \mathcal{N}$. Similarly, if $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$ and $E_{\vartheta_j} \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}$, with $\vartheta_i\neq \vartheta_j$ and $i,j \in \mathcal{N}$, it is dominant strategy for all consumers of $\vartheta_i$ energy profile not to compete for $RES$. Regarding consumers of $\vartheta_j$ energy profile, they end up competing with probability $p^{ES,NE}_{RES,\vartheta_j}$ that follows (\ref{eq:prop_alloc_eq_j_extra_demand1}). %, if their energy demand $E_{\vartheta_j}$ equals the threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$; otherwise, competing for $RES$ dominates reneging from RES, if $E_{\vartheta_j}$ is lower than this threshold value, and it is dominated by reneging from RES, if $E_{\vartheta_j}$ exceeds this threshold value.
%Furthermore, if $\epsilon_{\vartheta_i} \geq \gamma/\beta$, $\forall i\in \mathcal{N}$, it is dominant strategy for all consumer to compete for $RES$, since it holds that $c_{i}^{(\cdot)}(RES,p) < c_{i}^{(\cdot)}(nonRES,p)$, $\forall p$ and $\forall i\in \mathcal{N}$. Finally, if $\epsilon_{\vartheta_i} \geq \gamma/\beta$ and $\epsilon_{\vartheta_j} < \gamma/\beta$, with $\vartheta_i\neq \vartheta_j$ and $i,j \in \mathcal{N}$, then it is dominant strategy for all consumers of $\vartheta_i$ energy profile to compete, while all consumers of $\vartheta_j$ end up competing with $p^{PA,NE}_{RES,\vartheta_j}, ~0\leq p^{PA,NE}_{RES,\vartheta_j} \leq 1$,
%
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%p^{PA,NE}_{RES,\vartheta_j}  = 
%   \left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}-[r+(1-2r)\vartheta_i](N-1)E_{\vartheta_j}\right] \notag \\
%    \times  \frac{1}{[r+(1-2r)\vartheta_j](N-1)E_{\vartheta_j}} 
% \label{eq:es_eq_j_extra_demand2}
%\end{align}
%\normalsize


%if $E_{\vartheta_j}$ equals threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$. Otherwise, under lower energy demand $E_{\vartheta_j}$, the dominant strategy amounts to competing and under higher energy demand, they are motivated to resort to the safer option avoiding competition.

%It can be easily observed that the equal sharing and the proportional allocation policies may only cause different equilibrium states under the game variant where consumers risk only part of their maximum possible demand,i.e., with risk-conservative consumers. For instance the conditions of Eqs. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}, \eqref{eq:relation_E_0_E_1_es_ne_extra_demand} coincide for risk-seeking consumers. %In particular, the equal sharing differentiates from proportional allocation under two cases: (a) if $\epsilon_{\vartheta_i}<\gamma/\beta$, $\forall i\in \mathcal{N}$, $E_0 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$; (b) if $\epsilon_{\vartheta_i} \geq \gamma/\beta$, $\epsilon_{\vartheta_j} < \gamma/\beta$ and $E_{\vartheta_j}=\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$ with $\vartheta_i\neq \vartheta_j$ and $i,j \in \mathcal{N}$. Thus, 
%The set of mixed strategy equilibrium probabilities under equal sharing is also presented in Table \ref{table_eq_comp_pro}, by (i) replacing the probabilities in the second line, fifth and sixth columns, with the expressions in (\ref{eq:equal_sharing_eq_bounds_0_extra_demand}), (\ref{eq:equal_sharing_eq_bounds_1_extra_demand}), replacing the probability in the seventh line, sixth column with Eq. (\ref{eq:equal_sharing_eq_j_extra_demand2}), and (iii) replacing the thresholds $thr_e$, $thr_f$ with $\frac{thr_c}{( r+(1-2r)\vartheta_i)(N-1)+(r+(1-2r)\vartheta_j)(N-1)+1}$ and $thr_d$, correspondingly.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



In all cases where the PA and ES policies result in the same mixed strategy equilibrium probabilities, the corresponding expected aggregate demand for RES is the same under the two policies. 
Otherwise (i.e., for cases 2 and 4 described above), we can write the expected aggregate demand under the ES policy as follows:

\footnotesize
\begin{align}
& \hspace{-10pt}  D^{ES,NE}(\mathbf{p^{ES,NE}}) =N p^{ES,NE}_{RES,0} r_{0}E_{0}+N \sum_{\vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }E_{\vartheta_j} \nonumber \\
&=\Bigl (\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{0}\beta)E_{0}}-1- \sum_{\vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j } (N-1) \Bigr) \frac{N~E_0}{N-1} \nonumber \\ &+N \sum_{\vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }E_{\vartheta_j} \nonumber \\ &=D^{PA,NE}+N \sum_{ \vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }(E_{\vartheta_j} -E_0).
\label{eq:demand_es_ne_extra_demand}
\end{align}
\normalsize

%given in Table \ref{table_eq_comp_pro}. 
%Otherwise, %under the conditions of the second and seventh line of Table \ref{table_eq_comp_pro}, 
%the expected aggregate demand for renewable energy $D^{ES,NE}(p^{ES,NE})$ is an non-decreasing function of $p^{ES,NE}_{RES,1}$, that is,
%
%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%\hspace{-10pt}  && \hspace{-10pt}  D^{ES,NE}(p^{ES,NE}) =N \sum_{\vartheta_j\in \Theta} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }E_{\vartheta_j}.
%\label{eq:demand_es_ne_extra_demand}
%\end{eqnarray}
%\normalsize
% \hspace{-10pt} &=& \hspace{-10pt}  \frac{N}{(N-1)} \left[ \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{0}\beta)} -E_0\right] + (1-r)(E_1-E_0)N p^{ES,NE}_{RES,1}\nonumber\\
% \hspace{-10pt} &=& \hspace{-10pt} D^{PA,NE}(p^{PA,NE})+ (1-r)(E_1-E_0)N p^{ES,NE}_{RES,1}.



%The second line in Eq. \eqref{eq:demand_es_ne_extra_demand} derives by replacing in the first line that  $ p^{ES,NE}_{RES,0} =\frac{1}{r(N-1) } \Big[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)E_0}-1- (1-r) (N-1) p^{ES,NE}_{RES,1} \Big]$.
%Likewise, under the conditions of the sixth line of Table \ref{table_eq_comp_pro}, the expected total number of consumers that compete for $RES$ in equilibrium, equals $\frac{N}{(N-1)}  \left[ \frac{\mathcal{ER}}{E_{\vartheta_j}}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-1 \right]$ and the expected aggregate demand for renewable energy $D^{ES,NE}(p^{ES,NE})$ is given by (\ref{eq:demand_es_ne_extra_demand}).

%Conditions under which equilibrium competing probabilities generate inefficiencies, that is, a number of consumers incur the price of the lack of coordination are described in Section \ref{sec:coordinated}.


%\textbf{Social Cost:}  The expected aggregate cost incurred by the entire population is a function of $p^{ES,NE}$ (contrary to the Eq. \eqref{eq:social_cost_pa}) and is given by,
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%& C^{ES,NE}(p^{ES,NE})  \nonumber \\ &=  d(p^{ES,NE}) c_{RES} +(D^{ES,NE}-d(p^{ES,NE}))c_{nonRES,D} \nonumber \\
%&   + N\left[\sum_{\vartheta_j \in \Theta} r_{\vartheta_j }p^{ES,NE}_{nonRES,\vartheta_j}\epsilon_{\vartheta_j }E_{\vartheta_j}\right] c_{nonRES,N},
% \label{eq:social_cost_es_extra_demand}
% \end{align}
%\normalsize 


Finally, similarly to the proportionally-fair allocation, the expected aggregate social cost at NE takes an interesting form in the special case of risk-seeking consumers. Specifically, 
\footnotesize
\begin{align}
&C^{ES,NE}(\mathbf{p^{ES,NE}}) \nonumber\\ &=  d(\mathbf{p^{ES,NE}}) c_{RES} +(D^{ES,NE}(\mathbf{p^{ES,NE}}) -d(\mathbf{p^{ES,NE}}))c_{nonRES,D}\nonumber \\
&+ \hspace{-5pt} \left[ \left[  \sum_{ \vartheta_j=0}^{M-1} r_{\vartheta_j} N E_{\vartheta_j}\right]-D^{ES,NE}(\mathbf{p^{ES,NE}}) \right] c_{nonRES,N}.
 \label{eq:social_cost_es_sc}
 \end{align}
\normalsize
%with \footnotesize$d(p^{ES,NE})=min(sh(p^{ES,NE}), E_0)rNp_{RES,0}^{ES,NE}+min(sh(p^{ES,NE}), E_1)(1-r)Np_{RES,1}^{ES,NE}$ \normalsize the actual aggregate amount of RES  allocated to the consumers and \footnotesize$sh(p^{ES,NE}) =\frac{\mathcal{ER}}{rNp_{RES,0}^{ES,NE}+(1-r)Np_{RES,1}^{ES,NE}}$ \normalsize the fair share of RES disseminated to the consumers. 


%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%sh(p) \hspace{-5pt} &=& \hspace{-5pt} \frac{\mathcal{ER}}{rNp_{RES,0}+(1-r)Np_{RES,1}}
% \label{eq:sharing_es}
% \end{eqnarray}
%\normalsize





%\subsection{Social Cost}\label{sec:social_cost_extra_demand}
%
%In the game variant with risk-conservative consumers, the social cost becomes
%
%
%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%C(p) \hspace{-5pt} &=& \hspace{-5pt} min(\mathcal{ER}, D^{(\cdot)}(p)) c_{RES} +  max(0,D^{(\cdot)}(p)-\mathcal{ER})c_{nonRES,D} \nonumber \\
% \hspace{-42pt}  &&  \hspace{-42pt} + \left[ rNp_{nonRES,0}(\epsilon_{0}E_0) \hspace{-2pt} + \hspace{-2pt} (1-r)Np_{nonRES,1}(\epsilon_{1}E_1)\right] c_{nonRES,N}
% \label{eq:social_cost_pa_es_extra_demand}
% \end{eqnarray}
%\normalsize


%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%C(p) \hspace{-5pt} &=& \hspace{-5pt} min(\mathcal{ER}, D^{(\cdot)}(p)) c_{RES} +  max(0,D^{(\cdot)}(p)-\mathcal{ER})c_{nonRES,D} \nonumber \\
% \hspace{-5pt}   &+& \hspace{-5pt} \left[ rN\epsilon_{0}E_0 + (1-r)N\epsilon_{1}E_1-D^{(\cdot)}(p)\right] c_{nonRES,N}
% \label{eq:social_cost_pa_es_extra_demand}
% \end{eqnarray}
%\normalsize




==> old/coordinated.tex <==
\section{Centralized Coordinated energy source allocation}\label{sec:coordinated}

In this section, we study a centralized mechanism that coordinates how consumers' demand will be served (i.e., by which source) in order to minimize the social cost (i.e., Eqs. \eqref{eq:social_cost_pa_extra_demand} for proportional allocation and Eqs. \eqref{eq:social_cost_es} for equal sharing). Furthermore, we evaluate the side-effects that stem from the distributed, uncoordinated energy source selection as far as the social welfare is concerned via the Price of Anarchy (PoA) measure \cite{Koutsoupias09}. PoA is expressed as the ratio of the social cost in the worst-case equilibria over the optimal-minimum social cost of the centralized mechanism.
We study the PA mechanism analytically in most of the distinguished cases. For the ES mechanism, the centralized decisions for minimizing the social cost are harder to derive analytically and we will present numerical evaluations in Section \ref{sec:eval} using a software optimization tool such as Mathematica or MATLAB. The same is true for the PoA, which can be obtained as indicated in Section \ref{sec:poa}. %may be alleviated with control mechanisms that coordinate individual decisions towards more socially
%efficient choices. In the sequel, we describe two approaches that differ on the required infrastructure and the amount of control they impose upon the energy source allocation. Furthermore, the (in)efficiency of the equilibria action profiles as derived in Section \ref{sec:uncoordinated_extra_demand}, %Sections \ref{sec:uncoordinated_no_extra_demand} and \ref{sec:uncoordinated_extra_demand}, 
%resulting from the strategically selfish individual
%decisions, is assessed through the broadly used metric of the Price of Anarchy (\textit{PoA}) \cite{Koutsoupias09}. This metric
%expresses the ratio of the social cost in the worst-case equilibria over the optimal-minimum social cost as derived under the two coordination approaches.
%
%%\subsection{Centralized Coordination Mechanisms}\label{sec:opt_central_no_extra_demand}
%
%The side-effects in energy pursuit may be eliminated by introducing centralized mechanisms
%that undertake both the information processing and the decision-making tasks. These mechanisms coordinate the service of consumers' demand to ensure the optimal utilization of RES.%, on the one side, and the elimination of the congestion penalty, on the other side (Ref. Section \ref{sec:game}).

\subsubsection{Proportional Allocation}\label{sec:opt_pa_central_no_extra_demand}
 Let $p^{PA,OPT}_{RES,\theta_i} (p^{PA,OPT}_{nonRES,\theta_i})$ stand for the probability that users of energy profile $\theta_i \in \Theta$ opt (do not opt) for RES, as decided by the centralized coordinated mechanism, under the proportional allocation. $\mathbf{p^{PA,OPT}}$ is defined similarly to $\mathbf{p^{PA,NE}}$. The following cases are distinguished.

It is important to note that the centralized coordination mechanism will achieve a demand for RES equal to $D^{PA,OPT}=min(\sum_{\theta_j \in \Theta}r_{\theta_j}NE_{\theta_j},\mathcal{ER})$, in all considered cases. 

\textbf{Case $1$.} The RES capacity exceeds the aggregated consumer demand. Then, all consumers (for both cases of risk-seeking and risk-conservative) are directed to the RES and $p^{PA,OPT}_{RES,\theta_i}=1$, $\forall \theta_i \in \Theta$.

In all the rest cases, the aggregated consumer demand exceeds the RES capacity. 

\textbf{Case $2$.} The risk-aversion degrees satisfy $\epsilon_{\vartheta_i}=\epsilon'<\gamma/\beta$, $\forall i\in \mathcal{N}$. This case includes the risk-seeking consumers ($\gamma/\beta>1$). Then, $p^{PA,OPT}_{RES,\theta_i}$, for all  $\theta_i \in \Theta$ are chosen to match the RES demand to supply, that is, %$rNp^{PA,OPT}_{nonRES,0}E_0+(1-r)N p^{PA,OPT}_{nonRES,1}E_1=\mathcal{ER} $.

\vspace{-5pt}
\small
\begin{equation}
N \sum_{\theta_j \in \Theta}r_{\theta_j} E_{\theta_j}p^{PA,OPT}_{RES,\theta_j}=\mathcal{ER}.
\label{eq:optimal}
\end{equation}
\normalsize

The competing probabilities, $p^{PA,OPT}_{RES,\theta_i} $, lie in the range below, under the constraint of \eqref{eq:optimal},

\vspace{-5pt}
\footnotesize
\begin{align}
 \hspace{-5pt} 
 \Biggl[max\left\{0,\frac{\left[\mathcal{ER} -\sum_{\theta_j\neq \theta_i, \theta_j \in \Theta}r_{\theta_j}N E_{\theta_j}\right]}{r_{\theta_i}N E_{\theta_i}}\right\},
   %\notag\\
    % min\left(1,\mathcal{ER} \frac{1}{rNE_0}\right)
    min\left\{1,\frac{\mathcal{ER}}{r_{\theta_i}N E_{\theta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_opt_bounds_0}
\end{align}
\normalsize


The cost due to the demand at night-rate is constant and equal to 
$\epsilon' N \sum_{\theta_j \in \Theta}r_{\theta_j}E_{\theta_j}p^{PA,OPT}_{nonRES,\theta_j} c_{noRES,N}=\epsilon'  ( N\sum_{\theta_j \in \Theta}r_{\theta_j}E_{\theta_j}- \mathcal{ER}) c_{noRES,N}$.

\textbf{Case $3$.} The different energy profiles are coupled with different degrees of risk-aversion, %, which is less than $\gamma/\beta$, %depart in their policy in adjusting their demand level to the estimated risk of an action, 
\ie $\exists$  $i,j\in \mathcal{N}: \gamma/\beta>\epsilon_{\vartheta_i} > \epsilon_{\vartheta_j}$. In this case, the night-rate social cost to be minimized is $Nc_{noRES,N} \sum_{\theta_j \in \Theta}\epsilon_{\theta_j}r_{\theta_j}E_{\theta_j}p^{PA,OPT}_{nonRES,\theta_j} $. The solution can be derived by a software optimization tool such as Mathematica or MATLAB. In addition, due to the fact that the RES demand should match its supply as in Case $2$,  the probabilities, $p^{PA,OPT}_{RES,\theta_i} $, lie in the ranges given in (\ref{eq:prop_alloc_opt_bounds_0}). 


%Therefore, it is minimized when consumers with energy profiles $\theta_j \in \Theta$, corresponding to higher values of $\epsilon_{\theta_j}r_{\theta_j}E_{\theta_j}$ are assigned lower values of $p^{PA,OPT}_{nonRES,\theta_j} $ and thus higher values of $p^{PA,OPT}_{RES,\theta_j} $ (i.e., they are prioritized for RES). In addition, due to the fact that the RES demand should match its supply as in Case $2$,  the probabilities lie in the ranges given in (\ref{eq:prop_alloc_opt_bounds_0}). 

To illustrate this result in a simple scenario, let us assume the case of two energy profiles and let us examine the expected cost at night-rate; $(\epsilon_0 r_0 N p^{PA,OPT}_{nonRES,0}E_0+\epsilon_1 r_1 N p^{PA,OPT}_{nonRES,1} E_1) c_{nonRES,N}$. Let us assume that $\epsilon_0> \epsilon_1$, then we can write $\epsilon_0= \epsilon_0'+\epsilon_1$, with $\epsilon_0'>0$. Thus, the expected cost at night-rate becomes $(\epsilon_0' r_0N p^{PA,OPT}_{nonRES,0}E_0+\epsilon_1 (r_0 N E_0+r_1 N E_1- \mathcal{ER}) ) c_{nonRES,N}$. The only controllable term is $\epsilon_0' r_0 N p^{PA,OPT}_{nonRES,0}E_0$ that is minimized when $ p^{PA,OPT}_{nonRES,0}$ is minimized, i.e., when its complementary $ p^{PA,OPT}_{RES,0}$ is maximized. Note that the expected cost due to use of RES will be always equal to $c_{RES} \mathcal{ER}$.

\textbf{Case $4$.} The risk-aversion degrees satisfy $\epsilon_{\vartheta_i} \geq \gamma/\beta$, $\forall i\in \mathcal{N}$. Then, the optimal centralized coordination mechanism would direct all consumers to RES, \ie $p^{PA,OPT}_{RES,\theta_i}=1$. This derives similarly to Case $3$ of Section \ref{sec:prop_alloc_eq_extra_demand}.
 
\textbf{Case $5$.} In this case, there exist two distinct sets of consumers' profiles $\Sigma_1$, $\Sigma_2$ with $\Sigma_1 \cap \Sigma_2= \emptyset$ and it holds that $\Biggl\{\epsilon_{\vartheta_i} \geq \gamma/\beta,~ \forall \vartheta_i \in \Sigma_1\Biggr\}$, and $\Biggl\{\epsilon_{\vartheta_i} < \gamma/\beta, ~ \forall \vartheta_i \in \Sigma_2\Biggr\}$. Then, it is dominant strategy for all consumers with energy profiles in the set $\Sigma_1$ to compete for RES, while the probability that consumers with energy profiles in the set $\Sigma_2$ compete for RES is shaped to totally utilize the remaining RES, i.e.,
%$[r+(1-2r)\vartheta_i]NE_{\vartheta_i}+[r+(1-2r)\vartheta_j]NE_{\vartheta_j}p^{PA,OPT}_{RES,\vartheta_j}=\mathcal{ER}$.

\vspace{-5pt}
\footnotesize
\begin{align}
&p^{PA,OPT}_{RES,\vartheta_i}=1, \forall \vartheta_i \in \Sigma_1; \notag \\
&p^{PA,OPT}_{RES,\vartheta_i}\in \nonumber \\
&\Biggl[\max\left\{0,\frac{\mathcal{ER}-\sum_{\theta_i \neq \theta_j, \theta_j \in \Theta}r_{\theta_j}N E_{\theta_j}}{r_{\theta_i}N E_{\theta_i}}\right\}, \nonumber \\ & \min\left\{1,\frac{\mathcal{ER}-\sum_{ \theta_j \in \Sigma_1}r_{\theta_j}N E_{\theta_j}}{r_{\theta_i}N E_{\theta_i}}\right\}  \Biggr],~ \forall \vartheta_i \in \Sigma_2.
\label{eq:prop_alloc_opt_p_cond}
\end{align}
\normalsize

Note that the probabilities of $\Sigma_2$ should be chosen under Eq. \eqref{eq:optimal}. However, the probability assignment to the energy profiles in the set $\Sigma_2$ for minimizing the social cost (i.e., equivalently the night rate cost because the demand in the day will be equal to $\mathcal{ER}$) should be done with the help of a software optimization tool. An exception is the case where $|\Sigma_2|=1$. In this special case, for $\vartheta_i \in \Sigma_2$, $p^{PA,OPT}_{RES,\vartheta_i}=\max\left\{0, \min\left\{1,\frac{\mathcal{ER}-\sum_{ \theta_j \in \Sigma_1}r_{\theta_j}N E_{\theta_j}}{r_{\theta_i}N E_{\theta_i}}\right\}\right\}$.


\textbf{Social Cost:} It is given as follows.

\begin{small}
\begin{align}
&C^{PA,OPT}(\mathbf{p^{PA,OPT}})= D^{PA,OPT} c_{RES}  \nonumber \\ 
&+Nc_{noRES,N} \sum_{\theta_j \in \Theta}\epsilon_{\theta_j}r_{\theta_j}E_{\theta_j}p^{PA,OPT}_{nonRES,\theta_j}.
 \label{eq:social_cost_pa_op1t}
 \end{align}
\end{small}


In the special case of risk-seeking consumers the social cost has a constant value with respect to the decision probabilities:
\begin{small}
\begin{align}
&C^{PA,OPT}= D^{PA,OPT} c_{RES}  \nonumber \\ 
&+ c_{noRES,N} \Biggl[ N\sum_{\theta_j \in \Theta} r_{\theta_j}E_{\theta_j}- D^{PA,OPT} \Biggr].
 \label{eq:social_cost_pa_opt2}
 \end{align}
\end{small}


\subsubsection{Price of Anarchy:} \label{sec:poa}
The (in)efficiency of equilibrium strategies is quantified by the Price of Anarchy (PoA). In order to compute the PoA for each particular case (where cases are distinguished with respect to the risk-aversion degree values and energy consumption values), we should compute the mixed strategy equilibrium that leads to the worst social cost for this case. PoA is computed as follows: %with respect to the consumers behavior (e.g., risk-seeking and risk-conservative), risk-aversion degree values and energy consumption values $E_0$, $E_1$.

\vspace{-5pt}
\small
\begin{align}
 \hspace{-5pt} \textit{PoA}^{PA}  = \frac{C^{PA,NE}_w}{C^{PA,OPT}(\mathbf{p^{PA,OPT}})},
\label{eq:poa_pa}
\end{align}
\normalsize
where the $C^{PA,NE}_w$ is the worst case social cost of the distributed, uncoordinated mechanism for the case of interest. Note that $C^{PA,OPT}(\mathbf{p^{PA,OPT}})$ is uniquely determined for each particular case.

In order to obtain $C^{PA,NE}_w$, we can solve a simple optimization problem to minimize the social cost $C^{PA,NE}(\mathbf{p^{PA,NE}})$ with respect to $\mathbf{p^{PA,NE}}$ (when there are multiple possible NE e.g., cases 2(a), 2(b) and 4 and subject to the corresponding probability constraints using a software optimization tool. Importantly, for the uncoordinated energy selection under PA, minimizing $C^{PA,NE}(\mathbf{p^{PA,NE}})$  is equivalent to minimizing the night-zone cost. The last observation is due to the fact that the demand $D^{PA,NE}$ is constant with respect to $\mathbf{p^{PA,NE}}$. 

In the special case of the risk-seeking consumers, from Eq. \eqref{eq:social_cost_pa_sc}, the social cost is constant with respect to the probabilities $\mathbf{p^{PA,NE}}$ for each case of energy profile values. In this case, $C^{PA,NE}_w$ is given by Eq. \eqref{eq:social_cost_pa_sc}.

For the risk-conservative consumers, assume the simple case of two energy profiles. Then, in all cases except subcase 2(a), the social cost is uniquely determined giving directly the value of $C^{PA,NE}_w$. For subcase 2(a)  the multiple combinations of probabilities can lead to NE with possibly different social cost values. Under the conditions of subcase (a), we can show that $\epsilon_1>\epsilon_0$. Thus, in this case the social cost is decreasing with $p_{RES,1}^{PA,NE}$  more than with $p_{RES,0}^{PA,NE}$, and its worst case value, $C^{PA,NE}_w$, is obtained using the maximum value of $p_{RES,0}^{PA,NE}$ and minimum of $p_{RES,1}^{PA,NE}$ from the range in Eq. \eqref{eq:prop_alloc_pa_bounds_0_extra_demand}.

For the ES allocation, $\textit{PoA}^{ES}$ is defined in a similar way with $\textit{PoA}^{PA}$ and we study it numerically in Section \ref{sec:eval}.
%\subsubsection{Equal Sharing}\label{sec:opt_es_central_no_extra_demand}
%In this section, we examine the decisions of a centralized coordination mechanism for the probabilities that users of each energy profile will opt for RES, denoted as $p^{ES,OPT}_{RES,\theta_i}$, $\theta_i \in \Theta$, under equal sharing.
%
%%Under an ideal optimal centralized coordination mechanism that equally allocates the available RES capacity to competing consumers, the derivation of the associated competing probabilities $p^{ES,OPT}_{RES,0}$ and $p^{ES,OPT}_{RES,1}$ factors in two distinct cases: (a) $E_0=E_1=E$ and (b) $E_0 <  E_1$. In the first case, 
%If $E_0=E_1=E$ the two renewable energy allocation policies are equivalent and therefore, the decisions of the centralized mechanism are the same as those in Section \ref{sec:opt_pa_central_no_extra_demand}. 
%
%Differently, if $E_0 <  E_1$ we distinguish the following cases: %the centrally computed probabilities that optimize the social cost (Ref. eq. (\ref{eq:social_cost_es_extra_demand})) are described by Table \ref{tb:opt_es_extra}.
%
%
%%\begin{table}[]
%%\centering
%%\caption{Probabilities under centralized coordination and equal sharing.}
%%\footnotesize
%%\label{tb:opt_es_extra}
%%\begin{tabular}{lcl}
%% $p^{ES,OPT}_{RES,0}$ \hspace{150pt}  $p^{ES,OPT}_{RES,1}$\\ \hline
%%  0 \hspace{165pt}   $min\left(1, \frac{\mathcal{ER}}{(1-r)NE_1}\right) $ \\ 
%% $min\left(1, \frac{\mathcal{ER}}{rNE_0}\right) $ \hspace{145pt}   0\\ 
%% 1 \hspace{70pt}   $min\left(1,max\left(0,\frac{1}{(1-r)}\left[\sqrt{\frac{\mathcal{ER}r(\gamma-1)}{E_1N(\gamma-\epsilon_1\beta)}} - r\right] \right)\right)$\\
%% 1 \hspace{105pt}  $min\left(1,max\left(0, \frac{1}{(1-r)}\left(\frac{\mathcal{ER}}{E_0N}-r\right)\right)\right)$\\
%% $min\left(1,max\left(0, \frac{1}{rN}\left[\frac{\mathcal{ER}}{E_1}-(1-r)N\right]\right)\right)$ \hspace{50pt}   1\\  
%%  $min\left(1,max\left(0, \frac{1}{rN}\left[\frac{\mathcal{ER}}{E_0}-(1-r)N\right]\right)\right)$ \hspace{50pt}   1\\  
%%\end{tabular}
%%\vspace{-5pt}
%%\end{table}
%%\normalsize
%
%
%\textbf{Case $1$.} The RES capacity exceeds the aggregated consumer demand. Then, all consumers (for both cases of risk-seeking and risk-conservative) are directed to the RES and $p^{ES,OPT}_{RES,\theta_i}=1$, $\forall~\theta_i \in \Theta$.
%
%\textbf{Case $2$.} Each one of the quantities $rN E_0$ and $(1-r) N E_1$ exceed the RES capacity. Then, (i) if $\epsilon_i \geq \frac{\gamma}{\beta}, \forall i \in \mathcal{N}$, $p^{ES,OPT}_{RES,0}=1$, $p^{ES,OPT}_{RES,1}=1$ (shown as in Case $3$, Section \ref{sec:prop_alloc_eq_extra_demand}) and (ii) if $\gamma> min(\epsilon_0\beta, \epsilon_1\beta)$ then all consumers competing for RES should have the same energy profile. Thus, the renewable energy will not remain unused due to the equal sharing allocation. % (by providing energy shares that exceed low-to-moderate energy demand, $E_0$) while consumers incur congestion penalties (by providing energy shares not sufficient to respond to their energy demand).
%For case (ii), the centralized coordination mechanism allocates the RES exclusively to consumers of energy profile, $\vartheta_i$, coupled with the highest risk-aversion degree, i.e., $\epsilon_{\vartheta_i}>\epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$. This is shown in a similar way as in Case $3$ of Section \ref{sec:opt_pa_central_no_extra_demand} and considering that the demand for RES will be equal to $\mathcal{ER}$ and will be equal to the aggregate of the allocated RES to all consumers.%, namely, to consumers with the highest cost for reneging from competition, $\epsilon_{\vartheta_i}\beta$.
% For instance, if $\epsilon_0\geq\epsilon_1$ the competing probabilities under optimal allocation are $p^{ES,OPT}_{RES,1}=0$ and $p^{ES,OPT}_{RES,0}=min\left(1, \frac{\mathcal{ER}}{rNE_0}\right)$, if $\gamma >\epsilon_0\beta$, or $p^{ES,OPT}_{RES,0}=1$, otherwise. Similarly, if $\epsilon_1\geq\epsilon_0$ the competing probabilities under optimal allocation are $p^{ES,OPT}_{RES,0}=0$ and $p^{ES,OPT}_{RES,1}<min\left(1, \frac{\mathcal{ER}}{(1-r)NE_1}\right) $, if $\gamma > \epsilon_1\beta$, or $p^{ES,OPT}_{RES,1}=1$, otherwise.
%
%\textbf{Case $3$.} Each one of the quantities $rN E_0$ and $(1-r) N E_1$ by itself does not exceed the RES capacity. Then, if also $\epsilon_i \geq \frac{\gamma}{\beta}, \forall i \in \mathcal{N}$, then $p^{ES,OPT}_{RES,0}=1$, $p^{ES,OPT}_{RES,1}=1$ (shown as in Case $3$, Section \ref{sec:prop_alloc_eq_extra_demand}). However, the under other conditions, the solution is more complicated and can be derived by a tool such as Mathematica or MATLAB.
%
%%Under lower aggregate demand levels, the coordination mechanism allows serving with RES heterogeneous energy consumption profiles, taking into consideration first the degree of risk-aversion of the two classes of consumers  and second the aggregate demand shaped by each class. The resulting competing probabilities are drawn from Table \ref{tb:opt_es_extra}, starting from $p^{ES,OPT}_{RES,0}=p^{ES,OPT}_{RES,1}=1$ for low aggregate demand and converging to the previously cited values when both the aggregate demands shaped by low-to-moderate and high energy consumers exceed the RES capacity.
%
%The Price of Anarchy derives in a similar fashion as in Section \ref{sec:opt_pa_central_no_extra_demand} and we omit the details due to lack of space. Notice that for the uncoordinated scheme, the social cost is uniquely determined for all cases with respect to the consumers behavior (e.g., risk-seeking and risk-conservative), risk-aversion degree values and energy consumption values $E_0$, $E_1$ except the following one. Specifically, for the risk-conservative consumers, the social cost depends on the choice of $p^{ES,NE}$ (Eq. \eqref{eq:social_cost_es_extra_demand}). The latter dependence is of interest under the conditions of the first line of  Table \ref{table_eq_comp_pro}, since it is the only case where there exist multiple combinations of probabilities that can lead to equilibria. We can obtain the worst social cost by  comparing the cases (i) maximum value of $p_{RES,0}^{ES,NE}$ and minimum of $p_{RES,1}^{ES,NE}$ (from the ranges in Eqs. \eqref{eq:prop_alloc_eq_bounds_0_extra_demand}, \eqref{eq:prop_alloc_eq_bounds_1_extra_demand}), (ii) minimum value of $p_{RES,0}^{ES,NE}$ and maximum of $p_{RES,1}^{ES,NE}$, choosing the one that leads to the highest social cost.
%
%%\emph{Price of Anarchy:} %Concerning the (in)efficiency of equilibria, 
%%By Section \ref{sec:eq_sharing_eq_extra_demand}, under risk-seeking consumers, the equilibrium states are possible if $E_0=E_1$ which returns $\textit{PoA}^{ES}=\textit{PoA}^{PA}$. On the other hand, under risk-conservative consumers,  %equilibrium states are possible also under asymmetric energy consumption profiles. In this case, 
%%the social cost is a non-increasing function of the competing probability of the competitors of high energy demand (\ie $\frac{d C(p^{ES,NE})}{d p^{ES,NE}_{RES,1}}\leq 0$) and therefore the worst-case equilibrium occurs at $p'$ with $p'_{RES,1}=min(p^{ES,NE}_{RES,1})$ ($p'_{RES,0}=max (p^{ES,NE}_{RES,0})$). By (\ref{eq:social_cost_es_extra_demand}), the associated PoA is 
%%
%%
%%\vspace{-5pt}
%%\small
%%\begin{eqnarray}
%% \hspace{-5pt} \textit{PoA}^{ES}  &=& \frac{C(p')}{C(p^{ES,OPT})}
%%\label{eq:poa_es}
%%\end{eqnarray}
%%\normalsize
%
%%where both the social costs $C(p')$ and $C(p^{ES,OPT})$ are derived by (\ref{eq:social_cost_es_extra_demand}).
%
%%\subsection{Decentralized Coordination Mechanisms}\label{sec:opt_decentral_no_extra_demand}
%
%%Although the centralized coordination mechanisms ensure optimal efficiency in the energy source allocation, they need to pursue incentives that would engage the autonomous and selfish consumers into socially efficient actions. Otherwise, supervisory implementations need to vouch for system stability and robustness, since selfish behaviors can undermine its performance significantly. The analysis in Section \ref{sec:uncoordinated_extra_demand} suggests that two important factors \emph{under the control} of micro-grid operator(s), affect the game equilibrium competing probabilities. These factors are the renewable energy capacity, $\mathcal{ER}$, and the applied pricing scheme on the two energy sources. Typically, in the long-term, the operator copes with the energy demand and the emerging inefficiencies through strategic planning of $\mathcal{ER}$, involving re-dimensioning of the distribution network side (\eg solar panels or wind turbines). Whereas, in the short-term, it can do so by manipulating the prices charged for the two types of energy sources. In the sequel, we systematically study conditions on $\mathcal{ER}$ and pricing that optimize the distributed energy source selection in large-scale settings where both the aggregate demands shaped by low-to-moderate and high energy consumers exceed $\mathcal{ER}$.
%%
%%\subsubsection{Proportional Allocation}\label{sec:opt_pa_decentral_no_extra_demand}
%%
%%%On the one hand, by Sections \ref{sec:prop_alloc_eq}, under proportional allocation the competing influences are balanced if $rse^{NE}_{\vartheta_i}(\cdot)=rse^{PA}_{\vartheta_i}(\cdot)$. On the other hand, by equation (\ref{eq:optimal}), optimal utilization of renewable energy along with elimination of congestion penalties are possible if the renewable energy demand matches the supply.
%%%
%%%Overall, under the case of risk-seeking consumers, by equations (\ref{eq:prop_alloc_energy}), (\ref{eq:conditionEQ}) and (\ref{eq:optimal}) (alternatively by (\ref{eq:demand_pa_ne_no_extra_demand})), the uncoordinated energy source selection converges to the optimal coordinated energy source allocation only if $E_0=E_1=E$ and the renewable energy capacity is dimensioned according to
%%%
%%%\vspace{-5pt}
%%%\small
%%%\begin{equation}
%%%\mathcal{ER}^{OPT}=\frac{E \cdot N}{\frac{(\gamma-1)N}{(\gamma-\beta)}-(N-1)}
%%%\label{eq:optimal_ER_proportional_no_extra_demand}
%%%\end{equation}
%%%\normalsize
%%%
%%%or the charging costs satisfy
%%%
%%%\vspace{-5pt}
%%%\small
%%%\begin{equation}
%%%\frac{(\gamma-1)}{(\gamma-\beta)}\vert ^{OPT}=\frac{N-1}{N}+\frac{E}{\mathcal{ER}}
%%%\label{eq:optimal_pricing_proportional_no_extra_demand}
%%%\end{equation}
%%%\normalsize
%%
%%%Under the case of risk-conservative consumers, by equations (\ref{eq:prop_alloc_energy}), (\ref{eq:conditionEQ_extra_demand}) and (\ref{eq:optimal}) (alternatively by (\ref{eq:demand_pa_ne_extra_demand})), the uncoordinated energy source selection converges to the optimal coordinated energy source allocation if the renewable energy capacity is dimensioned according to
%%
%%By Section \ref{sec:opt_pa_central_no_extra_demand}, if $\epsilon_{\vartheta_i}<\gamma/\beta$, $\forall i\in \mathcal{N}$, optimal RES utilization along with elimination of congestion penalties are possible if the renewable energy demand matches the supply. Jointly by Table \ref{table_eq_comp_pro} and Section \ref{sec:opt_pa_central_no_extra_demand}, the optimization of the uncoordinated energy source selection requires dimensioning and pricing according to
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\mathcal{ER}^{OPT}=\frac{E_{\vartheta_i}N}{\frac{(\gamma-1)N}{(\gamma-\epsilon_{\vartheta_i}\beta) }-(N-1)} >0
%%\label{eq:optimal_ER_proportional_extra_demand}
%%\end{equation}
%%\normalsize
%%
%%%or the charging costs satisfy
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}\vert ^{OPT}=E_{\vartheta_i}\left[\frac{N-1}{N}+\frac{1}{\mathcal{ER}}\right] >1
%%\label{eq:optimal_pricing_proportional_extra_demand}
%%\end{equation}
%%\normalsize
%%
%%with $\epsilon_{\vartheta_i}>\epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$. Namely, the distributed energy source selection is optimized by allocating the RES only to consumers with the highest cost for reneging from competition, $\epsilon_{\vartheta_i}\beta$. Likewise, in the symmetric case where $\epsilon_{\vartheta_i}=\epsilon'<\gamma/\beta$, $\forall i\in \mathcal{N}$, by Table \ref{table_eq_comp_pro}, (\ref{eq:prop_alloc_opt_bounds_0}) and  (\ref{eq:prop_alloc_opt_bounds_1}), the values for $\mathcal{ER}$ and charging costs that optimize the efficiency of equilibria are also given by (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}) with $\vartheta_i=0$, when $E_0 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$ or $E_1 > max(\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}, \frac{E_0}{1-\frac{(N-1)}{N}\frac{(\gamma-\epsilon_0\beta)}{(\gamma-1)}})$. 
%%
%%Furthermore, in settings where $\exists i \in \mathcal{N} : \epsilon_{\vartheta_i}\geq\gamma/\beta$, by Table \ref{table_eq_comp_pro} and (\ref{eq:prop_alloc_opt_p_cond}), the optimal distributed energy selection is possible by prioritizing the use of RES facility by consumers that incur the highest cost for reneging from competition, $\epsilon_{\vartheta_i}\beta$, yet not blocking the other consumption profile from the distribution of the remaining RES capacity. In this case the optimal values for the renewable energy capacity and the charging costs are determined according to (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}) with $\epsilon_{\vartheta_i}<\epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$. If $\epsilon_{\vartheta_i}\geq\gamma/\beta$, $\forall i\in \mathcal{N}$, the dominant strategy for all consumer to compete for the renewable energy source is also the optimal one.
%%
%%The optimization of the distributed energy source selection by adopting particular values for the RES capacity and the charging costs, requires that both the equilibrium states and the optimal operation prioritize the same class(ses) of consumers in accessing the RES facility: if $E_0 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$, $E_1 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$ and $\epsilon_0<\epsilon_1<\gamma/\beta$ or if 
%%$E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$, $\forall i\in \mathcal{N}$, the price of the lack of coordination in the equilibria cannot be avoided by the decentralized mechanism. Overall, the use of optimal values for the RES capacity and the charging costs yields $\textit{PoA}^{PA} =1$, with the exception of settings where there is a unique optimal competing probability vector while the equilibrium states vary over a proper probability interval (\ie  when $E_0 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$,  $E_1 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$, $\epsilon_0<\epsilon_1$). In this case, the worst-case equilibrium occurs at $p'$ with $p'_{RES,1}=min(p^{PA,NE}_{RES,1})$ ($p'_{RES,0}=max (p^{PA,NE}_{RES,0})$) and the associated PoA is given by (\ref{eq:poa_pa}).
%%
%%%while they do not break condition (\ref{eq:relation_E_0_E_1_pa_ne_extra_demand}) that dictates the relation between $E_0$ and $E_1$ factoring in the renewable energy capacity and the charging costs. 
%%
%%%Ultimately, these values for the renewable energy capacity and charging costs optimize the efficiency of equilibria, yielding $\textit{PoA}^{PA} =1$.
%%
%%
%%\subsubsection{Equal Sharing}\label{sec:opt_es_decentral_no_extra_demand}
%%
%%By Section \ref{sec:eq_sharing_eq_extra_demand}, in the distributed energy source selection by risk-seeking consumers the equilibrium states under equal sharing and proportional allocation coincide, and hence the RES capacity and the charging costs that optimize the efficiency of the uncoordinated selection process ($\textit{PoA}^{ES} =1$) are given by equations (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}).
%%%By Section \ref{sec:eq_sharing_eq_extra_demand}, 
%%When the consumers are risk-conservative, a trivial but expensive methodology to optimize the distributed energy source selection amounts to increasing $\mathcal{ER}$ to guarantee that the faire shares suffice to serve all requests, \ie $\mathcal{ER}/N \geq E_1$. Alternatively, in settings with $\epsilon_{\vartheta_i}<\gamma/\beta$, $\forall i\in \mathcal{N}$, by Tables \ref{table_eq_comp_pro} and \ref{tb:opt_es_extra}, the decentralized optimization of energy source selection is realized under the same conditions as in proportional allocation (Ref. Section \ref{sec:opt_pa_decentral_no_extra_demand}).
%%
%%Otherwise, in settings where $\exists \epsilon_{\vartheta_i}, \epsilon_{\vartheta_j}:\epsilon_{\vartheta_i}\geq\gamma/\beta> \epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$, by Tables \ref{table_eq_comp_pro} and \ref{tb:opt_es_extra},  
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\mathcal{ER}^{OPT}=\frac{N}{\frac{(\gamma-1)N}{(\gamma-\epsilon_{\vartheta_j}\beta) E_{\vartheta_j}}-\frac{(N-1)}{E_{\vartheta_i}}} > 0
%%\label{eq:optimal_ER_ES_extra_demand1}
%%\end{equation}
%%\normalsize
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}\vert ^{OPT}=E_{\vartheta_j}\left[\frac{N-1}{NE_{\vartheta_i}}+\frac{1}{\mathcal{ER}}\right] > 1 
%%\label{eq:optimal_pricing_ES_extra_demand1}
%%\end{equation}
%%\normalsize
%%
%%which return $\textit{PoA}^{ES} =1$. In addition, by Table \ref{table_eq_comp_pro} and Section \ref{sec:opt_es_central_no_extra_demand}, if $\epsilon_{\vartheta_i}\geq\gamma/\beta$, $\forall i\in \mathcal{N}$, the dominant competing strategy equals to the optimal one.
%%
%%In a last note, the benefit of these decentralized coordination approaches can be also quantified by the Price of Stability (\textit{PoS}) which is a measure of inefficiency designed to differentiate between games in which \textit{all} equilibria are inefficient and those in which \textit{some} equilibria are inefficient \cite{Nisan07}. It is a ratio between the best objective function value at equilibrium and that of the optimal outcome. In the energy source selection game, with parametrization according to (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}) or (\ref{eq:optimal_ER_ES_extra_demand1}) and (\ref{eq:optimal_pricing_ES_extra_demand1}), the best-case equilibrium emerges at the optimal competing probabilities. Therefore, these decentralized coordination approaches guarantee $\textit{PoS}=1$.
%%
%% %emerges at $p'$ with $p'_{RES,1}=supremum(p^{ES,NE}_{RES,1})$ ($p'_{RES,0}=infimum (p^{ES,NE}_{RES,0})$) or $p'_{RES,1}=infimum(p^{ES,NE}_{RES,1})$ ($p'_{RES,0}=supremum (p^{ES,NE}_{RES,0})$), respectively. Therefore, these decentralized coordination approaches guarantee $\textit{PoS}=1$.
%%
%%


==> old/coordinated_lesia.tex <==
x\section{Centralized Energy Source Allocation Mechanism}\label{sec:coordinated}

In this section, we study the case in which a central energy community coordinator allocates the different energy resources among the $N$ consumers in the energy community so as to minimize the social cost of the overall community. This centralized energy source allocation mechanism (ESAM) is used as a ideal benchmark against which to evaluate the efficiency of the proposed decentralized ESSG.

\subsection{Optimization Problem Formulation}

In practice, in the ESAM, all consumers $i$ with type $\vartheta_i$ communicate their daily flexible load $U_{\vartheta_i}$ and risk-aversion degree $\mu_{\vartheta_i}$ (such that their day-time energy demand $E_{\vartheta_i}= \mu_{\vartheta_i}U_{\vartheta_i}$) to a central energy community coordinator. 
%Therefore, the aggregate amount of day-time loads is equal to $D^{Total}$. 
This coordinator optimally schedules the loads of the consumers during each time period (i.e. day or night) by selecting the optimal vector of mixed-strategies $\mathbf{p}^{OPT}=[\mathbf{p_0}^{OPT^\top};...;\mathbf{p_{M-1}}^{OPT^\top}]$ that minimizes the social cost $C(\mathbf{p}^{OPT})$ of the overall community. For each consumer $i$ of type $\vartheta_i$, the vector $\mathbf{p}^{OPT}_{\vartheta_i} = [\mathbf{p}^{OPT}_{RES,\vartheta_i},\mathbf{p}^{OPT}_{nonRES,\vartheta_i}]$ is defined, similarly to $\mathbf{p}^{NE}_{\vartheta_i}$, such that the share of their daily flexible load scheduled during the day equals $p^{OPT}_{RES,\vartheta_i}E_{\vartheta_i}$, and the share of their daily flexible load scheduled during the night equals $p^{OPT}_{nonRES,\vartheta_i}U_{\vartheta_i}$. 

As a result, this centralized ESAM is modelled as an optimization problem, defined as:

 \vspace{-0.1in} 
 \begin{small}
 \begin{subequations} \label{eq:social_cost_x_opt}
\begin{alignat}{2}
& \min_{\mathbf{p}^{OPT}} \ && C(\mathbf{p}^{OPT}) = \min\Bigl\{ \mathcal{ER}, N \sum_{{\ell} \in \Theta} r_{\ell} p_{RES,{\ell}}^{OPT}  E_{\ell}\Bigr\}  c_{RES} \nonumber \\ 
& \quad && + \max \Bigl\{ 0,N \sum_{{\ell} \in \Theta} r_{\ell} p_{RES,{\ell}}^{OPT}  E_{\ell}- \mathcal{ER}\Bigr\}  c_{nonRES}\nonumber \\
& \quad && + N  \sum_{{\ell} \in \Theta} r_{{\ell} }p^{OPT}_{nonRES,{\ell}}\varepsilon_{{\ell} }E_{{\ell}} c_{nonRES,N} \label{eq:opt_1} \\
 & \text{s.t. } && 0 \leq p^{OPT}_{RES,\ell} \leq 1 ,  \ \forall \ell \in \Theta \label{eq:opt_2} \\
  & \quad && 0 \leq p^{OPT}_{nonRES,\ell} \leq 1 ,  \ \forall \ell \in \Theta \label{eq:opt_3} \\
 & \quad && p^{OPT}_{RES,\ell} + p^{OPT}_{nonRES,\ell} = 1 , \ \forall \ell \in \Theta, \label{eq:opt_4}
 \end{alignat}
 \end{subequations}
\end{small} \vspace{-0.1in}  

\noindent which minimizes the objective function \eqref{eq:opt_1}, representing the social cost of the community, subject to constraints \eqref{eq:opt_2}-\eqref{eq:opt_4} defining the mixed-strategy probabilities. 
%\noindent where, the decision variables of the centralized mechanism are the optimal probability distributions ($p^{OPT}_{RES,\vartheta_i}$, $p^{OPT}_{nonRES,\vartheta_i}$), which represent the optimal probability that consumer $i$ with type $\vartheta_i$ engages its load during day, or during the night, respectively, for all consumers $i \in \mathcal{N}$. \footnote{The vector $\mathbf{p^{OPT}}$ is defined similarly to $\mathbf{p^{NE}}$.}

%where $N  \sum_{{\ell}\in \Theta} r_{\ell} p_{RES,{\ell}}^{OPT}  E_{\ell} $ represents the total RES production allocated in the day-zone, and $N  \sum_{{\ell} \in \Theta} r_{{\ell} }p^{OPT}_{nonRES,{\ell}}\varepsilon_{{\ell} }E_{{\ell}}$ represents the total nonRES production allocated in the night-zone. %The first summand refers to the consumers who are served by low-cost RES capacity during the day. The second summand is for the consumers who are served $nonRES$ duing the night-zone. 
%In other words, the part of the optimal social cost that corresponds to the day-zone peak-load production will be zero. %The social costs under the PA and ES policies are defined similarly to Eqs. \eqref{eq:social_cost_pa_extra_demand} and \eqref{eq:social_cost_es}, respectively. 


%The optimal solutions of this centralized mechanism will provide a benchmark against which to evaluate the side-effects that stem from the distributed, uncoordinated energy source selection, in terms of social cost. 
Although this optimization problem is nonconvex, due to its objective function, it can be linearized or formulated as an equivalent optimization problem depending on the values of RES capacity and the preferences of the consumers, i.e. their daily flexible loads and risk-aversion degrees.
In the following, we provide insights and analytical formulations of the optimal solutions $\mathbf{p^{OPT}}$ and objective cost $C(\mathbf{p^{OPT}})$ of this centralized ESAM in each one of the four cases described in Section \ref{sec:uncoordinated_extra_demand}. 

%and the PoA under the PA mechanism. %For the ES mechanism, the centralized decisions for minimizing the social cost are harder to derive analytically and we will present numerical evaluations in Section \ref{sec:eval} using software optimization tools, namely, Mathematica and MATLAB.

\subsection{Optimal Centralized Solutions}

%%%%%%%%% define these costs under each allocation policy!!!????
%We derive the properties of the solution provided by the centralized mechanism, $\mathbf{p^{OPT}}$, in four cases, identical to the ones defined in Section \ref{sec:uncoordinated_extra_demand}.
 
\subsubsection{\textbf{Case $1$: The RES capacity exceeds the maximum day-time energy demand}}

In this trivial case, the social cost reduces to:

 \vspace{-0.1in}
 \begin{small}
\begin{align}
C(\mathbf{p}^{OPT}) & = N \sum_{{\ell} \in \Theta} r_{\ell} p_{RES,{\ell}}^{OPT}  E_{\ell}   c_{RES}  \nonumber \\
& + N  \sum_{{\ell} \in \Theta} r_{{\ell} }p^{OPT}_{nonRES,{\ell}}\varepsilon_{{\ell} }E_{{\ell}} c_{nonRES,N},
 \label{eq:social_cost_x_opt_case1}
 \end{align}
\end{small} \vspace{-0.1in}  

\noindent and the optimal solutions to the centralized ESAM is to schedule all consumers during the day,i.e. $p^{OPT}_{RES,\vartheta_i}=1$, and $p^{OPT}_{nonRES,\vartheta_i}=0$, $\forall \vartheta_i \in \Theta$.

In all other cases considered, the RES capacity is lower than the maximum day-time energy demand.

\subsubsection{\textbf{Case $2$: The risk-aversion degrees of all consumer types are lower than $\gamma/\beta$}}

In this case, it is optimal for the centralized ESAM to schedule loads during the day so that the total RES capacity is utilized, and to schedule the remaining load during the night. Specifically, the social cost reduces to:

 \vspace{-0.1in} 
 \begin{small}
\begin{align}
C(\mathbf{p}^{OPT}) &=  \mathcal{ER} \cdot c_{RES}   \nonumber \\
&+N \left[ \sum_{{\ell} \in \Theta} r_{\ell }p^{OPT}_{nonRES,{\ell}}\varepsilon_{{\ell} }E_{{\ell}}\right] c_{nonRES,N}
 \label{eq:social_cost_pa_extra_demand_2}
 \end{align}
\end{small} \vspace{-0.1in}  

\noindent Therefore, the centralized ESAM optimization problem \eqref{eq:social_cost_x_opt} is equivalent to minimizing the night-time cost $N \left[ \sum_{{\ell} \in \Theta} r_{\ell }p^{OPT}_{nonRES,{\ell}}\varepsilon_{{\ell} }E_{{\ell}}\right] c_{nonRES,N}$, subject to constraints \eqref{eq:opt_2}-\eqref{eq:opt_4} and the condition that the total energy demand for RES equals the RES capacity:

 \vspace{-0.1in} 
 \small
\begin{align}
N \sum_{{\ell} \in \Theta}r_{{\ell}} E_{{\ell}}p^{OPT}_{RES,{\ell}}=\mathcal{ER}.
\label{eq:optimal}
\end{align}
\normalsize 
\vspace{-0.1in}  

\noindent As a result, the optimal competing probabilities $p^{OPT}_{RES,\vartheta_i}$ for all $ \vartheta_i \in \Theta$ lie in the range:

 \vspace{-0.1in} 
 \footnotesize
\begin{align}
 \hspace{-5pt} 
 \Biggl[max\left\{0,\frac{\left[\mathcal{ER} -\sum_{{\ell} \in \Theta \setminus \{\vartheta_i\}}r_{{\ell}}N E_{{\ell}}\right]}{r_{\vartheta_i}N E_{\vartheta_i}}\right\},
   %\notag\\
    % min\left(1,\mathcal{ER} \frac{1}{rNE_0}\right)
    min\left\{1,\frac{\mathcal{ER}}{r_{\vartheta_i}N E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_opt_bounds_0}
\end{align}
\normalsize 
\vspace{-0.1in}  

\subsubsection{\textbf{Case $3$: The risk-aversion degrees of all consumer types are greater than $ \gamma/\beta$}}

In this case, the optimal solutions to the centralized ESAM is to schedule all consumers during the day, i.e. $p^{OPT}_{RES,\vartheta_i}=1$ and $p^{OPT}_{onRES,\vartheta_i}=0$ $\forall \vartheta_i \in \Theta$. This result is derived in a similar fashion with the result of Case $3$ in Section \ref{sec:uncoordinated_extra_demand}.
 
\subsubsection{\textbf{Case $4$: The risk aversion degrees of certain consumer types are lower than $ \gamma/\beta$ (set $\Sigma_1$), while others are greater than $ \gamma/\beta$ (set $\Sigma_2$)}}

Then, it is optimal for the centralized ESAM to schedule all consumers whose types are in the set $\Sigma_1$ during the day, i.e., $p^{OPT}_{RES,\vartheta_i}=1$ $\forall \vartheta_i \in \Sigma_1$. Furthermore, the social cost of the remaining consumers whose types are in $\Sigma_2$ can be expressed as: 

 \vspace{-0.1in} 
 \begin{small}
\begin{align}
C_{\Sigma_2}(\mathbf{p}^{OPT}) &=  (\mathcal{ER} - \sum_{\ell \in \Sigma_1} r_\ell N E_\ell )\cdot c_{RES}   \nonumber \\
&+N \left[ \sum_{{\ell} \in \Theta} r_{\ell }p^{OPT}_{nonRES,{\ell}}\varepsilon_{{\ell} }E_{{\ell}}\right] c_{nonRES,N}
 \label{eq:social_cost_pa_extra_demand_2}
 \end{align}
\end{small} \vspace{-0.1in}  

\noindent where $ \mathcal{ER} - \sum_{\ell \in \Sigma_1} r_\ell N E_\ell $ represents the remaining available RES capacity, i.e., the available RES capacity minus the aggregate demand of consumers whose types are in $\Sigma_1$ and are scheduled during the day. 



Therefore, the probability that consumers whose type is in the set $\Sigma_2$ play $RES$ is optimized to minimize their night-time cost, while ensuring that they totally utilize the remaining RES capacity, such that:


 \vspace{-0.1in} 
 \small
\begin{align}
N \sum_{{\ell} \in \Theta}r_{{\ell}} E_{{\ell}}p^{OPT}_{RES,{\ell}}=\mathcal{ER} - \sum_{\ell \in \Sigma_1} r_\ell N E_\ell.
\label{eq:optimal}
\end{align}
\normalsize 
\vspace{-0.1in}  

This centralized problem can be solved using a software optimization tool. And, we show that the optimal competing probabilities $p^{OPT}_{RES,\vartheta_i}$ for all $ \vartheta_i \in \Sigma_2$ lie in the range:

 \vspace{-0.1in} 
 \footnotesize
\begin{align}
&\Biggl[\max\left\{0,\frac{\mathcal{ER}-\sum_{\ell \in \Theta \setminus \{\vartheta_i\}}r_{\ell}N E_{\ell}}{r_{\vartheta_i}N E_{\vartheta_i}}\right\}, \nonumber \\ & \min\left\{1,\frac{\mathcal{ER}-\sum_{ \ell \in \Sigma_1}r_{\ell}N E_{\ell}}{r_{\vartheta_i}N E_{\vartheta_i}}\right\}  \Biggr].
\label{eq:prop_alloc_opt_p_cond}
\end{align}
\normalsize 
\vspace{-0.1in}  

\noindent By analogy with Case $2$, this range is derived similarly to the one defined in \eqref{eq:prop_alloc_opt_bounds_0}.

\subsection{PoA}

The (in)efficiency of equilibrium strategies in the decentralized, uncoordinated mechanism is quantified by the Price of Anarchy (PoA) \cite{Koutsoupias09}. The PoA is expressed as the ratio of the worst case social cost among all mixed strategy NE, denoted as $C^{PA,NE}_w$, over the optimal minimum social cost of the centralized mechanism, denoted as $C(\mathbf{p^{OPT^*}})$, such that:

%\vspace{-5pt}
 \vspace{-0.1in} 
 \small
\begin{align}
 \hspace{-5pt} \textit{PoA}^{PA}  = \frac{C^{PA,NE}_w}{C(\mathbf{p^{OPT^*}})}.
\label{eq:poa_pa}
\end{align}
\normalsize 
\vspace{-0.1in}  

First observe that $C(\mathbf{p^{OPT^*}})$ is uniquely determined for each particular case. Now, in order to obtain $C^{PA,NE}_w$ when there exist multiple possible NE (e.g., in Cases $2$ and $4$), we can solve a simple optimization problem to maximize the social cost $C^{PA,NE}(\mathbf{p^{NE}})$ with respect to $\mathbf{p^{NE}}$ and subject to the corresponding probability constraints for NE defined in Section \ref{sec:uncoordinated_extra_demand}, using a software optimization tool. 

Note that $C^{PA,NE}(\mathbf{p^{NE}})$ takes its optimal value (i.e, minimum value) when the night-time cost is minimized. This solution coincides with the optimal centralized solution and thus in this case PoA takes the optimal (unity) value. 


 %The last observation is the fact that the demand $D^{PA,NE}$ is constant with respect to $\mathbf{p^{PA,NE}}$. Also, in the special case of the risk-seeking consumers, from Eq. \eqref{eq:social_cost_pa_sc}, the social cost is constant with respect to the probabilities $\mathbf{p^{PA,NE}}$ for each case of energy profile values. Thus, $C^{PA,NE}_w$ is given by Eq. \eqref{eq:social_cost_pa_sc}.

%$2$. If having risk-conservative consumers, there exist multiple possible equilibria in the sub-cases 2(a) and 2(c) as well as in case 4. Of course, the multiple combinations of probabilities can lead to NE with possibly different social cost values. Based on the Remark \ref{rem:risk_degrees_relation}, the existence of NE is possible if consumers with lower energy demands have lower risk aversion degrees. Thus, the night cost is minimized if the optimal probabilities for RES take lower values for consumers with lower energy demands. 


==> old/evaluations.tex <==
\section{Numerical Evaluations}
\label{sec:eval}

\subsection{Case Study Setup}

We consider a smart grid with $N=1000$ consumers, divided into $5$ distinct consumer types, with a maximum total demand for RESs $D^{Total} = 4250$. Table \ref{tab:residential} summarizes the consumer types parameters.
\begin{table}[b]
\vspace{-0.15in}
\footnotesize
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
        \hline
        Type $\ell$ & 0 & 1 & 2 & 3 & 4 \\
        \hline 
        $E_\ell$ (kWh)& 2 & 3 & 5 & 10 & 15 \\
        \hline
        $r_\ell$ & 0.20 & 0.40 & 0.30 & 0.07 & 0.03 \\
        \hline
    \end{tabular}
    \caption{Game parameters for residential smart-grid.}
    \vspace{-0.15in}
    \label{tab:residential}
\end{table}
The type distribution and the day-time energy demand levels are selected to be consistent with European households \cite{enerdata}. Most households are moderately energy efficient (types $1$ and $2$), combined with many highly efficient households (type $0$) and few inefficient ones (types $3$ and $4$). Consumers with type $0$ are assumed to be risk-seeking ($\epsilon_0=1$) and the risk-aversion degrees of all other types are determined by  \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}, and are close to $1$. We set the RES price as $c_{RES}=1$ \euro/kWh, and the parameters $\beta=2$ and $\gamma=3$. 

The proposed DRP with PA allocation is compared to a DRP with the naive ES allocation. Under ES, a so-called \textit{fair share} of RESs capacity is computed as

\vspace{-0.1in}
\begin{small}
\begin{align} \label{eq:fairshare}
 sh(\mathbf{p^{ES,NE}}) 
& =\frac{\mathcal{ER}}{ N \sum_{ \ell=0}^{M-1} r_{\ell}  p_{RES,\ell}^{ES,NE}},
\end{align}
\end{small}
\vspace{-0.1in}

\noindent where $  N \sum_{ \ell=0}^{M-1}  r_{\ell}  p_{RES,\ell}^{ES,NE}$ represents the number of consumers competing for $RES$ during the day. Under ES, consumers of type $\ell \in \Theta$ that play $RES$ and have a demand $E_{\ell} \leq sh(\mathbf{p^{ES,NE}})$ are allocated their full demand $E_{\ell} $, and the extra energy that they are entitled to $(sh(\mathbf{p^{ES,NE}})-E_{\ell})$ will remains unused. The remaining RESs capacity is allocated equally between the consumers of type $\ell \in \Theta$ that play $RES$ and have a demand $E_{\ell}$ larger than the fair share $sh(\mathbf{p^{ES,NE}})$. Therefore, the share of RESs received by a consumer $i$ of type $ \vartheta_i \in \Theta$ that plays $RES$ is $rse^{ES}_{\vartheta_i}(\mathbf{n_i}) = \min\left( E_{\vartheta_i}, sh(\mathbf{p^{ES,NE}}\right)$. This allocation policy may result in large inefficiencies due to unused RES capacity, even when the total aggregate demand for RESs $D^{ES,NE} (\mathbf{p^{ES,NE}})$ is higher than $\mathcal{ER}$. Therefore, this allocation policy is solely used as a base-case comparison to the PA allocation considered in this work.


\subsection{Social Costs and PoA}
\vspace{-0.07in}

\begin{figure}[ht!] 
     \centering
     \subfigure[Social Cost (in eurocents). \label{fig:4a}]{
         \includegraphics[width=0.2\textwidth]{plots/social_cost_PA_residential.eps}}
  \subfigure[PoA. \label{fig:4b}]{
         \includegraphics[width=0.2\textwidth]{plots/PoA_PA_residential.eps}}
        \caption{Social cost and PoA under PA rule for residential grid.}\vspace{-0.2in}
        \label{fig:sc_PoA_PA}
\end{figure}

\subsubsection{PA Rule}
Fig. \ref{fig:sc_PoA_PA} shows the social cost and the PoA with increasing $\mathcal{ER}$ that ranges from $5\%$ to $125\%$ of $D^{Total}$. First, we observe that the optimal social cost for the centralized approach decreases linearly with $\mathcal{ER}$. This is because the optimal allocation should equalize the RES demand and capacity, while minimizing the night-time cost. Since here all risk-aversion degrees are equal or close to 1, the cost at night can be approximated as {\small$N \sum_{{\ell} \in \Theta} r_{{\ell} } \cdot p_{nonRES,{\ell}} \cdot \epsilon_{{\ell} } \cdot E_{{\ell}} \cdot c_{nonRES,n}\approx N \sum_{{\ell} \in \Theta} r_{{\ell} } \cdot p_{nonRES,{\ell}} \cdot E_{{\ell}} \cdot c_{nonRES,n}\approx$ $N \sum_{{\ell} \in \Theta} r_{{\ell} } \cdot  E_{{\ell}} \cdot c_{nonRES,n} - \mathcal{ER}\cdot c_{nonRES,n} $}, which is constant with respect to the competing probabilities and linearly decreasing with $\mathcal{ER}$. Using the second in row approximation we can point out one more property of the optimal allocation: the night-time cost is mostly affected by the day-time energy demands and its minimization results in "big players" competing for RESs at the expense of smaller ones. This is indeed observed in our evaluations where consumers with lower day-time energy demand compete for RES with non-zero probability only if all consumers with higher day-time energy demand compete for RES with probability 1 and there exists still available RES capacity. %with type $4$ start competing for RES and only when their competing probability reaches $1$ (as $\mathcal{ER}$ increases) consumers with type $3$ start competing and so on for consumers of types 2 and 1.
%the night-time cost is mostly affected by the energy demand of each type. This explains why for values of $\mathcal{ER} < \mathcal{ER}_{max}$, %the centralized approach favours the types with the highest demand, namely, as $\mathcal{ER}$ increases, consumers with type $4$ start competing for RES and only when their competing probability reaches $1$, only then consumers with type $3$ start competing. Following the trend, type $2$ consumers compete for RES only when type $3$ consumers compete with probability equal to $1$, and so on. Therefore, 
%the PA rule indeed favours "big players" at the expense of smaller ones at the optimal allocation. %As a final note, naturally, for $\mathcal{ER} \geq \mathcal{ER}_{max}$, RES capacity adequately covers all the consumers, thus consumers of all types compete for RES.

On the other hand, for the uncoordinated mechanism the social cost decreases linearly with $\mathcal{ER}$, only when $\mathcal{ER}\in [0.5 D^{Total}, D^{Total}]$. The social cost barely reacts to the initial increase in RES capacity due to the fact that consumers tend to overcompete for RES, even for lower values of RES capacity, as it is observed in the obtained values of the compteting probabilities. Moreover note that the mixed strategy NE solution should satisfy \eqref{eq:probrelation1}, except if this does not give acceptable probability values. Since the maximum value that the right hand side of \eqref{eq:probrelation1} can take is $A^{Total}=D^{Total}- \sum_{ {\vartheta_l}\in \Theta} r_{\vartheta_l} E_{\vartheta_l} $ (when all competing probablilities are equal to $1$), this requirement is only possible if the left hand side is less or equal than $A^{Total}$. With the applied parameter values, the left hand side of \eqref{eq:probrelation1} is equal to $A^{Total}$ for 
$\mathcal{ER} \approx 50\% D^{Total}$. Therefore, for $\mathcal{ER} \geq 50\% D^{Total}$ \eqref{eq:probrelation1} cannot be strictly satisfied and the closest we can get to its satisfaction is by setting the competing probabilities of all consumers equal to $1$. Thus, all consumers compete for RES with probability equal to $1$ and there is extra demand, which costs the high day-time prices. Finally, when $\mathcal{ER}\in [0.5 D^{Total}, D^{Total}]$, the social cost is falling when $\mathcal{ER}$ is increasing because fewer highly priced day-time energy is required.

Fig. \ref{fig:4b} shows the PoA. The most inefficient outcome is  for $\mathcal{ER} \approx 0.5 \cdot D^{Total}$, which is the point that the social cost for the uncoordinated mechanism begins decreasing. This graph can provide valuable insight into how much RES capacity we should install. %in order to achieve the socially most efficient outcome.
We see two zones of high efficiency, namely for low and high RES capacity. In the first zone, this is due to the small gains in cost offered by low RES capacity. In the second, the NE solution has almost converged to the optimal solution and thus social costs are optimal as well. 

Finally, the value of $\mathcal{ER}$ at which PoA reaches its peak (most inefficient outcome) depends on the system model parameters and most importantly on $\beta, \gamma$, since the left hand side of \eqref{eq:probrelation1} includes the quantity $\eta=\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$. For instance if $\beta$ increases, $\eta$ increases and PoA reaches its peak at a lower value of $\mathcal{ER}$. This can be seen in Fig. \ref{fig:sc_PoA_PA_beta_higher} that shows the same evaluations as Fig. \ref{fig:sc_PoA_PA}, but with $\beta=2.5$. As expected, both centralized and uncoordinated social
costs are higher than with $\beta=2$ because with $\beta=2.5$ the night-zone price increases. Moreover, the change in PoA is quite significant: the uncoordinated social cost curve started falling earlier, namely
at $20 \% \cdot D^{Total}$. This is reflected on the PoA graph, which now peaks at
around $1.16$, much lower than before.

\begin{figure}[t] 
     \centering
     \subfigure[Social Cost (in eurocents). \label{fig:12a}]{
         \includegraphics[width=0.2\textwidth]{plots/social_cost_PA_residential_beta.eps}}
  \subfigure[PoA. \label{fig:12b}]{
         \includegraphics[width=0.2\textwidth]{plots/PoA_PA_residential_beta.eps}}
        \caption{Social cost and PoA under PA rule for residential grid with $\beta=2.5$.}\vspace{-0.2in}
        \label{fig:sc_PoA_PA_beta_higher}
\end{figure}


\subsubsection{ES Rule}

\begin{figure}[t] 
     \centering
     \subfigure[Social Cost (in eurocents). \label{fig:11a}]{
         \includegraphics[width=0.2\textwidth]{plots/social_cost_ES_residential.eps}}
  \subfigure[PoA. \label{fig:11b}]{
         \includegraphics[width=0.2\textwidth]{plots/PoA_ES_residential.eps}}
        \caption{Social cost and PoA under ES rule for residential grid.}\vspace{-0.2in}
        \label{fig:sc_PoA_ES}
\end{figure}

Fig. \ref{fig:sc_PoA_ES} shows the social cost and the PoA with increasing $\mathcal{ER}$ ranging from $5\%$ to $125\%$ of $D^{Total}$. 
Both centralized and uncoordinated curves decrease with increasing $\mathcal{ER}$, but not in a linear way contrary to the PA rule (Fig. \ref{fig:sc_PoA_PA}). This is because the social cost for ES is not linear with $\mathcal{ER}$ (see for example \eqref{eq:social_cost_es_sc}). Moreover, we observe that the uncoordinated curve follows the same trend as the PA rule, namely, it is flat for small values of $\mathcal{ER}$ and then it decreases. This is because similarly to the PA rule, consumers tend to overcompete for RES also under the ES rule. %This is seen in the competing probability values obtained in our evaluations and can be explained analytically in a similar way as with the PA rule (using \eqref{eq:probrelationes1}). 
Also, we should note that in the optimal allocation the competing probabilities may not be all equal to $1$ even for $\mathcal{ER}=125\%\mathcal{ER}_{max}$. We can attribute this observation to the fact that smaller players may need to reduce their competing probability in order to increase the RES share and subsequently the RES utilization, even if that means they forgo the chance to pay less. In addition, the social cost for ES is higher than for PA, regardless of the $\mathcal{ER}$ value. This can be easily explained by observing that, under the ES rule, either part of the RES capacity is unused because some consumers have lower demand than their share, or consumers are forced to pay the day-zone nonRES because their share is less than their demand. In both cases, the social cost increases. 

The PoA (Fig \ref{fig:sc_PoA_ES}) takes generally lower values than in the case of the PA rule. On the other hand, the game outcome is $100\%$ efficient only when the RES capacity is $\mathcal{ER}=125\%\mathcal{ER}_{max}$, whereas for the PA rule the PoA is equal to 1 when $\mathcal{ER}= 110\%\mathcal{ER}_{max}$. Hence, using the ES rule over the PA rule maybe more expensive as more RES capacity should be installed for ensuring efficiency of the uncoordinated demand side management. Finally, due to the non-linearity of the social cost function with $\mathcal{ER}$, the PoA curve does not decrease monotonously after the initial peak.


\subsection{Evaluation of Distributed Algorithm}

Here, we evaluate the performance and convergence of the distributed algorithm \ref{algorithm}. For better visualization purposes, we have implemented the algorithm considering two consumer types and the following parameter values: $N=500$, $E_0=100$ kWh, $E_1=200$ kWh, $r_0=0.7$, $r_1=0.3$, $\epsilon_0=1$, $\epsilon_1=1.004$ (derives from \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} using $\epsilon_0$), $c_{RES}=100$ \euro/kWh, $\beta=2$, $\gamma=4$. Also, $D^{Total}=65000$ kWh and $\mathcal{ER}=25\% \cdot D^{Total}=16250$ kWh. We study three capping systems, namely, (i) $cap$ is constant and equal to $0.1$, (ii) $cap=rand$ and (iii) $cap=1$, i.e., practically there is no capping system.

Fig \ref{fig:algo_PA_ES} shows the solution paths given by the algorithm for both PA and ES policies and for all three capping systems. Also, it shows the line of the NE solutions that derive from \eqref{eq:probrelation1} for the PA policy and from \eqref{eq:probrelationes1} for the ES policy. It can be observed that all solution paths converge to a theoretically proven NE. For the constant cap ($cap=0.1$), the solution path oscillates around the $45^{\circ}$ line. Therefore, the achieved NE solution consists of similar competing probability values for both consumer types. Actually, imposing a constant cap greatly dampens any bias towards any type. %If a lower value was chosen for the $cap$ parameter, the effect of the cap would be magnified, since players would be even more restricted when contributing to their type's competing probability. 
If the random cap method is implemented, the solution path is naturally random. On the one hand, no type is systematically favored, at the expense of having no control over the solution path. Lastly, if there is no cap at all, the behavior is different under the PA and ES rules. For the PA policy, the consumer type that plays first gains a considerable advantage (see Fig. \ref{fig:algoPArule}). The behavior is not the same under the ES policy, as we see in Fig. \ref{fig:algoESrule}, since type $1$ achieves a higher competing probability at the end, even if type $0$ plays first. This could be explained by the non linear nature of the corresponding social cost.


\begin{figure}[t] 
     \centering
     \subfigure[PA rule. \label{fig:algoPArule}]{
         \includegraphics[width=0.2\textwidth]{plots/algo_sol_small_grid_PA.eps}}
  \subfigure[ES rule. \label{fig:algoESrule}]{
         \includegraphics[width=0.2\textwidth]{plots/algo_sol_small_grid_ES.eps}}
        \caption{Algorithmic solution under PA and ES rules.}\vspace{-0.2in}
        \label{fig:algo_PA_ES}
\end{figure}


 Tables \ref{tab:algo_sc_PA} and \ref{tab:algo_sc_ES} summarize the evaluation results on the social cost, the demand for RESs and the PoA for the optimal centralized solution as well as for the solution of the distributed algorithm for the three capping systems.

{\footnotesize \begin{table}[h!]
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Solution & Social Cost ($\times 10^6$) & Demand & PoA \\
        \hline 
        Optimal & 11.37 & 16250 & 1\\
        %\hline
       % Worst case & 13.01 & 24324 & 1.14\\
        \hline
        Equal cap & 13.00 & 24321 & 1.14\\
        \hline
        Random cap & 12.99 & 24286 & 1.14\\
        \hline
        No cap & 13.01 & 24324 & 1.14 \\
        \hline
    \end{tabular}
    \caption{Social cost, demand and PoA under the PA rule for centralized and distributed algorithmic solutions.}
    \label{tab:algo_sc_PA}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Solution & Social Cost ($\times 10^6$) & Demand & PoA \\
        \hline 
        Optimal & 12.75 & 16250 & 1\\
       % \hline
        %Worst case & 15.99 & 39253 & 1.25\\
        \hline
        Equal cap & 15.99 & 32281 & 1.25\\
        \hline
        Random cap & 15.98 & 38045 & 1.25\\
        \hline
        No cap & 15.99 & 37137 & 1.25 \\
        \hline
    \end{tabular}
    \caption{Social cost, demand and PoA under the ES rule for centralized and distributed algorithmic solutions.}
    \label{tab:algo_sc_ES}
\end{table}}

For both policies, all three capping methods lead to similar social cost and PoA values. Thus, the choice of capping method can only influence the competing probabilities to introduce a sense of fairness for sharing the RES capacity among the consumer types, without affecting the social cost. With respect to the demand, we can observe that it is much higher for the ES policy, similarly with the social cost. This is due to the fact that consumers overcompete for RES, and particularly small players, leading to wasted renewable energy. 

%As for the demand, at first we see a difference between the PA and ES rules, namely demand is considerably higher in all uncoordinated equilibria under the ES rule than the PA rule. This is due to the incentive that small players have to compete. thus increasing total demand.

Table \ref{tab:convergence} summarizes the convergence results, where one round is equivalent to one player taking their turn to compute their best response. The tolerance is set to $tol=10^{-4}$. If we do not apply a capping scheme the algorithm has the fastest convergence at the expense of fairness to the allocation of RES. This happens, because we do not restrict the rate at which the solution reaches the NE line. Introducing a constant capping system renders convergence slightly worse, but a similar number of rounds is required at every run. %This is due to fact that the first steps of the solution path are identical every time we run the algorithm and the difference comes only from the final steps.
 Note that, although lower values of $cap$ increase fairness among consumer types, they also increase the number of rounds until convergence. Lastly, with the random cap, we have no control over the solution path and thus no control over the convergence speed. This is why we see a big variance in the required number of rounds to convergence. However, most importantly, we see that the number of rounds until convergence is much lower than the number of players ($N=500$), which showcases the efficiency of the algorithm. 

\begin{table}[h!]
    \centering
    \begin{tabular}{|c||c|c|}
        \hline
        Cap method & PA & ES \\
        \hline 
        Equal cap & $18$ & $21-23$ \\
        \hline
        Random cap & $17-27$ & $17-34$ \\
        \hline
        No cap & $14$ & $17-18$ \\
        \hline
    \end{tabular}
    \caption{Rounds until convergence.}
    \label{tab:convergence}
\end{table}

==> old/game.tex <==
\section{Modeling the energy source selection}\label{sec:game}
%\textbf{we need to specify a time-unit of taking the decisions: if we take them only once then (i) ER cannot be known, (ii) why not centralized approach. This is studied for one time interval. Can I decide at a next time interval to move back some loads sent to night rate at a previous interval to ER - intra-day re- scheduling per interval? Nice to describe how this is done. }


We assume a micro-grid with $N$ (eligible) consumers. Let $\mathcal{ER}$ stand for the available RES capacity in energy units (\eg kWh) for the considered time-period in the day-zone. Also, we define the following per unit of energy cost values, namely, (i) $c_{RES}$ for RES, (ii) $c_{nonRES,N} = \beta \cdot c_{RES}$, for night-zone nonRES with $\beta>1$, and (iii) $c_{nonRES,D}= \gamma \cdot  c_{RES}$ for day-zone nonRES with $ \gamma>\beta$. Notice that an \emph{excess penalty cost}, equal to $(\gamma-\beta) \cdot c_{RES}$ per unit of energy load, will be paid by consumers that was engaged in the day-zone but not served due to the limited RES capacity. % and captures the impact of congestion (in case of the uncoordinated competition) for RES. 
All aforementioned costs, as well as the amount of the available RES, $\mathcal{ER}$, are assumed as known to the consumers. %We also assume that the consumers do not increase their demand when opting for the night-zone. 
%The challenge addressed in this paper is finding a distributed and uncoordinated scheduling of the consumer loads in day and night-zones so that the consumers' average cost is minimized. Based on the prices, if the consumers' average cost is minimized, the amount of RES actually used (and not curtailed) should be maximized. %More specifically, we solve the problem of the energy source selection, between RES and night-zone nonRES, by the consumers themselves. %We first present a short discussion on a benchmark centralized solution and afterwards we will discuss the simpler to implement distributed one. 
%
%In time zones when the capacity of RES suffices to serve the entire energy demand, consumers can readily opt for using it and gain the price differential between the two resources. When, however, the demand exceeds the limited RES, an inherent competition emerges that should be factored by consumers in their decision to opt for requesting this resource or not at the particular time period. The underlying assumption is that the decision to opt for the finite RES bears the risk of experiencing the congestion penalties induced by the lack of coordination and pay for the more expensive, top-priced nonRES. Essentially, the main dilemma faced by consumers is whether to compete or not for requesting RES or settle for less favoured time zones and pay for medium-priced energy (assumed being covered by a nonRES facility).
%
%In order to analytically investigate the suffered congestion penalties due to the uncoordinated access to the limited resource, it is important to identify and model those key features and critical parameters that tune the intensity of competition. In this respect, we may consider $N$ consumers that decide between RES and nonRES. The first facility is capacity-constrained and able to serve a total energy demand of $\mathcal{ER}$ energy units (\eg kilowatt-hours, kWh) while the second one responds to every possible level of energy demand, yet heavily burdens the environment producing large amounts of pollutants. In the pricing arena, RES is offered at $c_{RES}$ cost units, whereas for nonRES different rates are used for daily and night energy consumption: moderate-priced night energy rate of $c_{nonRES,N} = \beta \cdot c_{RES}, \beta>1$, units and top-priced daily energy rate of $c_{nonRES,D}= \gamma \cdot  c_{RES}, \gamma>\beta$, units. The excess penalty cost $\delta\cdot c_{RES}$, with $\delta=\gamma-\beta>0$, captures the impact of congestion for RES.

%\textbf{Optimal coordinated RES allocation:} 
The allocation of the available RES, $\mathcal{ER}$, to the consumers could be carried out optimally through a fully coordinated centralized approach. %Typically, smart grid-enabled information flow from and to the consumers could be exploited to ensure that (a) the RES is fully used and fairly distributed among the consumers and (b) no consumer would pay the excess congestion penalty. 
This can be implemented by having consumers issue energy demand requests to a central server that processes the requests; if the aggregate amount of loads does not exceed $\mathcal{ER}$, they are all selected during the day-zone, otherwise, certain loads are selected so that their aggregate amount is less or equal to $\mathcal{ER}$ and the remaining non-selected loads are shifted to the night-zone. Besides the increased communication and processing requirements, a coordinated RES allocation is a complex process that needs to take into account fairness criteria, the complex interplay between energy consuming devices, %the heterogeneity of the micro-grid environments often consisting of fairly diverse components such as electric cars, wind turbines, solar farms and all kinds of different appliances with various capabilities and requirements, weather conditions, 
user preferences/comfort, \etc, and it is not scalable. In addition, a major concern of a centralized solution is the privacy of consumers, since they should reveal their demands/constraints to a central server. Also, there is no guarantee that consumers will report their demands truthfully.
%Note that when consumers increase their demand when avoiding the competition, the optimal allocation becomes more complex since it should compare the aggregate cost for consuming nonRES at day-zone against the aggregate cost for consuming (more) nonRES at night-zone. These decisions are communicated to the consumers through the smart-grid facility. 

%
%
%Under the optimal coordinated energy source allocation scheme, %the full information processing and decision-making tasks lie with a central entity.
%micro-grid operators %, operators of energy efficient neighbourhoods and operators of building blocks that host smart metering 
%use the smart grid-related information so as to coordinate the actions of all different stakeholders involved and secure that (a) the local RES - and storage systems - are optimally used and fairly distributed among consumers and (b) no one would pay the excess congestion penalty. In essence, individual customers/consumers that range from owners/operators of large building and facilities to house customers, are expected to issue energy demand requests to a central server, which monitors RES, possesses precise information about its availability, and assigns it so that the aggregate consumers' cost is minimized. Ideally, the efficient exploitation of the smart meter attributes requires the use of a highly intelligent mechanism which takes into account the complex interplay between energy consuming devices, weather conditions, building dynamics, user preferences and comfort, grid status, availability of RES or storage systems \etc.
%
%Overall, in an micro-grid environment where the aggregate demand exceeds the RES capacity of $\mathcal{ER}$ energy units, %with RES capacity of $\mathcal{ER}$ energy units, whereby such an coordination system serves the energy requests of $N$ consumers that jointly shape an energy demand exceeding the RES capacity, 
%exactly $\mathcal{ER}$ units of demand would be directed to RES and no one would pay the excess congestion penalty cost. Advanced decentralized realizations of optimal coordination mechanisms may optimally shape the $\mathcal{ER}$ capacity, pricing and the energy demand of all different consumers within the operator's entity so as the locally available RES is exploited to the maximum while the needs from purchasing from the top-priced conventional grid are minimized.

%\textbf{Uncoordinated energy source selection:} As already mentioned, the design and implementation of a coordinated energy source selection is complex due to the required information exchange, fairness criteria to be considered, heterogeneity of the micro-grid environments (often consisting of fairly diveRES components such as electric cars, wind turbines, solar farms and all kinds of different appliances with various capabilities and requirements), \etc. 
Consequently, in this paper we investigate a simpler to implement distributed, uncoordinated energy source selection approach. Each consumer acts selfishly aiming at minimizing the cost of the acquired energy. Based on the prices' definitions, if the consumers' average cost is minimized, the amount of RES actually used (and not curtailed) should be maximized. As aforementioned in the introduction, the intuitive tendency to opt for RES combined with its scarcity foster the tragedy of commons effects and highlight the game-theoretic dynamics behind the energy source selection task. Thus, the decision-making on energy source selection can be formulated in game-theoretic terms, whereby $N$ rational players/consumers compete against each other for a capacity of $\mathcal{ER}$ low-cost energy units. We will compare the optimal (theoretical) performance (expressed in terms of the minimum average aggregate consumer cost) achieved via the centralized coordinated energy allocation, against the one under the distributed, uncoordinated approach proposed in this paper. 



%Advanced decentralized realizations of the aforementioned optimal centralized coordination may also be considered, but this is outside the focus of this paper. We are only interested in comparing the optimal (theoretical) performance (expressed in terms of the minimum average aggregate consumer cost) delivered through centralized or decentralized coordinated energy allocation, against that under the (simpler to implement) uncoordinated approach considered in this paper. 

%
%Typically, the research in the optimization of energy grid system operation, amounts to defining and solving a system-level optimization problem based on a centralized objective function. However, under heterogeneous micro-grid networks, often consisting of different components such as electric cars, diesel generators, wind turbines, solar farms and all different appliances with various capabilities and objectives, specific objective function for each individual component should be taken into account. Indeed, considering the demand side, in the absence of central coordination, each consumer acts selfishly aiming at minimizing the cost of the acquired energy. The intuitive tendency to opt for RES combined with its scarcity, foster tragedy of commons effects and highlight the game-theoretic dynamics behind the energy source selection task.
%
 %coming up with optimal decisions for operating their associated energy consuming devices. 
%In doing so, they are assumed here to hold precise information about the RES capacity and the pricing on all energy sources involved (RES, day and nigh time grid energy). They also may or may not hold precise information about the actual demand, \ie competition. These assumptions are fairly realistic and feasible since the decision-making task can be assigned to intelligent meters that leverage the available information (through the communication network layer within the smart grid infrastructure) to perform complex computations and best respond to others' actions. Furthermore, these meters may account for user preferences and comfort in the reasoning process. To this end, we assume \textit{two} generic energy consumption profiles corresponding to low-to-moderate and high consumption level energy users.

\vspace{-2pt}
\subsection{Game setting}\label{sec:game_definition}

Overall, the distributed, uncoordinated decision-making on energy source selection can be expressed via the following game: 
\begin{definition}\label{def:energy_source_game}
An \emph{Energy Source Selection Game} is a tuple
\\$\Gamma=(\mathcal{N}, \mathcal{ER}, \{\vartheta_{i}\}_{i\in \mathcal{N}}, \{A_{i}\}_{i\in\mathcal{N}},  \{w_{A_{i},\vartheta_{i}}\}_{i\in \mathcal{N}})$, where:
\begin{itemize}
\item $\mathcal{N}=\{1,...,N\}$, $N>1$, the set of energy consumers/users acting as players,
\item $\mathcal{ER}>0$, the RES capacity in energy units,
\item $\vartheta_{i} \in \Theta=\{0,1,...,M-1\}$ is the type of user $i$ ($i\in \mathcal{N}$) corresponding to an energy consumption profile (load) with demand of $E_{\vartheta_i}$ energy units. It should hold that $M \leq N$ and it is assumed that $E_0<E_1<...<E_{M-1}$, %where $0$ ($1$) stands for low-to-moderate (high) energy level users with demand of $E_0$ ($E_1$, $E_1 \geq E_0$) energy units,
\item $A_{i} $ is the pure strategy of player $i$ taking values in the set of potential pure strategies $\mathcal{A}=\{RES,nonRES\}$ (same for all consumers $i\in \mathcal{N}$), consisting of the choices ``low-priced renewable-source energy'' (RES) and ``medium-priced night-zone non-renewable-source energy'' (nonRES),
%\item $s_{i}: \Theta \rightarrow A$, the strategy function for each consumer $i\in \mathcal{N}$,
\item $w_{RES,\vartheta_i}$, $w_{nonRES,\vartheta_i}: \mathbb{R}^2 \rightarrow \mathbb{R}$ are cost functions indexed by the pure strategy RES or nonRES, and the user type $i\in \mathcal{N}$. 
\end{itemize}
\end{definition}
In addition, 
\begin{itemize}
\item a consumer has an energy demand level $E_{\ell}$ with probability $r_{\ell}$, where $\sum_{\ell\in \Theta} r_{\ell}=1$,
\item $\mathbf{p}_{\boldsymbol \vartheta_i}=(p_{RES,\vartheta_i}, p_{nonRES,\vartheta_i})^T$ is the mixed strategy of user $i$ with profile $\theta_i$ and let $\mathbf{p}=(\mathbf{p_0}^T;\mathbf{p_1}^T;...;\mathbf{p_{M-1}}^T)$,
\item $\upsilon_{RES, \theta_i}(p)$,  $\upsilon_{nonRES, \theta_i}(p)$ are expected cost values for each pure strategy RES, nonRES, respectively, of user $i$ with type $\theta_i$ given the mixed strategies of all other users; the expected value is over both the strategy choice by other consumers and their energy profile.   
%\item $c_{i}^{N_0}(A_i,\vartheta_i)$ are cost functions under particular type, $\vartheta_i$, and strategy, $A_i$, that are basically determined based on $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$.
%$c_{i}^{(\cdot)}(s(\vartheta),\vartheta)= c_{i}^{(\cdot)}(s_{i}(\vartheta_{i}),s_{-i}(\vartheta_{-i}),\vartheta_{i},\vartheta_{-i})$, are the expected cost functions for each consumer $i\in \mathcal{N}$, for every type profile $\vartheta\in \times_{k=1}^{N}\Theta_{k}$ and strategy profile $s(\vartheta)\in \times_{k=1}^{N}S_{k}$, ($c_{i}^{N_0}(s(\vartheta),\vartheta)$ are cost functions under particular type, $\vartheta$, and strategy, $s(\vartheta)$, profile with $N_0=N-\sum_k \vartheta_k$), that are functions of $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$,
\end{itemize}

The number of users with energy profile $E_\ell$, $\ell \in \Theta$, taking action $RES$, excluding player $i$, is denoted as $n_{\ell}$. %and it is equal to $\sum_{j \in \mathcal{N}\setminus {i}} \mathbf{1}_{(A_j=RES)}\cdot \mathbf{1}_{(\theta_j=\ell)}$. %and similarly the corresponding number of competitors of high energy profile is $n_{1}$ ($=\sum_{j \in \mathcal{N}\setminus {i}} A_j \mathbf{1}_{(\theta_j=1)}$). 
The cost function $w_{RES,\vartheta_i}(.)$, is non-decreasing with the {number} of players competing for RES ($n_{\ell}$,  $\ell \in \Theta$) and has the same value for all players of the {same} energy profile that play the same strategy. Let us denote as $\mathbf{n}=(n_0, n_1,..., n_{M-1})^T$. %consumers who decide to compete for RES undergo the risk of incurring congestion penalties. 
In addition, $w_{RES,\vartheta_i}(.)$ is determined %based on the actions taken by the entire population, on the one side, and 
based on the allocation rule that the micro-grid operator adopts to distribute RES among those who compete for it. %, on the other side. %We denote an action profile by the vector $a=(a_{i},a_{-i})\in\times_{k=1}^{N}A_{k}$, where $a_{-i}$ denotes the actions of all other consumers but player $i$ in the profile $a$. The full set of $2^N$ different action profiles maps into $(N_0+1)(N-N_0+1)$ different action \emph{meta-profiles}, where $N_0$ is the number of low-to-moderate energy consumption users. Each meta-profile $a(k_0,k_1)$, with $k_0$, $k_1$ denoting the number of competitors of low-to-moderate and high energy profile, respectively, encompasses all different action profiles that correspond to the same number of consumers of the two energy profiles competing for RES. The expected costs for these $k_0$, $k_1$ consumers and for the $N-(k_0+k_1)$ ones choosing directly the medium-priced nonRES alternative are functions of $a(k_0,k_1)$ rather than the exact action profile.
Thus, the cost for a consumer $i\in \mathcal{N}$ of consumption profile $\vartheta_i$ (and associated energy demand $E_{\vartheta_i}$) that plays the action $RES$ is:
\begin{small}
\begin{align}
w_{RES,\vartheta_i}(n) =
rse_{\vartheta_i}(n) \cdot c_{RES} + (E_{\vartheta_i}-rse_{\vartheta_i}(n) ) \cdot c_{nonRES,D},
\label{eq:RES_cost}
\end{align}
\end{small}
where $rse_{\vartheta_i}(n) $ is the amount of RES allocated to consumer profile $\vartheta_i$. Note that all consumers $j \neq i, ~j \in \mathcal{N}$ with $\vartheta_j=\vartheta_i$ and strategy RES are granted with the same amount of RES. On the other hand, the cost for those avoiding competition, $w_{nonRES,\vartheta_i}$, is oblivious to others' actions, that is, 
%\vspace{-7pt}
%\small
\begin{equation}
w_{nonRES,\vartheta_i}=E_{\vartheta_i} \cdot c_{nonRES,N}.
\label{eq:nonRES_cost}
\end{equation}
\normalsize
%In general, the cost $c_i^{N_0}(a_i,a_{-i})$ for consumer $i$ under the action profile $a=(a_i,a_{-i})$ is
%
%%\vspace{-10pt}
%\small
%\begin{eqnarray}
%\hspace{-1pt}c_{i}^{N_0}(a_{i},a_{-i})=\left\{
%\begin{array}{l l}
%\hspace{-5pt}w_{RES,\vartheta_i}(N_{RES,0}(a), n_{1}(a)), \text{if~ $a_{i}=RES$} \nonumber\\
%\hspace{-5pt}w_{nonRES,\vartheta_i}, \text{if~ $a_{i}=nonRES$} \nonumber\\
%\end{array} \right.
%\label{equ:consumer_cost_profile}
%\end{eqnarray}
%\normalsize
%
%where $N_{RES,0}(a), n_{1}(a)$ are the numbers of competitors of low-to-moderate and high energy profile \textit{but} player $i$, respectively, under action profile $a$.
Besides the two pure strategies, RES, nonRES, the consumers may also randomize over them\footnote{Note that a pure strategy is a special case of a mixed strategy.}. We mainly draw our attention on symmetric mixed strategies for each energy consumption profile, since these can be more helpful in dictating practical strategies in real systems. In particular, as defined above a player's \emph{mixed strategy} corresponds to a probability distribution $\mathbf{p}_{\boldsymbol \vartheta_i}$. %=(p_{RES,\vartheta_i},p_{nonRES,\vartheta_i})$, where $p_{RES,\vartheta_i}$ and $p_{nonRES,\vartheta_i}$ are the probabilities of selecting the pure strategies RES and nonRES, respectively, with $p_{RES,\vartheta_i}+p_{nonRES,\vartheta_i}=1$ ($\theta_i \in \Theta$). %Also, let $p=(p_0^T;p_1^T)$ be the matrix with lines the symmetric mixed strategies for each energy profile, namely, $p_0=(p_{RES,0}; p_{nonRES,0})$ and $p_1=(p_{RES,1}; p_{nonRES,1})$. %associated with the two energy profiles. 
Assume that consumers play the mixed-action strategy $\mathbf{p}$. In this case, the expected costs for player $i$, with energy profile $\theta_i$, when playing RES (nonRES) is %is a weighted sum of the cost functions $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$ and is given by
%\vspace{-15pt}
%\small
%\begin{eqnarray}\label{eq:costs_symRES}
%    c_{i}(RES,p, p_{0}, p_{1}) = \sum_{N_0=0}^{N-1}\sum_{N_{RES,0}=0}^{N_0}\sum_{n_{1}=0}^{N-1-N_0}    w_{RES,\vartheta_i}(\cdot)  && \nonumber\\
%    \cdot B(n_{1};N-1-N_0,p_{RES,1}) \cdot  B(N_{RES,0};N_0,p_{RES,0}) && \nonumber\\
%      \cdot B(N_0;N-1,p) &&
%    \vspace{-10pt}
%\end{eqnarray}
%\normalsize
%\begin{align}
%   \upsilon_{ \theta_i}^{N_0}(p_0,p_1) = &  p_{RES,\theta_i} ~\upsilon_{RES, \theta_i}^{N_0}(p_0,p_1)  \nonumber \\&  + p_{nonRES,\theta_i} \upsilon_{nonRES, \theta_i}^{N_0}(p_0,p_1),\label{eq:costs_tot}
%\end{align}
%\noindent where the expected costs of the pure strategies RESs, nonRES of consumer $i$ are expressed as
\begin{align}& \upsilon_{RES, \theta_i}(\mathbf{p})=  \sum_{N_{0}=0}^{N}~ \sum_{N_{1}=0}^{N-N_0} ... \sum_{N_{M-1}=0}^{N-\sum_{k=0}^{M-2}{N_k}}\nonumber\\  & \Bigl( \sum_{n_{0}=0}^{N_0-\mathbf{1}_{(\theta_i=0)}}~\sum_{n_{1}=0}^{N_1-\mathbf{1}_{(\theta_i=1)}}...  \sum_{n_{M-1}=0}^{N_{M-1}-\mathbf{1}_{(\theta_i=M-1)}} ~w_{RES,\vartheta_i}(n) \cdot \nonumber\\
 &B(n_{0};N_0-\mathbf{1}_{(\theta_i=0)},p_{RES,0}) \cdot \nonumber \\& B(n_{1};N_1-\mathbf{1}_{(\theta_i=1)},p_{RES,1}) \cdot... \nonumber \\& B(n_{M-1};N_{M-1}-\mathbf{1}_{(\theta_i=M-1)},p_{RES,M-1})\Bigr) \cdot... \nonumber \\&B(N_0;N,r_0)B(N_1;N,r_1)...B(N_{M-1};N,r_{M-1}),  \label{eq:costs_symRES}
\end{align}
\begin{align}
\label{eq:costs_symnonRES}
   \upsilon_{nonRES, \theta_i}(\mathbf{p}) = w_{nonRES,\vartheta_i},
\end{align}
\noindent where $N_{\vartheta_i}$ is the number of consumers of type $\theta_i\in \Theta$, $B(n_{0};N_0-\mathbf{1}_{(\theta_i=0)},p_{RES,0}) $ is the value of the Binomial probability distribution with parameters $N_0-\mathbf{1}_{(\theta_i=0)}$ and $p_{RES,0}$, for $n_{0}$ consumers of energy profile $E_0$ competing for RES, and $B(N_0;N,r_0)$ is the value of the Binomial distribution for $N_0$ consumers of energy profile $E_0$ with parameters $N$ and $r_0$. %and $B(N_0;N-1,p)$ is the Binomial probability distribution with parameters $N-1$ and $p$, for $N_0$ consumers of low-to-moderate energy consumption users.

The Energy Source Selection Game has at least one (mixed) Nash Equilibrium, as it is a game with finite set of players and finite strategy sets (Nash's original result). To derive the equilibria, we recall that any mixed strategy equilibrium $\mathbf{p^{NE}}=(\mathbf{p_0^{NE}}, \mathbf{p_1^{NE}}, ..., \mathbf{p_{M-1}^{NE}})^T$ must fulfill

\vspace{-5pt}
\small
\begin{equation}\label{eq:cost_equality_mixed}
\upsilon_{RES, \theta_i}(\mathbf{p^{NE}})= \upsilon_{nonRES, \theta_i}(\mathbf{p^{NE}}), ~\forall \theta_i \in \Theta.
\end{equation}
\normalsize

Namely, the expected costs of each pure strategy that belongs to the support of the equilibrium mixed strategy are equal. %By Eq. (\ref{eq:costs_symnonRES}), the expected cost of action nonRES, $ \upsilon_{nonRES, \theta_i}(p_0^{NE}, p_1^{NE})$, is insensitive to $N_0$ (or $N-N_0$), that is, the cardinality of the two sets of consumers. 
%In addition, in order to accommodate different risk attitudes, it becomes $c_{i}^{(\cdot)}(nonRES,p) = (\epsilon_{\vartheta_i}  E_{\vartheta_i})  c_{nonRES,N}$. 
%Likewise, by Definition \ref{def:energy_source_game}, the expected cost of action RES is given by $c_{i}^{(\cdot)}(RES,p) =\sum_{N_0=0}^{N}c_{i}^{N_0}(RES,p) B(N_0;N,r)$, where the cost $c_{i}^{N_0}(RES,p)$ follows equation (\ref{eq:costs_symRES}). 
The cost for the RES pure strategy, $\upsilon_{RES, \theta_i}(p^{NE})$, given by Eq. (\ref{eq:costs_symRES}), under large populations of consumers, can be approximated by

\vspace{-5pt}
\small
\begin{align}
&\upsilon_{RES, \theta_i}(\mathbf{p^{NE}})=w_{RES,\vartheta_i}(\mathbf{n}),\nonumber \\&
\mathbf{n}=(r_0 p_{RES,0}^{NE}, r_1 p_{RES,1}^{NE}, ...,  r_{M-1} p_{RES,M-1}^{NE})^T\cdot (N-1).\label{eq:gen_costs_symRES}
\end{align} \normalsize
%In the rest of the paper, we will apply the definition of $n$ of Eq. \eqref{eq:gen_costs_symRES}.


%As a result, the player $i$, with energy profile $\theta_i$, and mixed strategy $p_{\vartheta_i}=(p_{RES,\vartheta_i};p_{nonRES,\vartheta_i})$ will have an expected cost equal to
%\begin{align}
%   \upsilon_{ \theta_i}^{N_0}(p_0,p_1) = &  p_{RES,\theta_i} ~\upsilon_{RES, \theta_i}^{N_0}(p_0,p_1)  \nonumber \\&  + p_{nonRES,\theta_i} \upsilon_{nonRES, \theta_i}^{N_0}(p_0,p_1).\label{eq:costs_tot}
%\end{align}
\subsection{Risk Attitude of the Consumers}
%Various expressions of consumers' risk attitude are considered yielding different variants of the game prescribed under Definition \ref{def:energy_source_game}. 
In the game of Definition \ref{def:energy_source_game}, we take into account various risk attitudes of the consumers.  %Specifically, the risk attitude of a consumer is expressed by adjusting the reported energy demand to its level of risk. 
A \textit{risk-seeking} consumer when playing the RES strategy will gamble its total energy demand in the game; that is, it will attempt to have its entire possible energy demand served by the RES and minimize its cost. On the contrary, a \textit{risk-conservative} consumer with RES strategy gambles part of its possible total energy demand. 

The above described risk attitude is captured by adjusting the energy demand of consumer $i\in \mathcal{N}$ when served at the night zone as $\epsilon_{\vartheta_i} E_{\vartheta_i}$, where the parameter $\epsilon_{\vartheta_i}$ is the ``{risk-aversion degree}'' and $\epsilon_{\vartheta_i}\geq 1$. For example, $\epsilon_{\vartheta_i}=1$ in case of a risk-seeking consumer $i$ and $\epsilon_{\vartheta_i}>1$ in case of a risk-conservative consumer $i$. The consumer's $i$ energy demand when competing for RES remains equal to $E_{\vartheta_i}$. Note that we assume that consumers with the same energy profile $\theta_i$ will have the same risk attitude. In order to capture these risk attitudes, Eq. \eqref{eq:nonRES_cost} should take the form
\begin{small}
\begin{equation}
w_{nonRES,\vartheta_i}=\epsilon_{\vartheta_i} \cdot E_{\vartheta_i} \cdot c_{nonRES,N}.
\label{eq:nonRES_cost2}
\end{equation}
\end{small}

==> old/game_lesia.tex <==
\section{Uncoordinated energy source selection game}\label{sec:game}
%\textbf{we need to specify a time-unit of taking the decisions: if we take them only once then (i) ER cannot be known, (ii) why not centralized approach. This is studied for one time interval. Can I decide at a next time interval to move back some loads sent to night rate at a previous interval to ER - intra-day re- scheduling per interval? Nice to describe how this is done. }




%We also assume that the consumers do not increase their demand when opting for the night-zone. 
%The challenge addressed in this paper is finding a distributed and uncoordinated scheduling of the consumer loads in day and night-zones so that the consumers' average cost is minimized. Based on the prices, if the consumers' average cost is minimized, the amount of RES actually used (and not curtailed) should be maximized. %More specifically, we solve the problem of the energy source selection, between RES and night-zone nonRES, by the consumers themselves. %We first present a short discussion on a benchmark centralized solution and afterwards we will discuss the simpler to implement distributed one. 
%
%In time zones when the capacity of RES suffices to serve the entire energy demand, consumers can readily opt for using it and gain the price differential between the two resources. When, however, the demand exceeds the limited RES, an inherent competition emerges that should be factored by consumers in their decision to opt for requesting this resource or not at the particular time period. The underlying assumption is that the decision to opt for the finite RES bears the risk of experiencing the congestion penalties induced by the lack of coordination and pay for the more expensive, top-priced nonRES. Essentially, the main dilemma faced by consumers is whether to compete or not for requesting RES or settle for less favoured time zones and pay for medium-priced energy (assumed being covered by a nonRES facility).
%
%In order to analytically investigate the suffered congestion penalties due to the uncoordinated access to the limited resource, it is important to identify and model those key features and critical parameters that tune the intensity of competition. In this respect, we may consider $N$ consumers that decide between RES and nonRES. The first facility is capacity-constrained and able to serve a total energy demand of $\mathcal{ER}$ energy units (\eg kilowatt-hours, kWh) while the second one responds to every possible level of energy demand, yet heavily burdens the environment producing large amounts of pollutants. In the pricing arena, RES is offered at $c_{RES}$ cost units, whereas for nonRES different rates are used for daily and night energy consumption: moderate-priced night energy rate of $c_{nonRES,N} = \beta \cdot c_{RES}, \beta>1$, units and top-priced daily energy rate of $c_{nonRES,D}= \gamma \cdot  c_{RES}, \gamma>\beta$, units. The excess penalty cost $\delta\cdot c_{RES}$, with $\delta=\gamma-\beta>0$, captures the impact of congestion for RES.

%\textbf{Optimal coordinated RES allocation:} 

%Note that when consumers increase their demand when avoiding the competition, the optimal allocation becomes more complex since it should compare the aggregate cost for consuming nonRES at day-zone against the aggregate cost for consuming (more) nonRES at night-zone. These decisions are communicated to the consumers through the smart-grid facility. 

%
%
%Under the optimal coordinated energy source allocation scheme, %the full information processing and decision-making tasks lie with a central entity.
%micro-grid operators %, operators of energy efficient neighbourhoods and operators of building blocks that host smart metering 
%use the smart grid-related information so as to coordinate the actions of all different stakeholders involved and secure that (a) the local RES - and storage systems - are optimally used and fairly distributed among consumers and (b) no one would pay the excess congestion penalty. In essence, individual customers/consumers that range from owners/operators of large building and facilities to house customers, are expected to issue energy demand requests to a central server, which monitors RES, possesses precise information about its availability, and assigns it so that the aggregate consumers' cost is minimized. Ideally, the efficient exploitation of the smart meter attributes requires the use of a highly intelligent mechanism which takes into account the complex interplay between energy consuming devices, weather conditions, building dynamics, user preferences and comfort, grid status, availability of RES or storage systems \etc.
%
%Overall, in an micro-grid environment where the aggregate demand exceeds the RES capacity of $\mathcal{ER}$ energy units, %with RES capacity of $\mathcal{ER}$ energy units, whereby such an coordination system serves the energy requests of $N$ consumers that jointly shape an energy demand exceeding the RES capacity, 
%exactly $\mathcal{ER}$ units of demand would be directed to RES and no one would pay the excess congestion penalty cost. Advanced decentralized realizations of optimal coordination mechanisms may optimally shape the $\mathcal{ER}$ capacity, pricing and the energy demand of all different consumers within the operator's entity so as the locally available RES is exploited to the maximum while the needs from purchasing from the top-priced conventional grid are minimized.

%\textbf{Uncoordinated energy source selection:} As already mentioned, the design and implementation of a coordinated energy source selection is complex due to the required information exchange, fairness criteria to be considered, heterogeneity of the micro-grid environments (often consisting of fairly diveRES components such as electric cars, wind turbines, solar farms and all kinds of different appliances with various capabilities and requirements), \etc. 

%%%%%%%%%%%%%%%%

We consider a micro-grid with $N$ (eligible) consumers which have access to multiple sources of energy.
In the day-zone, consumers have access to (i) a limited RES capacity $\mathcal{ER}>0$ (in energy units \eg kWh) at a low-cost price $c_{RES}$ per unit of energy, and (ii) an unlimited peak-load production at a high-cost price $c_{nonRES,D}= \gamma \cdot  c_{RES}$, with $\gamma>1$. In the night-zone, consumers have access to an unlimited base-load production, with a medium-cost $c_{nonRES,N} = \beta \cdot c_{RES}$, with $\gamma>\beta>1$.
%%% assumptions
All prices, as well as the amount of the available RES $\mathcal{ER}$ are assumed known to the consumers. %urthermore, network constraints are neglected.

The allocation of the available RES $\mathcal{ER}$ to the consumers could be carried out optimally through a fully coordinated centralized approach, such as described in Section \ref{sec:coordinated}. Besides the increased communication and processing requirements, a coordinated RES allocation is a complex process that needs to take into account fairness criteria, the complex interplay between energy consuming devices, %the heterogeneity of the micro-grid environments often consisting of fairly diverse components such as electric cars, wind turbines, solar farms and all kinds of different appliances with various capabilities and requirements, weather conditions, 
user preferences/comfort, \etc, and it is not scalable. In addition, a major concern of a centralized solution is the privacy of consumers, since they should reveal their preferences/constraints to a central server. Besides, there is no guarantee that consumers will act truthfully.

Consequently, this section describes a distributed, uncoordinated energy source selection approach. Based on the known costs and available RES capacity, the consumers can choose to engage their load during the day-zone or the night-zone. Each consumer acts selfishly aiming at minimizing the cost of the acquired energy.
%%%
A micro-grid operator collects these loads and allocates the energy sources accordingly. If the aggregate amount of day-zone loads does not exceed $\mathcal{ER}$, they are all allocated RES production during the day-zone. Otherwise, certain day-zone loads are allocated the RES production, and the remaining ones are allocated the peak-load production in the day-zone. Therefore, these loads will incur an \emph{excess penalty cost} equal to $(\gamma-\beta) \cdot c_{RES}$ per unit of energy load, compared to being engaged during the night-zone.

%prices' definitions, if the consumers' average cost is minimized, the amount of RES actually used (and not curtailed) should be maximized. 


%Advanced decentralized realizations of the aforementioned optimal centralized coordination may also be considered, but this is outside the focus of this paper. We are only interested in comparing the optimal (theoretical) performance (expressed in terms of the minimum average aggregate consumer cost) delivered through centralized or decentralized coordinated energy allocation, against that under the (simpler to implement) uncoordinated approach considered in this paper. 

%
%Typically, the research in the optimization of energy grid system operation, amounts to defining and solving a system-level optimization problem based on a centralized objective function. However, under heterogeneous micro-grid networks, often consisting of different components such as electric cars, diesel generators, wind turbines, solar farms and all different appliances with various capabilities and objectives, specific objective function for each individual component should be taken into account. Indeed, considering the demand side, in the absence of central coordination, each consumer acts selfishly aiming at minimizing the cost of the acquired energy. The intuitive tendency to opt for RES combined with its scarcity, foster tragedy of commons effects and highlight the game-theoretic dynamics behind the energy source selection task.
%
 %coming up with optimal decisions for operating their associated energy consuming devices. 
%In doing so, they are assumed here to hold precise information about the RES capacity and the pricing on all energy sources involved (RES, day and nigh time grid energy). They also may or may not hold precise information about the actual demand, \ie competition. These assumptions are fairly realistic and feasible since the decision-making task can be assigned to intelligent meters that leverage the available information (through the communication network layer within the smart grid infrastructure) to perform complex computations and best respond to others' actions. Furthermore, these meters may account for user preferences and comfort in the reasoning process. To this end, we assume \textit{two} generic energy consumption profiles corresponding to low-to-moderate and high consumption level energy users.

We will compare the optimal (theoretical) performance of the minimum average aggregate consumer cost, achieved via a centralized coordinated energy allocation, against the one under the proposed distributed, uncoordinated approach.


\vspace{-2pt}
\subsection{Energy Source Selection Game}\label{sec:game_definition}



As mentioned in the introduction, the intuitive tendency to opt for RES combined with its scarcity foster the tragedy of commons effects and highlight the game-theoretic dynamics behind the energy source selection task. Thus, the distributed uncoordinated decision-making on energy source selection can be formulated in game-theoretic terms, whereby $N$ rational players/consumers compete against each other for a limited capacity $\mathcal{ER}$ of low-cost RES. In detail, the game is defined as follows.

%This distributed, uncoordinated decision-making on energy source selection can be defined via the following game: 
\begin{definition}\label{def:energy_source_game}
An \emph{Energy Source Selection Game} is a tuple
\\$\Gamma=(\mathcal{N}, \mathcal{ER}, \{\vartheta_{i}\}_{i\in \mathcal{N}}, \{A_{i}\}_{i\in\mathcal{N}},  \{w_{A_{i},\vartheta_{i}}\}_{i\in \mathcal{N}})$, where:
\begin{itemize}
\item $\mathcal{N}=\{1,...,N\}$, $N>1$ is the set of players, i.e., energy consumers.
\item $\mathcal{ER}>0$ is the limited RES capacity in energy units.
\item $\vartheta_{i} \in \Theta=\{0,1,...,M-1\}$ is the type of consumer $i$ ($i\in \mathcal{N}$) corresponding to an energy consumption profile (load) $E_{\vartheta_i}$, in energy units. We define as $0\leq r_{\vartheta_{i}}\leq 1$, the probability that a consumer has a type $\vartheta_{i} \in \Theta$. Then, we denote with $N_{\vartheta_{i}} = r_{\vartheta_{i}} N $ the total number of consumers of type $\vartheta_{i}$. It should hold that $M \leq N$ and it is assumed, without loss of generality, that $E_0<E_1<...<E_{M-1}$. %where $0$ ($1$) stands for low-to-moderate (high) energy level users with demand of $E_0$ ($E_1$, $E_1 \geq E_0$) energy units,
\item $A_{i} $ is the pure strategy of player $i$ taking values in the set of potential pure strategies $\mathcal{A}=\{RES,nonRES\}$ (same for all consumers), consisting of the choice to engage their load in the day-zone to compete for ``low-priced renewable-source energy'' ($RES$) and the choice to engage their load during the night-zone to access the ``medium-priced base-load energy source'' ($nonRES$).
%\item $s_{i}: \Theta \rightarrow A$, the strategy function for each consumer $i\in \mathcal{N}$,
\item $w_{A_i,\vartheta_i}: \mathbb{R}^M \rightarrow \mathbb{R}$ is the cost function of a player $i$ with type $\vartheta_i$ and pure strategy $A_i$. 
\end{itemize}
\end{definition}




%In addition, 

%\item a consumer has an energy demand level $E_{\ell}$ with probability $r_{\ell}$, where $\sum_{\ell\in \Theta} r_{\ell}=1$,

%\item $c_{i}^{N_0}(A_i,\vartheta_i)$ are cost functions under particular type, $\vartheta_i$, and strategy, $A_i$, that are basically determined based on $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$.
%$c_{i}^{(\cdot)}(s(\vartheta),\vartheta)= c_{i}^{(\cdot)}(s_{i}(\vartheta_{i}),s_{-i}(\vartheta_{-i}),\vartheta_{i},\vartheta_{-i})$, are the expected cost functions for each consumer $i\in \mathcal{N}$, for every type profile $\vartheta\in \times_{k=1}^{N}\Theta_{k}$ and strategy profile $s(\vartheta)\in \times_{k=1}^{N}S_{k}$, ($c_{i}^{N_0}(s(\vartheta),\vartheta)$ are cost functions under particular type, $\vartheta$, and strategy, $s(\vartheta)$, profile with $N_0=N-\sum_k \vartheta_k$), that are functions of $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$,
%\end{itemize}

Furthermore, in the game of Definition \ref{def:energy_source_game}, we take into account various risk attitudes of the consumers.
We characterize a consumer as \textit{risk-seeking} when it gambles its total demand in the game when playing the strategy $RES$; that is, it will attempt to have its entire possible energy demand served by RES and minimize its cost. On the contrary, a \textit{risk-conservative} consumer when playing the $RES$ strategy it gambles part of its total possible energy demand. Note that we assume that consumers with the same type $l \in \Theta$ will have the same risk attitude, but this is not limiting, as we can have as many consumer types as the total number of consumers.  

The above-described risk attitude is captured by adjusting the energy demand of a consumer $i\in \mathcal{N}$ only if he decides to engage its loads in the night-zone. Specifically, in the night-zone, the energy demand of consumer $i$ becomes $\epsilon_{\vartheta_i} E_{\vartheta_i}$, where the parameter $\epsilon_{\vartheta_i}\geq 1$ is the ``{risk-aversion degree}''. Then, $\epsilon_{\vartheta_i}=1$ represents a risk-seeking consumer $i$, and $\epsilon_{\vartheta_i}>1$ a risk-conservative consumer $i$. Besides, when a consumer decides to engage its loads during the day-zone, its energy demand remains equal to $E_{\vartheta_i}$. Thus, a risk conservative consumer has a total possible energy demand equal to $\epsilon_{\vartheta_i} E_{\vartheta_i}$ with $\epsilon_{\vartheta_i}>1$ and (i) when it decides the strategy $RES$, it engages part of its load equal to $E_{\vartheta_i}$  and not its maximum possible demand $\epsilon_{\vartheta_i}E_{\vartheta_i}$, (ii) when it decides $nonRES$, it engages all of its load equal to $E_{\vartheta_i}$. 
%Note that if a risk-averse consumer type $\vartheta_i$ with risk aversion degree $\epsilon_{\vartheta_i}>1$ goes for RES, it engages a load equal to $E_{\vartheta_i}$ and not its maximum possible demand $\epsilon_{\vartheta_i}E_{\vartheta_i}$.



%and similarly the corresponding number of competitors of high energy profile is $n_{1}$ ($=\sum_{j \in \mathcal{N}\setminus {i}} A_j \mathbf{1}_{(\vartheta_j=1)}$).

Next, we give the expressions of the cost functions and the aggregate demand for RESs. Let us first define $n_{l,i} = \sum_{j \in \mathcal{N}\setminus {i}} \mathbf{1}_{(A_j=RES)}\cdot \mathbf{1}_{(\vartheta_j=l)}$ as the number of consumers of type $l \in \Theta$ taking action $RES$, excluding consumer $i \in \mathcal{N}$ of type $\vartheta_i \in \Theta$. Also
% $\footnote{Note that if $\vartheta_i \neq l$, $n_{l,i} = \sum_{j \in \mathcal{N}} \mathbf{1}_{(A_j=RES)}\cdot \mathbf{1}_{(\vartheta_j=l)}$.},
let $\mathbf{n_i}=[n_{0,i}, n_{1,i},..., n_{M-1,i}]^T$ be the vector collecting $n_{l,i}$ for all consumer types $l \in \Theta$.

Then, the cost function $w_{RES,\vartheta_i}(.)$ for a consumer $i$ of type $\vartheta_i$ that chooses the pure strategy $RES$ is defined as

\begin{small}
\begin{align}
w_{RES,\vartheta_i}(\mathbf{n_i}) =
rse_{\vartheta_i}(\mathbf{n_i}) \cdot c_{RES} + (E_{\vartheta_i}-rse_{\vartheta_i}(\mathbf{n_i}) ) \cdot c_{nonRES,D},
\label{eq:RES_cost}
\end{align}
\end{small}
where $rse_{\vartheta_i}(\mathbf{n_i}) $ is the amount of RES allocated to a consumer $i$ of type $\vartheta_i$. %Note that all consumers $j \in \mathcal{N} \setminus {i}$ with $\vartheta_j=\vartheta_i$ and strategy RES are granted with the same amount of RES. Therefore, 
This cost function %is non-decreasing with the number of players competing for RES ($n_{\ell,i}$,  $\ell \in \Theta$) and 
has the same value for all players of the {same} energy profile that play RES.
%consumers who decide to compete for RES undergo the risk of incurring congestion penalties. 
In addition, $rse_{\vartheta_i}(.) $ (and therefore $w_{RES,\vartheta_i}(.)$), is determined based on the actions taken by the entire population, as well as the allocation rule that the micro-grid operator adopts to distribute RES among those who compete for it. %, on the other side. %We denote an action profile by the vector $a=(a_{i},a_{-i})\in\times_{k=1}^{N}A_{k}$, where $a_{-i}$ denotes the actions of all other consumers but player $i$ in the profile $a$. The full set of $2^N$ different action profiles maps into $(N_0+1)(N-N_0+1)$ different action \emph{meta-profiles}, where $N_0$ is the number of low-to-moderate energy consumption users. Each meta-profile $a(k_0,k_1)$, with $k_0$, $k_1$ denoting the number of competitors of low-to-moderate and high energy profile, respectively, encompasses all different action profiles that correspond to the same number of consumers of the two energy profiles competing for RES. The expected costs for these $k_0$, $k_1$ consumers and for the $N-(k_0+k_1)$ ones choosing directly the medium-priced nonRES alternative are functions of $a(k_0,k_1)$ rather than the exact action profile.

On the other hand, the cost function $w_{nonRES,\vartheta_i}(.)$ for a consumer $i$ of type $\vartheta_i$ that chooses the pure strategy $nonRES$ is oblivious to others' actions, that is, 
%\vspace{-7pt}
%\small
\begin{equation}
%w_{nonRES,\vartheta_i}=E_{\vartheta_i} \cdot c_{nonRES,N}.
%\label{eq:nonRES_cost}
w_{nonRES,\vartheta_i}=\epsilon_{\vartheta_i} \cdot E_{\vartheta_i} \cdot c_{nonRES,N}.
\label{eq:nonRES_cost2}
\end{equation}
\normalsize
%In general, the cost $c_i^{N_0}(a_i,a_{-i})$ for consumer $i$ under the action profile $a=(a_i,a_{-i})$ is
%
%%\vspace{-10pt}
%\small
%\begin{eqnarray}
%\hspace{-1pt}c_{i}^{N_0}(a_{i},a_{-i})=\left\{
%\begin{array}{l l}
%\hspace{-5pt}w_{RES,\vartheta_i}(N_{RES,0}(a), n_{1}(a)), \text{if~ $a_{i}=RES$} \nonumber\\
%\hspace{-5pt}w_{nonRES,\vartheta_i}, \text{if~ $a_{i}=nonRES$} \nonumber\\
%\end{array} \right.
%\label{equ:consumer_cost_profile}
%\end{eqnarray}
%\normalsize
%
%where $N_{RES,0}(a), n_{1}(a)$ are the numbers of competitors of low-to-moderate and high energy profile \textit{but} player $i$, respectively, under action profile $a$.
Finally, the aggregate demand for RES can be defined as:
\begin{equation} \label{eq:demand_RES}
    D_{RES} = \sum_{l \in \Theta} n_{l,i} E_l + E_{\vartheta_i}, \forall i \in \Theta
\end{equation}
In addition, we define the quantity $D^{Total}=N\sum_{\ell \in \Theta}r_{\ell}E_{\ell}$ which represents the aggregated demand for RES if all consumers play the strategx $RES$. 

\subsection{Mixed strategies}

Besides choosing one of the two pure strategies, $RES$ and $nonRES$, the consumers may also randomize their actions over them. A mixed strategy is a probability distribution over the pure actions\footnote{Note that a pure strategy is a special case of a mixed strategy.}. We mainly draw our attention on symmetric mixed strategies as being more helpful in dictating practical strategies in real systems. In particular, the \emph{mixed strategy} of all consumers of type $\vartheta_i$ corresponds to the probability distribution $\mathbf{p}_{\boldsymbol \vartheta_i}=[p_{RES,\vartheta_i}, p_{nonRES,\vartheta_i}]^T$, where $p_{RES,\vartheta_i}$ is the probability of playing the strategy $RES$ and $p_{nonRES,\vartheta_i}$ of the strategy $nonRES$. We denote with $\mathbf{p}=[\mathbf{p_0}^T;\mathbf{p_1}^T;...;\mathbf{p_{M-1}}^T]$ the vector of mixed strategies for all consumer types.

%=(p_{RES,\vartheta_i},p_{nonRES,\vartheta_i})$, where $p_{RES,\vartheta_i}$ and $p_{nonRES,\vartheta_i}$ are the probabilities of selecting the pure strategies RES and nonRES, respectively, with $p_{RES,\vartheta_i}+p_{nonRES,\vartheta_i}=1$ ($\vartheta_i \in \Theta$). %Also, let $p=(p_0^T;p_1^T)$ be the matrix with lines the symmetric mixed strategies for each energy profile, namely, $p_0=(p_{RES,0}; p_{nonRES,0})$ and $p_1=(p_{RES,1}; p_{nonRES,1})$. %associated with the two energy profiles. 
Assuming that all other consumers play the mixed strategy $\mathbf{p}$. In this case, the expected costs for a player $i$ of type $\vartheta_i$ playing the pure strategies $RES$ and $nonRES$ take the respective forms:%is a weighted sum of the cost functions $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$ and is given by
%\vspace{-15pt}
%\small
%\begin{eqnarray}\label{eq:costs_symRES}
%    c_{i}(RES,p, p_{0}, p_{1}) = \sum_{N_0=0}^{N-1}\sum_{N_{RES,0}=0}^{N_0}\sum_{n_{1}=0}^{N-1-N_0}    w_{RES,\vartheta_i}(\cdot)  && \nonumber\\
%    \cdot B(n_{1};N-1-N_0,p_{RES,1}) \cdot  B(N_{RES,0};N_0,p_{RES,0}) && \nonumber\\
%      \cdot B(N_0;N-1,p) &&
%    \vspace{-10pt}
%\end{eqnarray}
%\normalsize
%\begin{align}
%   \upsilon_{ \vartheta_i}^{N_0}(p_0,p_1) = &  p_{RES,\vartheta_i} ~\upsilon_{RES, \vartheta_i}^{N_0}(p_0,p_1)  \nonumber \\&  + p_{nonRES,\vartheta_i} \upsilon_{nonRES, \vartheta_i}^{N_0}(p_0,p_1),\label{eq:costs_tot}
%\end{align}
%\noindent where the expected costs of the pure strategies RESs, nonRES of consumer $i$ are expressed as
\begin{align}& \upsilon_{RES, \vartheta_i}(\mathbf{p})=  \sum_{N_{0}=0}^{N}~ \sum_{N_{1}=0}^{N-N_0} ... \sum_{N_{M-1}=0}^{N-\sum_{k=0}^{M-2}{N_k}}\nonumber\\  & \Bigl( \sum_{n_{0,i}=0}^{N_0-\mathbf{1}_{(\vartheta_i=0)}}~\sum_{n_{1,i}=0}^{N_1-\mathbf{1}_{(\vartheta_i=1)}}...  \sum_{n_{M-1,i}=0}^{N_{M-1}-\mathbf{1}_{(\vartheta_i=M-1)}} ~w_{RES,\vartheta_i}(n) \cdot \nonumber\\
 &B(n_{0,i};N_0-\mathbf{1}_{(\vartheta_i=0)},p_{RES,0}) \cdot \nonumber \\& B(n_{1,i};N_1-\mathbf{1}_{(\vartheta_i=1)},p_{RES,1}) \cdot... \nonumber \\& B(n_{M-1,i};N_{M-1}-\mathbf{1}_{(\vartheta_i=M-1)},p_{RES,M-1})\Bigr) \cdot... \nonumber \\&B(N_0;N,r_0)B(N_1;N,r_1)...B(N_{M-1};N,r_{M-1}),  \label{eq:costs_symRES}
\end{align}
\begin{align}
\label{eq:costs_symnonRES}
   \upsilon_{nonRES, \vartheta_i}(\mathbf{p}) = w_{nonRES,\vartheta_i},
\end{align}
\noindent where $B(n_{l,i};N_l-\mathbf{1}_{(\vartheta_i=l)},p_{RES,l}) $ is the value of the Binomial probability distribution for $n_{l,i}$ consumers (excluding consumer $i$) of type $l \in \Theta$ competing for RES, with parameters $N_l-\mathbf{1}_{(\vartheta_i=l)}$ and $p_{RES,l}$, and $B(N_l;N,r_l)$ is the value of the Binomial distribution for $N_l$ consumers of type $l \in \Theta$ with parameters $N$ and $r_0$. %and $B(N_0;N-1,p)$ is the Binomial probability distribution with parameters $N-1$ and $p$, for $N_0$ consumers of low-to-moderate energy consumption users.
%These expected values are defined based on both the strategy choice by other consumers and their energy profile.

Under large populations of prosumers, the cost for the pure strategy $RES$, $\upsilon_{RES, \vartheta_i}(\mathbf{p})$, given by Eq. (\ref{eq:costs_symRES}), can be approximated by

\begin{small}
\begin{align}
&\upsilon_{RES, \vartheta_i}(\mathbf{p})=w_{RES,\vartheta_i}(\mathbf{n_i}),\label{eq:gen_costs_symRES1} \\&
\mathbf{n_i}=(r_0 p_{RES,0}, r_1 p_{RES,1}, ...,  r_{M-1} p_{RES,M-1})^T\cdot (N-1).\label{eq:gen_costs_symRES2}
\end{align} 
\end{small}

For the rest of the paper, the considered cost functions will be Eqs. \eqref{eq:gen_costs_symRES1}-\eqref{eq:gen_costs_symRES2} for the RES strategy and Eq. \eqref{eq:costs_symnonRES} for the nonRES strategy. 






\subsection{Nash equilibrium}


\begin{theorem}
The Energy Source Selection Game has at least one (mixed) Nash Equilibrium.\label{thm:nash}
\end{theorem}
The proof of Theorem \ref{thm:nash} is based on the well-known property that a game with a finite set of players and finite set of strategies has at least one (mixed) Nash Equilibrium. To derive the equilibria, we recall that any mixed strategy equilibrium $\mathbf{p^{NE}}=(\mathbf{p_0^{NE}}, \mathbf{p_1^{NE}}, ..., \mathbf{p_{M-1}^{NE}})^T$ must fulfill

\vspace{-0.1in}
\small
\begin{equation}\label{eq:cost_equality_mixed}
\upsilon_{RES, \vartheta_i}(\mathbf{p^{NE}})= \upsilon_{nonRES, \vartheta_i}(\mathbf{p^{NE}}), ~\forall \vartheta_i \in \Theta.
\end{equation}
\normalsize
\vspace{-0.1in}

\noindent Namely, the expected costs of each pure strategy that belongs to the support of the equilibrium mixed strategy are equal.

Furthermore, at NE the amount of RES allocated to a consumer type $\vartheta_i \in \theta$ satisfies\footnote{This is derived by replacing Eqs. (\ref{eq:costs_symnonRES})-%(\ref{eq:gen_costs_symRES1}), 
(\ref{eq:gen_costs_symRES2}) to Eq. \eqref{eq:cost_equality_mixed}, using \eqref{eq:RES_cost}, \eqref{eq:nonRES_cost2}.}

\vspace{-0.1in}
\small
\begin{equation}\label{eq:conditionEQ_extra_demand}
rse^{NE}_{\vartheta_i}(\mathbf{n_{i}}) = \frac{\gamma-\epsilon_{\vartheta_i}\beta}{\gamma-1}E_{\vartheta_i},~ \forall \vartheta_i \in \Theta.
\end{equation}
\normalsize
\vspace{-0.1in}

Note that the probability that a consumer $i \in \mathcal{N}$ of type $\vartheta_i \in \Theta$ plays the strategy $RES$ (resp. $nonRES$) at NE also depends on the energy source allocation policy used by the micro-grid operator. This Nash equilibrium probability, under a specific allocation mechanism $x$, is denoted $p^{x,NE}_{RES,\vartheta_i}$ (resp. $p^{x,NE}_{nonRES,\vartheta_i}$) and the corresponding probability distribution is denoted $\mathbf{p}^{x,NE}_{\vartheta_i}=[p^{x,NE}_{RES,\vartheta_i}, p^{x,NE}_{nonRES,\vartheta_i}]^T$.

In addition, for a given allocation mechanism $x$, we express the expected aggregate demand for RES at NE as %$N\sum_{\vartheta_j \in \Theta} r_{\vartheta_j }~p^{PA,NE}_{RES,\vartheta_j}~E_{\vartheta_j}$. % with respect to the energy profile 

\vspace{-0.1in}
\begin{small}
\begin{eqnarray}
\hspace{-30pt} && D^{x,NE} (\mathbf{p^{x,NE}})= N\sum_{\ell\in \Theta} r_{\ell }~p^{x,NE}_{RES,\ell}~E_{\ell}.
\label{eq:expected_demand}
\end{eqnarray}
\end{small}
\vspace{-0.1in}

This is .

In the following section, we describe two energy source allocation policies, namely the Proportional Allocation (PA) and Equal Sharing (ES) policies. Note that, while the game described above is guaranteed to have at least one mixed-strategy NE, a mixed-strategy NE is not guaranteed to exist under a specific allocation policy. Therefore, Section \ref{sec:uncoordinated_extra_demand} focuses on examining the existence of a mixed-strategy NE under the considered allocation policies.

%By Eq. (\ref{eq:costs_symnonRES}), the expected cost of action nonRES, $ \upsilon_{nonRES, \vartheta_i}(p_0^{NE}, p_1^{NE})$, is insensitive to $N_0$ (or $N-N_0$), that is, the cardinality of the two sets of consumers. 
%In addition, in order to accommodate different risk attitudes, it becomes $c_{i}^{(\cdot)}(nonRES,p) = (\epsilon_{\vartheta_i}  E_{\vartheta_i})  c_{nonRES,N}$. 
%Likewise, by Definition \ref{def:energy_source_game}, the expected cost of action RES is given by $c_{i}^{(\cdot)}(RES,p) =\sum_{N_0=0}^{N}c_{i}^{N_0}(RES,p) B(N_0;N,r)$, where the cost $c_{i}^{N_0}(RES,p)$ follows equation (\ref{eq:costs_symRES}). 

%In the rest of the paper, we will apply the definition of $n$ of Eq. \eqref{eq:gen_costs_symRES}.


%As a result, the player $i$, with energy profile $\vartheta_i$, and mixed strategy $p_{\vartheta_i}=(p_{RES,\vartheta_i};p_{nonRES,\vartheta_i})$ will have an expected cost equal to
%\begin{align}
%   \upsilon_{ \vartheta_i}^{N_0}(p_0,p_1) = &  p_{RES,\vartheta_i} ~\upsilon_{RES, \vartheta_i}^{N_0}(p_0,p_1)  \nonumber \\&  + p_{nonRES,\vartheta_i} \upsilon_{nonRES, \vartheta_i}^{N_0}(p_0,p_1).\label{eq:costs_tot}
%\end{align}

\subsection{Energy Source Allocation Policies}\label{sec:policies}

The allocation of scarce resources to human-driven agents with distinct demands, is challenging. In this paper, we examine two types of allocations with different fairness properties, namely, the proportional allocation and the equal sharing.%The engagement of humans (behind the machines) transfuse social features and require careful consideration of the fairness properties of the resource allocation policy, as it impacts on users' satisfaction, participation, compliance pervasion, and ultimately, on system's efficiency \cite{Busqu12}.

%In multiplexing settings, the division of scarce resources motivates a number of challenges with respect to the properties that should characterize the allocation mechanism. Most commonly, the allocation mechanisms pursue an utilitarian view of the allocation (\ie aggregation of agents' utility on the allocated resources). However, practical circumstances that engage humans (and machines) transfuse social features to the allocation process and raise some concerns about the level of fairness that should vouch for. The fairness properties of an allocation mechanism have a direct impact on agents' satisfaction, participation, compliance pervasion, and ultimately, on system's efficiency \cite{Busqu12}.

\paragraph{Proportional Allocation}\label{sec:prop_alloc}

The proportional allocation allocates resources in proportion to the consumer demand. Under this policy, the amount of RES received  by a consumer of type $ \vartheta_i \in \Theta$ is given by,
% all users a level of service proportional to their actual needs. In turn, applying this allocation rule in the distribution of RES capacity, consumers that compete for RES capacity are endowed with an amount of energy that is given by 

\vspace{-0.1in}
\begin{small}
\begin{eqnarray}
rse^{PA}_{\vartheta_i}(\mathbf{n_i}) &=& \frac{E_{\vartheta_i}}{\max(\mathcal{ER} , D^{PA,NE} (\mathbf{p^{PA,NE}}))}\mathcal{ER},
\label{eq:prop_alloc_energy}
\end{eqnarray}
\end{small}
\vspace{-0.1in}

%where $n_0=n_{RES,0}$, $n_1=n_{RES,1}$ and 
\noindentwhere $ D^{PA,NE} (\mathbf{p^{PA,NE}})$ is given by \eqref{eq:expected_demand}. Eq. \eqref{eq:prop_alloc_energy} ensures that, if the available RES capacity $\mathcal{ER}$ is greater than the aggregate expected demand for RES, then each consumer $ i \in \mathcal{N}$ competing for RES receives a RES share equal to its energy demand profile $E_{\vartheta_i }$. Otherwise, it receives a share of the available capacity $\mathcal{ER}$ proportional to its energy profile. Note that in proportional allocation, the available RESs capacity is wasted only if $ D^{PA,NE} (\mathbf{p^{PA,NE}})\leq \mathcal{ER}$, otherwise, it is fully utilized. 

\paragraph{Equal Sharing}\label{sec:eq_sharing}

Under equal sharing, all consumers competing for RES in the day-zone will have access to exactly the same share value of RES capacity. Here, we call this quantity as the ``fair share" and is given by:

\begin{small}
\begin{align}
   sh(\mathbf{p^{ES,NE}}) 
=\frac{\mathcal{ER}}{ N \sum_{ \ell=0}^{M-1} r_{\ell}  p_{RES,\ell}^{ES,NE}} \label{eq:fairshare}
\end{align}
\end{small}
or equivalently,
\begin{small}
\begin{align}
   sh(\mathbf{n_i})
=\frac{\mathcal{ER}}{\sum_{\ell \in \Theta } n_{\ell ,i }+1}, \forall i \in \mathcal{N},
\end{align}
\end{small}
where the equivalence derives using Eq. \eqref{eq:gen_costs_symRES2}. However, if the energy demand of a user is smaller that the fair share, then the extra energy will remain unused. 
To express this, the amount of RES capacity granted to a consumer of type $ \vartheta_i \in \Theta$ that competes for RESs, is given by,
%benefits from accessing a particular service. In the energy front, all consumers that compete for RES capacity are endowed with an amount of energy that is given by


\begin{small}
\begin{eqnarray}
\hspace{-30pt} && rse^{ES}_{\vartheta_i}(\mathbf{n_i}) = \min\left( E_{\vartheta_i}, sh(\mathbf{n}_i)\right)
\label{eq:eq_sharing_energy}
\end{eqnarray}
\end{small}
As a result, in equal sharing part of the available RES capacity may remain unused, even if the total aggregate demand for RESs is higher than $\mathcal{ER}$ ($ D^{ES,NE} (\mathbf{p^{ES,NE}})\geq \mathcal{ER}$, ). This happens when the fair share (Eq. \eqref{eq:fairshare}) is greater than consumers demand. 

%where $n_0,n_1$ denote the number of competitors %of low-to-moderate and high energy profile \textit{but} player $i$, respectively, as also defined in Section 
%\ref{sec:prop_alloc}, and $n_0+n_1+1$ is the total number of competitors.
%where $\sum_{\ell \in \Theta } %n_{\ell , i}+1$ is the total number of consumers competing for RES,where $ n_{\ell , i}$ is explained above Eq. \eqref{eq:demand_RES}. 
%Taking the minimum ensures that, no consumer $ i \in \mathcal{N}$ receives a share of the available RESs capacity $\mathcal{ER}$ that is greater than its energy demand profile $E_{\vartheta_i}$.%, with $n_0,n_1$ as in Section \ref{sec:prop_alloc}.

Generally, policies for sharing resources that accommodate a level of fairness that prioritizes classes of users with specific characteristics may provide high efficiency (by prioritizing ``strong players'') but lack stability (``weak players'' may continuously change behavior/strategy to improve the acquired service). For instance, the proportional allocation may cause unstable operational states since it entails the risk of starvation of users with low energy demand, and eventually result in fewer satisfied players. On the other hand, equal sharing of resources favors stability since it prevents strong energy players (consumers with high demand) from obtaining more resources that any other player. Yet, equal sharing may result in inefficient and wasteful utilization of energy resources, since the ``fair share'' of energy resources may exceed the energy requirements of particular consumers of low energy demand.

%
%enabling varying notions of fairness
%derive the stable operational states under the two allocation policies in terms of the associated equilibrium strategies, assuming fully rational players, free of knowledge and computational constraints.% and emotional biases.
%


% and analyze the resulting dynamics under different allocation policies that conceptualize various levels of fairness in energy resource sharing. In all cases, we derive the stable operational conditions (\ie equilibria) and the associated costs incurred by the players, and assess their efficiency by comparing them with those under optimal coordinated energy source allocation. 



\subsection{Social Cost}\label{sec:socialcost}
The social cost at NE is computed differently for the proportional allocation and the equal sharing. 

In proportional allocation, the social cost at NE is given by:

\begin{small}
\begin{align}
C^{PA,NE}(\mathbf{p}^{PA,NE}) &=  \min(\mathcal{ER}, D^{PA,NE}(\mathbf{p^{PA,NE}})) c_{RES} \nonumber \\&+  \max(0,D^{PA,NE}(\mathbf{p^{PA,NE}})-\mathcal{ER})c_{nonRES,D} \nonumber \\
&+N \left[ \sum_{\ell \in \Theta} r_{\ell }p^{PA,NE}_{nonRES,\ell}\varepsilon_{\ell }E_{\ell}\right] c_{nonRES,N}.
 \label{eq:social_cost_pa_extra_demand}
 \end{align}
\end{small}

The first two summands refer to the consumers who played RESs.
The first summand is for the demand served by low-cost RES capacity during the day-zone. The second summand is for the demand served by high-cost peak-load production during day-zone. Finally, the third summand is for the consumers who played $nonRES$.



In the case of equal sharing, we need to account for the fact that part of the available RESs capacity may remain unused even if $ D^{ES,NE} (\mathbf{p^{ES,NE}})\geq \mathcal{ER}$. To do so, let us first define the quantity
\begin{small}$$d(\mathbf{p^{ES,NE}})= N \sum_{ \ell=0}^{M-1} r_{\ell} p_{RES,\ell}^{ES,NE}  \min(sh(\mathbf{p^{ES,NE}}), E_{\ell}),$$\end{small} which is equal to the part of the expected aggregate demand for RESs that is actually served by RESs.   
 
Then, we can define the social cost as:

\begin{small}
\begin{align}
C^{ES,NE}(\mathbf{p^{ES,NE}})& =  d(\mathbf{p^{ES,NE}}) c_{RES} \nonumber\\ &+(D^{ES,NE}(\mathbf{p^{ES,NE}}) -d(\mathbf{p^{ES,NE}}))c_{nonRES,D}\nonumber \\
&+N \left[ \sum_{\ell\in \Theta} r_{\ell}p^{ES,NE}_{nonRES,\ell}\varepsilon_{\ell }E_{\ell}\right] c_{nonRES,N}
 \label{eq:social_cost_es}
 \end{align}
\end{small}



Later, we will provide more explicit expressions for the expected aggregate demand and the social cost at NE depending on the available RES capacity, energy profiles and risk aversion parameters of all consumers.


In the following sections, we analytically and numerically study the distributed, uncoordinated energy selection game. We study the stability and efficiency of energy resource allocation by considering the two different notions of fairness above. Specifically, for each allocation policy we analytically derive its equilibrium states (stability) and we numerically compare the costs incurred by the consumers' strategies against the costs of an optimal centralized coordinated operation (efficiency).



==> old/policies.tex <==
\subsection{Renewable Energy Allocation Policies}\label{sec:policies}

The allocation of scarce resources to human-driven agents with distinct demands, is challenging. In this paper, we examine two types of allocations with different fairness properties, namely, the proportional allocation and the equal sharing.%The engagement of humans (behind the machines) transfuse social features and require careful consideration of the fairness properties of the resource allocation policy, as it impacts on users' satisfaction, participation, compliance pervasion, and ultimately, on system's efficiency \cite{Busqu12}.

%In multiplexing settings, the division of scarce resources motivates a number of challenges with respect to the properties that should characterize the allocation mechanism. Most commonly, the allocation mechanisms pursue an utilitarian view of the allocation (\ie aggregation of agents' utility on the allocated resources). However, practical circumstances that engage humans (and machines) transfuse social features to the allocation process and raise some concerns about the level of fairness that should vouch for. The fairness properties of an allocation mechanism have a direct impact on agents' satisfaction, participation, compliance pervasion, and ultimately, on system's efficiency \cite{Busqu12}.

\paragraph{Proportional Allocation}\label{sec:prop_alloc}

The proportional allocation allocates resources in proportion to the consumer demand. Under this policy, the amount of RES received by a consumer of type $\vartheta_i$ is given by,
% all users a level of service proportional to their actual needs. In turn, applying this allocation rule in the distribution of RES capacity, consumers that compete for RES capacity are endowed with an amount of energy that is given by 

\vspace{-5pt}
\footnotesize
\begin{eqnarray}
rse^{PA}_{\vartheta_i}(\mathbf{n}) &=& \frac{E_{\vartheta_i}}{\max(\mathcal{ER} ,(\sum_{\ell \in \Theta } n_{\ell  } E_{\ell  }+ E_{\vartheta_i })}\mathcal{ER},
\label{eq:prop_alloc_energy}
\end{eqnarray}
\normalsize

%where $n_0=n_{RES,0}$, $n_1=n_{RES,1}$ and 
where $\sum_{\ell \in \Theta } n_{\ell  } E_{\ell  }+ E_{\vartheta_i}$ is the total energy demand.

\paragraph{Equal Sharing}\label{sec:eq_sharing}

Under equal sharing, all competing consumers will obtain the same amount of resources (as long as they have a need for). Under this policy, the amount of RES received by a consumer of type $ \vartheta_i$ is given by,
%benefits from accessing a particular service. In the energy front, all consumers that compete for RES capacity are endowed with an amount of energy that is given by

\vspace{-5pt}
\footnotesize
\begin{eqnarray}
\hspace{-30pt} && rse^{ES}_{\vartheta_i}(\mathbf{n}) = \min\left( E_{\vartheta_i}, \frac{\mathcal{ER}}{\sum_{\ell \in \Theta } n_{\ell }+1}\right),
\label{eq:eq_sharing_energy}
\end{eqnarray}
\normalsize
%where $n_0,n_1$ denote the number of competitors %of low-to-moderate and high energy profile \textit{but} player $i$, respectively, as also defined in Section 
%\ref{sec:prop_alloc}, and $n_0+n_1+1$ is the total number of competitors.
where $\sum_{\ell \in \Theta } n_{\ell }+1$ is the total number of competitors.%, with $n_0,n_1$ as in Section \ref{sec:prop_alloc}.

Generally, policies for sharing resources that accommodate a level of fairness that prioritizes classes of users with specific characteristics may provide high efficiency (by prioritizing ``strong players'') but lack stability (``weak players'' may continuously change behavior/strategy to improve the acquired service). For instance, the proportional allocation may cause unstable operational states since it entails the risk of starvation of users with low energy demand, and eventually result in fewer satisfied players. On the other hand, equal sharing of resources favors stability since it prevents strong energy players (consumers with high demand) from obtaining more resources that any other player. Yet, equal sharing may result in inefficient and wasteful utilization of energy resources, since the ``fair share'' of energy resources may exceed the energy requirements of particular consumers of low energy demand.

In the following sections, we analytically and numerically study the distributed, uncoordinated energy selection game. We study the stability and efficiency of energy resource allocation by considering the two different notions of fairness above. Specifically, for each allocation policy we analytically derive its equilibrium states (stability) and we numerically compare the costs incurred by the consumers' strategies against the costs of an optimal centralized coordinated operation (efficiency).

%
%enabling varying notions of fairness
%derive the stable operational states under the two allocation policies in terms of the associated equilibrium strategies, assuming fully rational players, free of knowledge and computational constraints.% and emotional biases.
%


% and analyze the resulting dynamics under different allocation policies that conceptualize various levels of fairness in energy resource sharing. In all cases, we derive the stable operational conditions (\ie equilibria) and the associated costs incurred by the players, and assess their efficiency by comparing them with those under optimal coordinated energy source allocation. 


\subsection{Demand}\label{sec:demand}
The expected aggregate demand for RES at NE, denoted as $D^{x,NE}$, is given as: %$N\sum_{\vartheta_j \in \Theta} r_{\vartheta_j }~p^{PA,NE}_{RES,\vartheta_j}~E_{\vartheta_j}$. % with respect to the energy profile 
\vspace{-5pt}
\footnotesize
\begin{eqnarray}
\hspace{-30pt} && D^{x,NE} (\mathbf{p^{x,NE}})= N\sum_{\ell\in \Theta} r_{\ell }~p^{x,NE}_{RES,\ell}~E_{\ell},
\label{eq:expected_demand}
\end{eqnarray}\normalsize where $x$ is replaced by $PA$ for the proportional allocation and by $ES$ for the equal sharing, and $p^{x,NE}_{RES,\vartheta_j}$ stands for the Nash equilibrium probability of profile $\vartheta_j \in \Theta$ competing for RES for each $x$ value. 

In Section, \ref{sec:uncoordinated_extra_demand}, we will give more explicit expressions for the expected aggregate demand dependent on the case.

\subsection{Social Cost}\label{sec:socialcost}
The social cost is computed differently for the proportional allocation and the equal sharing. In proportional allocation and at NE, 

\vspace{-5pt}
\footnotesize
\begin{align}
C^{PA,NE}(\mathbf{p}^{PA,NE}) &=  \min(\mathcal{ER}, D^{PA,NE}(\mathbf{p^{PA,NE}})) c_{RES} \nonumber \\&+  \max(0,D^{PA,NE}(\mathbf{p^{PA,NE}}))-\mathcal{ER})c_{nonRES,D} \nonumber \\
&+N \left[ \sum_{\ell \in \Theta} r_{\ell }p^{PA,NE}_{nonRES,\ell}\varepsilon_{\ell }E_{\ell}\right] c_{nonRES,N}.
 \label{eq:social_cost_pa_extra_demand}
 \end{align}
\normalsize

For the equal sharing, we need to account for the extra renewable energy allocated to users, e.g., when all users (both profiles) compete for RES and possibly the lower energy profile users are allocated more RES than they need for or when the amount of RES is higher than the overall users' demand. The fair share of RES at NE, $sh(\mathbf{p^{ES,NE}})$, can be approximated by 

\vspace{-5pt}
\footnotesize
\begin{eqnarray}
sh(\mathbf{p^{ES,NE}}) \hspace{-5pt} &=& \hspace{-5pt} \frac{\mathcal{ER}}{ N \sum_{ \ell=0}^{M-1} r_{\ell}  E_{\ell} p_{RES,\ell}^{ES,NE}}.
 \label{eq:sharing_es}
 \end{eqnarray}
\normalsize

Therefore,
\vspace{-5pt}
\footnotesize
\begin{align}
&C^{ES,NE}(\mathbf{p^{ES,NE}}) \nonumber\\ &=  d(\mathbf{p^{ES,NE}}) c_{RES} +(D^{ES,NE} -d(\mathbf{p^{ES,NE}}))c_{nonRES,D}\nonumber \\
&+N \left[ \sum_{\ell\in \Theta} r_{\ell}p^{ES,NE}_{nonRES,\ell}\varepsilon_{\ell }E_{\ell}\right] c_{nonRES,N},
 \label{eq:social_cost_es}
 \end{align}
\normalsize

with \footnotesize$d(\mathbf{p^{ES,NE}})= N \sum_{ \ell=0}^{M-1} r_{\ell} p_{RES,\ell}^{ES,NE}  \min(sh(\mathbf{p^{ES,NE}}), E_{\ell})$.\normalsize


==> old/related work/v2_intro/brief/introduction.tex <==
\section{Introduction}\label{sec:intro}

One of the key features of the SG is the replacement of conventional mechanical meters with smart meters to enable efficient, flexible and reliable two-way flow of energy and information for better coordination between suppliers and customers and control of the power grids. Renewable energy sources (RES), e.g. wind turbines and solar photovoltaics, have become one of the critical parts in SG, as well as more and more users are willing to deploy the RES and energy storage devices at their homes \cite{farmad2012integration}. This paper explores an approach to utilize the maximum available of RES taking into consideration the recognized problem of carbon pollution. By 2020, it is expected that almost 72\% of European consumers will have a smart electric meter.

Demand response management (DRM) smooths out the system power demand profile across time and provides short-term reliability benefits as it can offer load relief to resolve system and/or local capacity constraints. Thus, from the operator aspect, DRM reduces the cost of operating the grid, while from the user aspect it lowers their bills. In most of the past papers that have modeled renewable energy (RE), e.g \cite{bu2011stochastic}, \cite{he2011multiple}, the key focus has been on exploring DRM in the context of multiple energy sources, incorporating RESs on the supply side and minimizing the cost of this side. Instead, \cite{maharjanuser} includes multiple renewable and non-renewable energy sources based utility companies and focuses on minimizing the cost for each user.
Recently, game theory has been applied to the Demand Response programs \cite{saad2012game}. For example, the non-cooperative game was utilized to minimize the electricity cost of consumers \cite{mohsenian2010autonomous}, where based on a common scenario, with a single utility company serving multiple customers, the global optimal performance in terms of minimizing the energy costs is achieved at the Nash equilibrium of the formulated energy consumption scheduling game

Most of the demand-side management (DSM) approaches that have been deployed over the past three decades (e.g. \cite{ruiz2009direct}), focus on the interactions between a utility company (UC) and its customers or users. In contrast, Mohsedian-Rad et al. \cite{mohsenian2010autonomous} argue that rather than focusing on how each user behaves individually, a good DSM program should have the objective that the aggregate load satisfies some desired properties. More specifically, this work presents an incentive-based energy consumption scheduling scheme, where through an appropriate pricing scheme, the Nash equilibrium of the energy consumption game among the participating users who share the same energy source is the optimal solution that minimizes the energy cost in the system.

However, in the future SGs, energy storage is expected to be a key component in smart homes and thus, it has a strong impact on DSM. In \cite{vytelingum2010agent}, Vytelingum et al. provide a general framework within which to analyze the Nash equilibrium of an electricity grid and devise new agent-based storage learning strategies that adapt to market conditions. The simulation results show that the learning scheme converges to a Nash equilibrium while reducing the peak demand which also leads to reduce costs and carbon emissions. Based on the normal electricity usage profile of all the users in the considered SG, it is then possible to compute the Nash equilibrium points, which describe when it is best for the agents to charge their batteries, use their stored electricity, or use electricity from the SG \cite{fadlullah2011survey}.

Storage devices may be used to compensate for the variability of typical renewable electricity generation including wind, wave and solar energy. With this motivation, \cite{maharjanuser} includes multiple renewable energy sources on the supply side, in addition to the traditional fossil-fuel based sources. In \cite{mohsenian2010autonomous}, \cite{ibars2010distributed}, \cite{jia2012optimal} users are price anticipating (i.e., they take into account how their consumptions will affect the prices). For example, in \cite{ibars2010distributed} is defined a non-cooperative congestion game among users, which is used to set the price levels for the demand vector of each user. On the contrary, in case where users are price taking (\cite{li2011optimal},\cite{yang2013game}), they aim to minimize their costs.

There has been a growing interest in last years in modeling ICT systems and applications where a number of selfish agents compete over a limited capacity and low-cost resource. Very recent work, \cite{hasan2012non} and \cite{shi2011competition} has been focused on addressing the competition in game-theoretic terms. With the same spirit, in \cite{holzman2003network}, the drivers choose between a number of routes from a common-to-all origin to a common-to-all destination. In a nutshell, all the works noted above, apply selection games where players choose between specific available resources. In contrast, in this paper we consider the choice between specific sources at any time period. In our uncoordinated source selection problem, consumers are viewed as strategic decision-makers that aim at maximizing their own individual welfare.






==> old/related work/v2_intro/extended/introduction.tex <==
\section{Introduction}\label{sec:intro}

Recently, the Smart Grid (SG) has been proposed as the next-generation architecture of electrical grid that modernizes the current power grids for better utilization of existing assets. One of the key features of the SG is the replacement of conventional mechanical meters with smart meters to enable efficient, flexible and reliable two-way flow of energy and information for better coordination between suppliers and customers and control of the power grids. Renewable energy sources (RES), e.g. wind turbines and solar photovoltaics, have become one of the critical parts in SG, as well as more and more users are willing to deploy the RES and energy storage devices at their homes \cite{farmad2012integration}. This paper explores an approach to utilize the maximum available of RES taking into consideration the recognized problem of carbon pollution.
Based on a report of the European Wind Energy Association, in 2013 EU member states had an installed wind generation capacity of 117,289MW. This is expected to increase to meet the EU Commission's sustainability target, which is that 27\% of generation must come from renewable sources by 2030. Germany is leading the world in the development and implementation of photovoltaic solar power. Japan has similarly moved to the forefront of distribution automation through its use of advanced battery-storage technology. Totally, EU member states have committed to rolling out close to 200 million smart electric meters. By 2020, it is expected that almost 72\% of European consumers will have a smart electric meter. These smart meters can be used not only to provide more accurate billing for customers but can also be leveraged by distribution network operators for improved outage management processes, power quality and demand response programs, each of which will allow for increased network reliability.

Demand Response (DR) is the response system of the end-users to manage their consumption of electricity in response to supply conditions. Demand response management (DRM) smooths out the system power demand profile across time and provides short-term reliability benefits as it can offer load relief to resolve system and/or local capacity constraints. Thus, from the operator aspect, DRM reduces the cost of operating the grid, while from the user aspect it lowers their bills. In most of the past papers that have modeled renewable energy (RE), e.g \cite{bu2011stochastic}, \cite{he2011multiple}, the key focus has been on exploring DRM in the context of multiple energy sources, incorporating RESs on the supply side and minimizing the cost of this side. Instead, \cite{maharjanuser} includes multiple renewable and non-renewable energy sources based utility companies and focuses on minimizing the cost for each user.
Recently, game theory has been applied to the DR programs \cite{saad2012game}. For example, the non-cooperative game was utilized to minimize the electricity cost of consumers \cite{mohsenian2010autonomous} and the congestion game was applied to control the electricity consumption by dynamic pricing \cite{ibars2010distributed}. The research work in \cite{mohsenian2010autonomous} formulates an energy consumption scheduling game, where the players are the users and their strategies are the daily schedules of their household appliances and loads. Based on a common scenario, with a single utility company serving multiple customers, the global optimal performance in terms of minimizing the energy costs is achieved at the Nash equilibrium of the formulated energy consumption scheduling game.

Most of the demand-side management (DSM) approaches that have been deployed over the past three decades (e.g. \cite{ruiz2009direct}), focus on the interactions between a utility company (UC) and its customers or users (via Real-Time Pricing, Direct Load Control, etc.), that reveal users' privacy problems when it comes to residential load control and home automation. In contrast, Mohsedian-Rad et al. \cite{mohsenian2010autonomous} argue that rather than focusing on how each user behaves individually, a good DSM program should have the objective that the aggregate load satisfies some desired properties. More specifically, this work presents an incentive-based energy consumption scheduling scheme, where through an appropriate pricing scheme, the Nash equilibrium of the energy consumption game among the participating users who share the same energy source is the optimal solution that minimizes the energy cost in the system. The experimental results reveal that this approach is able to reduce the peak-to-average ratio of the total energy demand, the total energy costs, and also each user's individual daily electricity bills.
The previous work was focused on how the users can schedule their appliances so as to minimize their billing charges. The underlying assumption was that the users are acquiring energy so as to immediately use it for their appliances.

However, in the future SGs, energy storage is expected to be a key component in smart homes and thus, it has a strong impact on DSM. In \cite{vytelingum2010agent}, Vytelingum et al. provide a general framework within which to analyze the Nash equilibrium of an electricity grid and devise new agent-based storage learning strategies that adapt to market conditions. The simulation results show that the learning scheme converges to a Nash equilibrium while reducing the peak demand which also leads to reduce costs and carbon emissions. Based on the normal electricity usage profile of all the users in the considered SG, it is then possible to compute the Nash equilibrium points, which describe when it is best for the agents to charge their batteries, use their stored electricity, or use electricity from the SG \cite{fadlullah2011survey}.

Storage devices may be used to compensate for the variability of typical renewable electricity generation including wind, wave and solar energy. With this motivation, \cite{maharjanuser} includes multiple renewable energy sources on the supply side, in addition to the traditional fossil-fuel based sources. Specifically, the users schedule their demands by optimally choosing the UCs and by optimally scheduling their shiftable appliances in order to minimize their payments to the providers. They formulate the problem as a game, incorporating the uncertainty associated with the power supply of the renewable sources, and prove that there exists a Nash equilibrium for the game.

In \cite{mohsenian2010autonomous}, \cite{ibars2010distributed}, \cite{jia2012optimal} users are price anticipating (i.e., they take into account how their consumptions will affect the prices). For example, in \cite{ibars2010distributed} is defined a non-cooperative congestion game among users, which is used to set the price levels for the demand vector of each user. The work demonstrates that the game formulated as such converges to a stable equilibrium point in a distributed manner. Furthermore, the work not only finds the local optimum points of the Nash equilibria but also shows that it is possible to arrive at a global solution to the network problem by using the equivalence between the congestion and potential games. On the contrary, in case where users are price taking (\cite{li2011optimal},\cite{yang2013game}), they aim to minimize their costs.

There has been a growing interest in last years in modeling ICT systems and applications where a number of selfish agents compete over a limited capacity and low-cost resource. Very recent work, \cite{hasan2012non} and \cite{shi2011competition} has been focused on addressing the competition in game-theoretic terms. With the same spirit, in \cite{holzman2003network}, the drivers choose between a number of routes from a common-to-all origin to a common-to-all destination. Likewise, in an instance of the access-point association problem, a number of mobiles compete over a finite number of access points where high access delays occur when many users associate with the same wireless access point \cite{hasan2012non}. In a nutshell, all the works noted above, apply selection games where players choose between specific available resources. In contrast, in this paper we consider the choice between specific sources at any time period. In our uncoordinated source selection problem, consumers are viewed as strategic decision-makers that aim at maximizing their own individual welfare.






==> old/related.tex <==





==> old/uncoordinated.tex <==
%\section{Uncoordinated energy source selection under risk-seeking consumers}\label{sec:uncoordinated_no_extra_demand}
%%
%We investigate the operational states of the uncoordinated distributed energy source selection when the consumers are risk-seeking, i.e., $\epsilon_{\vartheta_i}=1, \forall i$. %determine their actions with respect to their energy consumption profile and the associated energy demand level, as reported in Definition \ref{def:energy_source_game}. 
%%
%%\subsection{Mixed-action equilibrium strategies}\label{sec:equilibria_no_extra_demand}
%%For the Energy Source Selection Game, the strategy profile $s'\in\times_{k=1}^{N}S_{k}$ is a Bayesian Nash equilibrium if for all $i\in\mathcal{N}$:
%%\small
%%\begin{equation}\label{equ:exp_cost1}
%%s_{i}(\vartheta_{i})\in \arg \min_{s'_{i}\in S_{i}}
%%(c_{i}^{(\cdot)}(s_{i}',s_{-i}(\vartheta_{-i}),\vartheta_{i},\vartheta_{-i}))\nonumber \text{ ~~~~~or, }
%%\end{equation}
%%\normalsize
%%\small
%%\begin{equation}\label{equ:exp_cost2}
%%s_{i}(\vartheta_{i})\in \arg \min_{s'_{i}\in S_{i}}\sum_{\vartheta_{-i}}f_{\Theta}(\vartheta_{-i}/\vartheta_{i})c_{i}^{(N-\sum_{k}\vartheta_{k})}(s_{i}',s_{-i}(\vartheta_{-i}),\vartheta_{i},\vartheta_{-i})
%%\nonumber
%%\end{equation}
%%\normalsize
%%where $f_{\Theta}(\vartheta_{-i}/\vartheta_{i})$ is the posterior conditional probability of the low-to-moderate energy consumers \emph{given} the energy profile of user $i$, as derived from the application of the Bayesian rule. Therefore, $s'$ minimizes the expected cost over all possible combinations of the other consumers' types and strategies so that no player can further lower its expected cost by unilaterally changing his strategy.
%%
%%\textbf{Existence:} Game with finite set of players and finite strategy sets has at least
%%one (mixed) Nash Equilibrium \cite{Nash51}.
%%
%%\textbf{Derivation:} Any mixed-action equilibrium $p^{NE}$ must fulfil
%%\vspace{-5pt}
%%\small
%%\begin{equation}\label{eq:cost_equality_mixed}
%%c_{i}^{(\cdot)}(RES,p)=c_{i}^{(\cdot)}(nonRES,p)
%%\end{equation}
%%\normalsize
%%
%%Namely, the expected costs of each pure action belonging to the support of the equilibrium mixed-action strategy are equal. By equation (\ref{eq:costs_symnonRES}), the expected cost of action nonRES is given by
%%$c_{i}^{(\cdot)}(nonRES,p) = E_{\vartheta_i} \cdot c_{nonRES,N}$, irrespective of $N_0$ (or $N-N_0$), that is, the cardinality of the two sets of consumers. Likewise, by Definition \ref{def:energy_source_game}, the expected cost of action RES is given by $c_{i}^{(\cdot)}(RES,p) =\sum_{N_0=0}^{N}c_{i}^{N_0}(RES,p) B(N_0;N,r)$, where the cost $c_{i}^{N_0}(RES,p)$ follows equation (\ref{eq:costs_symRES}). Under high populations of energy nodes, the expected cost of action RES can be approximated by
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}\label{eq:gen_costs_symnonRES}
%%c_{i}^{(\cdot)}(RES,p)=w_{RES,\vartheta_i}(r(N-1)p_{RES,0}, (1-r)(N-1)p_{RES,1})
%%\end{equation}
%%\normalsize
%%
%By replacing  Eqs. (\ref{eq:costs_symnonRES}), (\ref{eq:gen_costs_symRES}) to Eq. \eqref{eq:cost_equality_mixed} and after a few algebraic manipulations, we obtain that in the mixed strategies equilibrium $p^{NE}$ it holds that
%
%\vspace{-5pt}
%\small
%\begin{equation}\label{eq:conditionEQ}
%rse^{NE}_{\vartheta_i}(n) = \frac{\gamma-\beta}{\gamma-1}E_{\vartheta_i}.
%\end{equation}
%
%\normalsize
%
%
%\subsection{Proportional Allocation}\label{sec:prop_alloc_eq}
%
%In the first three cases, we assume that the users' aggregate demand exceeds the RES capacity.
%
%\textbf{Case $1$.} If $E_{i}=E \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}$, $\forall i \in \mathcal{N}$, there exists a mixed strategy equilibrium for all consumer profiles. The competing strategies are in equilibrium when it holds that  $rse^{PA}_{\vartheta_i}(\cdot)=rse^{NE}_{\vartheta_i}(\cdot)$, $\forall i\in \mathcal{N}$. By replacing to the latter relation the right-hand sides of Eqs. (\ref{eq:prop_alloc_energy}) and (\ref{eq:conditionEQ}), we obtain, 
%\begin{align}
%\sum_{\vartheta_j \in \Theta } n_{\vartheta_j }E_{\vartheta_j} +E_{\vartheta_i}=\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}.
%    \label{eq:forranges}
%\end{align}
%The last equality should be true for all user profiles. Therefore, a mixed strategies equilibrium is possible if all distinct groups of consumers demand the same amount of energy, that is $E_{\vartheta_i}=E \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}$, $\forall i \in \mathcal{N}$. The competing probabilities, $p^{PA,NE}_{RES,\vartheta_i}$ that lead to mixed strategies equilibrium range in
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%\Biggl[ max\left(0,\left[\frac{\mathcal{ER} }{E}\frac{(\gamma-1)}{(\gamma-\beta)}-1-\sum_{\vartheta_j \neq \vartheta_i } r_{\vartheta_j } (N-1)\right]\frac{1}{r_{\vartheta_i}(N-1)}\right),
%   \notag\\
%     min\left(1,\left[\frac{\mathcal{ER} }{E}\frac{(\gamma-1)}{(\gamma-\beta)}-1\right]\frac{1}{r_{\vartheta_i} (N-1)}\right)
%    \Biggr],
%    \label{eq:prop_alloc_eq_bounds_0}
%\end{align}
%\normalsize
%%\vspace{-5pt}
%%\footnotesize
%%\begin{align}
%%  p^{PA,NE}_{RES,1}
%%  \in \Biggl[ max\left(0,\left[\frac{\mathcal{ER} }{E}\frac{(\gamma-1)}{(\gamma-\beta)}-1-r(N-1)\right]\frac{1}{(1-r)(N-1)}\right),
%%   \notag\\
%%     min\left(1,\left[\frac{\mathcal{ER} }{E}\frac{(\gamma-1)}{(\gamma-\beta)}-1\right]\frac{1}{(1-r)(N-1)}\right)
%%    \Biggr].
%%    \label{eq:prop_alloc_eq_bounds_1}
%%\end{align}
%%\normalsize
%The latter ranges derive via Eq. \eqref{eq:forranges} by replacing $E_{\vartheta_i}=E$, $n_{\vartheta_i}=p^{PA,NE}_{RES,\vartheta_i}r_{\vartheta_i}(N-1)$, $\forall \vartheta_i \in \Theta$, and then taking the extreme values of probabilities (i.e., $0,1$) to compute the range for the considered one. Note that the probabilities $p^{PA,NE}_{RES,\vartheta_i}$, $\forall \vartheta_i \in \Theta$, should be chosen in the above ranges but so that they satisfy $\frac{\mathcal{ER}}{E}\frac{(\gamma-1)}{(\gamma-\beta)}-1=\sum_{ \vartheta_j \in \Theta}r_{\vartheta_j} (N-1) p^{PA,NE}_{RES,\vartheta_j} $. In Section \ref{}, we provide an algorithm that leads to ....
%
%
%\textbf{Case $2$.} If $E_{\vartheta_i}  > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}$, the dominant strategy for all consumers is to defer from competing for $RES$, namely $\upsilon_{RES, \vartheta_i}(p)>\upsilon_{nonRES, \vartheta_i}(p)$, $\forall p$ and $\forall i\in \mathcal{N}$. To show this, assume that $\vartheta_i=0$ and the allocated energy is $E'$. Then, in a large population regime $\upsilon_{RES, \theta_i}(p)= E'  c_{RES}+(E_0-E') \gamma  c_{RES}$ and 
%$\upsilon_{nonRES, \theta_i}(p)=E_0 \beta c_{RES}$. The inequality $\upsilon_{RES, \theta_i}(p)>\upsilon_{nonRES, \theta_i}(p)$ is then equivalent to the inequality $E_0 >E' \frac{(\gamma-1)}{(\gamma-\beta)}$ which is true by assumption and by the fact that the allocated energy $E'$ will be less than the available energy $\mathcal{ER}$. The same can be shown for all $\vartheta_i \in \Theta$. Therefore, in this case $p^{PA,NE}_{RES, \vartheta_i}=0$, for all $\vartheta_i \in \Theta$.
%
%
%\textbf{Case $3$.} In the asymmetric case where $E_{M-1}> ..>E_K > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)} \geq E_{K-1}>..>E_0$, %the resulting interaction of consumers can be approached as a dominance-solvable game. Namely, it is assumed that rationality (as conceptualized by performing the best-response action) among players is common knowledge, that is, each player knows that the rest of the players are rational, and each player knows that the rest of the players know that he knows that the rest of the players are rational, and so on ad infinitum. In particular, 
%it is dominant strategy for all consumers $i$ ($i \in \mathcal{N}$) of higher energy profiles, i.e., $\vartheta_i\geq K$, not to compete for $RES$ (shown as in Case $2$ by comparing the costs of each pure strategy). Therefore, $p^{PA,NE}_{RES,\vartheta_i}=0$ for all $i \in \mathcal{N}$ with $\vartheta_i\geq K$. For consumers of lower energy profiles, there exists a mixed strategy equilibrium obtained as in Case $1$, under the same conditions.  Specifically, a mixed strategies equilibrium is possible if for all $\vartheta_i\leq K-1$, it holds that $E_{\vartheta_i}=E \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}$. For those user profiles, the competing probabilities, $p^{PA,NE}_{RES,\vartheta_i}$ that lead to mixed strategies equilibrium range in
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%   \Biggl[ max\left(0,\left[\frac{\mathcal{ER} }{E}\frac{(\gamma-1)}{(\gamma-\beta)}-1-\sum_{\vartheta_j \neq \vartheta_i, \vartheta_j<K } r_{\vartheta_j } (N-1)\right]\frac{1}{r_{\vartheta_i} (N-1)}\right),
%   \notag\\
%     min\left(1,\left[\frac{\mathcal{ER} }{E}\frac{(\gamma-1)}{(\gamma-\beta)}-1\right]\frac{1}{r_{\vartheta_i} (N-1)}\right)
%    \Biggr],
%    \label{eq:prop_alloc_eq_bounds_new}
%\end{align}
%\normalsize%by equalizing the right-hand sides of Eqs. (\ref{eq:prop_alloc_energy}) and (\ref{eq:conditionEQ}) and replacing $n_0=p^{PA,NE}_{RES,0}(1-r)(N-1)$. Indeed, this leads to the equation $p^{PA,NE}_{RES,0} r(N-1)E_0 +E_0= \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}$ from where 
%
%\textbf{Case $4$.} Finally, when the RES capacity exceeds the total demand it is trivial to show that the dominant strategy is competing for $RES$. Therefore, $p^{PA,NE}_{RES,\vartheta_i}=1$, $\forall \vartheta_i \in \Theta$.
%
%\textbf{Demand:} In Case $1$, the resulting expected aggregate demand for renewable energy is $N  \sum_{\vartheta_j \in \Theta} r_{\vartheta_j }p^{PA,NE}_{RES,\vartheta_j}E_{\vartheta_j}$ where the mixed strategy equilibrium probabilities $p^{PA,NE}_{RES,\vartheta_j}$, for all $\vartheta_j \in \Theta$ lie in the intervals (\ref{eq:prop_alloc_eq_bounds_0}). In Case $2$ the demand for renewable energy is zero. In Case $3$, the expected aggregate demand is defined similarly to Case $1$ and in Case $4$, it is $N  \sum_{\vartheta_j \in \Theta} r_{\vartheta_j }E_{\vartheta_j}$. Thus, is all cases the expected aggregate demand can be summarized as:
%
%%\vspace{-5pt}
%%\footnotesize
%%\begin{align}
%%  D^{PA,NE}(p^{PA,NE}) =  N  \left[ r  p^{PA,NE}_{RES,0}E_0+(1-r)  p^{PA,NE}_{RES,1}E_1\right] \notag \\
%%= min\left(N[rE_0+(1-r)E_1],\frac{N}{(N-1)}  \left[ \frac{\mathcal{ER}(\gamma-1)}{(\gamma-\beta)}-E_0 \right]\right)
%%\label{eq:demand_pa_ne_no_extra_demand}
%%\end{align}
%%\normalsize
%
%%\footnotesize
%\begin{scriptsize}
%\begin{eqnarray}
%D^{PA,NE} =  \nonumber \\ \left\{\hspace{-5pt}
%\begin{array}{l l}
%min\left(\sum_{ \vartheta_j=0}^{K-1} r_{\vartheta_j} N E_{\vartheta_j},max\left(0,\frac{N}{(N-1)}  \left[ \frac{\mathcal{ER}(\gamma-1)}{(\gamma-\beta)}-E_0 \right]\right)\right), \nonumber \\ \text{~if~ $E_{M-1}> ..>E_K > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)} \geq E_{k-1}>..>E_0$} \\
%min\left(\sum_{ \vartheta_j=0}^{M-1} r_{\vartheta_j} N E_{\vartheta_j},max\left(0,\frac{N}{(N-1)}  \left[ \frac{\mathcal{ER}(\gamma-1)}{(\gamma-\beta)}-E_0 \right]\right)\right), \text{o/w}.  \nonumber \\
%\end{array} \right.\\\hspace{-200pt}
%\label{eq:demand_pa_ne_no_extra_demand}
%\end{eqnarray}
%\end{scriptsize}
%\normalsize
%
%%Otherwise, in the symmetric case with $E_1 \geq E_0 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}$ the demand is zero while under the asymmetry $E_1 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)} \geq E_0$, the demand amounts to $rNE_0$. 
%
%Notice that the impact of the lack of coordination arises when the competing probabilities, $p^{PA,NE}_{RES,\vartheta_i}$, $\vartheta_i \in \Theta$ generate $D^{PA}$ exceeding the available renewable energy capacity $\mathcal{ER}$ (case $1$) or the consumers are overconservative in (and refrain more than they should) competing for $RES$. In the next sections, we quantify this inefficiency of equilibria by using the Price of Anarchy metric.
%
%\textbf{Social Cost:} The expected aggregate cost incurred by the entire population (\ie social cost) is given by
%
%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%C^{PA,NE} \hspace{-5pt} &=& \hspace{-5pt} min(\mathcal{ER}, D^{PA,NE}) c_{RES} +  max(0,D^{PA,NE}-\mathcal{ER})\cdot  \nonumber \\ c_{nonRES,D} 
% \hspace{-5pt}   &+& \hspace{-5pt} \left[ \left( \sum_{ \vartheta_j=0}^{M-1} r_{\vartheta_j} N E_{\vartheta_j}\right)-D^{PA,NE} \right] c_{nonRES,N}.
% \label{eq:social_cost_pa}
% \end{eqnarray}
%\normalsize
%
%
%\subsection{Equal Sharing}\label{sec:eq_sharing_eq}
%
%In this case, no player has the incentive to change his decision unilaterally, if the amount of RES allocated satisfies $rse^{ES}_{\vartheta_i}(\cdot)=rse^{NE}_{\vartheta_i}(\cdot)$, $\forall i\in \mathcal{N}$. Replacing in this equality the right-hand sides of Eqs. (\ref{eq:eq_sharing_energy}) and (\ref{eq:conditionEQ}), we obtain that the equilibrium states are possible when $E_{\vartheta_j}=E$, $\forall \vartheta_j \in \Theta$. Therefore, the probabilities, $p^{ES,NE}_{RES,\vartheta_j}$, $\forall \vartheta_j \in \Theta$, which lead to equilibrium states lie in the intervals (\ref{eq:prop_alloc_eq_bounds_0}), respectively, similarly to the proportional allocation. Also, for all other cases with respect to the values of $E_{\vartheta_j}$, $\forall \vartheta_j \in \Theta$ the mixed strategies that are dominant or equilibria coincide with the corresponding ones of Section \ref{sec:prop_alloc_eq}.
%
%%The expected aggregate demand for renewable energy $D^{ES,NE}$ is equal to $D^{PA,NE}$ (Eq. (\ref{eq:demand_pa_ne_no_extra_demand})). Finally, the social cost under equal sharing is derived in a similar fashion as Eq. (\ref{eq:social_cost_pa}). However, to do so, we need to account for the extra allocated renewable energy to users due to equal sharing, e.g., when all users (both profiles) compete for $RES$ and possibly the lower energy profile users are allocated more RES than their requested one or when the amount of RES is higher than the overall users' demand. The fair share of RES, $sh(p^{ES,NE})$, and the expected aggregate social cost, $C^{ES,NE}(p^{ES,NE})$, can be approximated by 
%%
%%\vspace{-5pt}
%%\footnotesize
%%\begin{eqnarray}
%%sh(p^{ES,NE}) \hspace{-5pt} &=& \hspace{-5pt} \frac{\mathcal{ER}}{ \sum_{ \vartheta_j=0}^{M-1} r_{\vartheta_j} N E_{\vartheta_j} p_{RES,\vartheta_j}^{ES,NE}},
%% \label{eq:sharing_es}
%% \end{eqnarray}
%%\normalsize
%%
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%&C^{ES,NE}(p^{ES,NE}) \nonumber\\ &=  d(p^{ES,NE}) c_{RES} +(D^{ES,NE} -d(p^{ES,NE}))c_{nonRES,D}\nonumber \\
%&+ \hspace{-5pt} \left[ \left[  \sum_{ \vartheta_j=0}^{M-1} r_{\vartheta_j} N E_{\vartheta_j}\right]-D^{ES,NE} \right] c_{nonRES,N},
% \label{eq:social_cost_es}
% \end{align}
%\normalsize
%
%with \footnotesize$d(p^{ES,NE})= \sum_{ \vartheta_j=0}^{M-1} r_{\vartheta_j} p_{RES,\vartheta_j}^{ES,NE} N min(sh(p^{ES,NE}), E_{\vartheta_j})$.\normalsize
%
%%\subsection{Social Cost}\label{sec:social_cost_no_extra_demand}
%%
%%The expected aggregate cost incurred by the entire population (\ie social cost) under mixed-action strategies is a function of competing probabilities and is given by
%%
%%\vspace{-5pt}
%%\footnotesize
%%\begin{eqnarray}
%%C(p) \hspace{-5pt} &=& \hspace{-5pt} min(\mathcal{ER}, D^{(\cdot)}(p)) c_{RES} +  max(0,D^{(\cdot)}(p)-\mathcal{ER})c_{nonRES,D} \nonumber \\
%% \hspace{-5pt}   &+& \hspace{-5pt} \left[ \left[ rNE_0 + (1-r)NE_1\right]-D^{(\cdot)}(p) \right] c_{nonRES,N}
%% \label{eq:social_cost_pa_es}
%% \end{eqnarray}
%%\normalsize
%%
%%Notice that the use of equation (\ref{eq:social_cost_pa_es}) to derive the social cost under equal sharing, implies an advanced implementation that provides the amount of renewable energy that possibly remains unused to increase the share of competitors with excess energy requirements. This is the case of equilibrium states where all consumers of low-to-moderate energy profile are motivated to compete while the renewable energy capacity exceeds their total demand. 
%%
%
%
%%or equivalently, with $x=max(\mathcal{ER} ,(r N  p_{nonRES,0}E_0+(1-r) N p_{nonRES,1}E_1))$
%%
%%\vspace{-5pt}
%%\footnotesize
%%\begin{align}
%% C(p) =
%%   r\cdot N \Bigl[ p_{nonRES,0} \Bigl[ \mathcal{ER} \cdot E_0/x \cdot c_{RES} +  \notag\\
%%  (E_0-\mathcal{ER} \cdot E_0/x)\cdot c_{nonRES,D} \Bigr] +  (1-p_{nonRES,0})E_0 \cdot c_{nonRES,N} \Bigr] + \notag\\
%%   (1-r)\cdot N \cdot \Bigl[  p_{nonRES,1} \Bigl[ \mathcal{ER} \cdot E_1/x \cdot c_{RES} + \notag\\
%%   (E_1-\mathcal{ER} \cdot E_1/x)\cdot c_{nonRES,D} \Bigr] +  (1-p_{nonRES,1})E_1 \cdot c_{nonRES,N}  \Bigr]
%%\label{eq:social_cost_pa_es}
%%\end{align}
%%\normalsize
%
%%%%%%%%%%%%%%%%%%%&& (1-r)\cdot N \cdot \left[p_{nonRES,1} \left[ x_1 \cdot c_{RES} +  (E_1-x_1)\cdot c_{nonRES,D} \right] + (1-p_{nonRES,1})E_1 \cdot c_{nonRES,N}  \right]
%
%
%
%

\section{Study of uncoordinated energy source selection}% under risk-conservative consumers}
\label{sec:uncoordinated_extra_demand}

In this section, we investigate the operational states of the distributed, uncoordinated energy source selection for both risk-conservative and risk-seeking consumers. Specifically, we study the conditions on the parameter values for the existence of dominant strategies or mixed-strategy NE under PA. To derive the NE, we recall that any mixed strategy NE $\mathbf{p^{NE}}$
%=(\mathbf{p_0^{NE}}, \mathbf{p_1^{NE}}, ..., \mathbf{p_{M-1}^{NE}})^T$, with $\mathbf{p}^{NE}_{\ell}=[p^{NE}_{RES,\ell}, p^{NE}_{nonRES,\ell}]^T$,
must fulfill

\vspace{-0.08in}
\small
\begin{equation}\label{eq:cost_equality_mixed}
\upsilon_{RES, \ell}(\mathbf{p^{NE}})= \upsilon_{nonRES, \ell}(\mathbf{p^{NE}}), ~\forall \ell \in \Theta.
\end{equation}
\normalsize
Namely, the expected costs of each pure strategy in the support of the mixed-strategy equilibrium  ($\mathcal{A}$) are equal. By substituting the expressions of \eqref{eq:RES_cost} and \eqref{eq:nonRES_cost2} in \eqref{eq:cost_equality_mixed}, we obtain that the amount of RESs allocated to $\ell \in \Theta$ at a NE should satisfy

\vspace{-0.08in}
\small
\begin{equation}\label{eq:conditionEQ_extra_demand}
rse^{PA, NE}_{\ell}(\mathbf{p^{NE}}) = \frac{\gamma-\epsilon_{\ell}\beta}{\gamma-1}E_{\ell},~ \forall \ell \in \Theta.
\end{equation}
\normalsize
%\subsection{Close-form expression of NE}
Thus, when combining the Energy Source Selection Game with the PA policy, the existence of a NE is under the condition

\vspace{-0.08in}
\small
\begin{equation}\label{eq:condition_PA_NE}
rse_{\ell}^{PA}(\mathbf{p}^{NE}) =rse_{\ell}^{PA,NE}(\mathbf{p}^{NE}), \forall \ell \in \Theta. \end{equation}
\normalsize
Therefore, for all cases, any existing mixed-strategy NE competing probabilities, $\mathbf{p}^{NE}$, are obtained so as to satisfy the relation \eqref{eq:condition_PA_NE}. In the following we distinguish several cases based on the parameters values, namely the RES capacity, the risk aversion degrees, and the day-time energy demand levels.

\subsubsection{\textbf{Case $1$}} \emph{The RES capacity, $\mathcal{ER}$, exceeds the maximum total demand for RES $D^{Total}$ ($\mathcal{ER} \geq D^{Total}$).}

As the consumers have knowledge of $\mathcal{ER}$ and $D^{Total}$, it is straightforward to show that the dominant-strategy for all consumers is to select the strategy $RES$. As result, the competing probabilities that lead to equilibrium states are equal to $1$ for all consumers' types, and the expected aggregate demand for RES at NE is equal to $D^{Total}$.

In all the remaining cases, we assume that $\mathcal{ER}< D^{Total}$. Three distinct cases are defined with respect to the risk aversion degrees of the consumers and energy prices.

\subsubsection{\textbf{Case $2$}} \emph{The risk aversion degrees of all consumers satisfy $1\leq \epsilon_{\vartheta_i}<\gamma/\beta$, $\forall i\in \mathcal{N}$.}

Note that Case $2$ includes both risk-seeking and risk-averse consumers.
We distinguish the following Sub-cases with respect to the energy demand profiles $E_{\vartheta_i }$ of the consumers. 
\vspace{5pt}

\textbf{Sub-case $2(a)$:} 
\emph{The energy demand profiles of all consumers satisfy  $E_{\vartheta_i } \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i }\beta)}$,  for all $\vartheta_i \in \Theta$.} %or $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$  for all $\vartheta_i \in \Theta$.}


A mixed strategy equilibrium with the PA policy exists if and only if for every $E_{\vartheta_i}$, $E_{\vartheta_j}$, $\vartheta_i, \in \Theta$ and $ \vartheta_j \in \Theta \setminus \{\vartheta_i\}$, it holds that
\small
\begin{eqnarray}\label{eq:relation_E_0_E_1_pa_ne_extra_demand}
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i }\beta)}-E_{\vartheta_i} &=& \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j }\beta)}-E_{\vartheta_j}.
 \end{eqnarray}
\normalsize
This condition is derived by equalizing the right-hand sides of Eqs. \eqref{eq:prop_alloc_energy} and \eqref{eq:conditionEQ_extra_demand} for $\vartheta_i \in \Theta$ and $\vartheta_j \in \Theta \setminus \{\vartheta_i\}$, and obtaining:
\begin{small}
\begin{align}
&  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}= \sum_{ {\vartheta_l}\in \Theta} r_{\vartheta_l} (N-1)E_{\vartheta_l} p^{PA,NE}_{RES,\vartheta_l}
    \label{eq:probrelation1}\\
  &  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}=  \sum_{ {\vartheta_l}\in \Theta} r_{\vartheta_l} (N-1)E_{\vartheta_l} p^{PA,NE}_{RES,\vartheta_l}
    \label{eq:probrelation2}  
\end{align}
\end{small}
where the right hand sides of Eqs. \eqref{eq:probrelation1}-\eqref{eq:probrelation2} are equal.

Under condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}, the competing probabilities $p^{PA,NE}_{RES,{\vartheta_i }}$ that lead to equilibrium states lie in the range
\footnotesize
\begin{align}
&  \Biggl[ \max \left\{0,\left(\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{ {\vartheta_l}\in \Theta \setminus \{{\vartheta_i}\}} r_{\vartheta_l} (N-1)E_{\vartheta_l}\right)\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\},
     \min\left\{1,\left(\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}\right)\frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_pa_bounds_0_extra_demand}
\end{align}
\normalsize
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%  p^{PA,NE}_{RES,1}
%  \in
%   \notag\\\Biggl[ max\left(0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{1}\beta)}-E_1-r(N-1)E_0\right]\frac{1}{(1-r)(N-1)E_1}\right),
%   \notag\\
%     min\left(1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{1}\beta)}-E_1\right]\frac{1}{(1-r)(N-1)E_1}\right)
%    \Biggr].
%    \label{eq:prop_alloc_eq_bounds_1_extra_demand}
%\end{align}
%\normalsize
This range is derived by equalizing the right-hand sides of Eqs. (\eqref{eq:prop_alloc_energy} and \eqref{eq:conditionEQ_extra_demand} for $\vartheta_i \in \Theta$ and obtaining \eqref{eq:probrelation1}. Then, we take extreme values ($0$ and $1$) of all other probabilities except the one of interest in order to compute its range of values. Specifically, to obtain the lower (upper) bound we assign unary (zero) probablities to all other consumer types except $\vartheta_i$.

%Note that the equilibrium probabilities $p^{PA,NE}_{RES,\vartheta_i},$  $\forall \vartheta_i \in \Theta$ should satisfy \eqref{eq:probrelation1}, except if this requires values .  %This might not be possible only due to the need of being  \eqref{eq:prop_alloc_pa_bounds_0_extra_demand}. 

Furthermore, at NE, the expected aggregated demand for RES can be expressed as
\footnotesize
\begin{align}
& D^{PA,NE}=\nonumber \\ & \min\Bigl\{D^{Total}, \max\Bigl\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}\right]\frac{N}{(N-1)},0\Bigr\}\Bigr\},
    \label{eq:demand1}
\end{align}
\normalsize
for any $\vartheta_i \in \Theta$. To obtain \eqref{eq:demand1}, we observe that, by using \eqref{eq:probrelation1}, $D^{PA,NE}=N\sum_{ {\vartheta_l}\in \Theta} r_{\vartheta_l} E_{\vartheta_l} p^{PA,NE}_{RES,\vartheta_l}=
\frac{N}{(N-1)}\Bigl( \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}\Bigr)$.

\begin{remark}In case that all consumers are risk-seeking (i.e., $\epsilon_{\vartheta_i}= 1, \forall i \in \mathcal{N}$), there exist equilibrium states only if  $E_{\vartheta_i}=E_{\vartheta_j}$, for every pair $\vartheta_i, \vartheta_j$ with $\vartheta_i, \vartheta_j \in \Theta$. On the contrary, if there exists risk-conservative consumers, there may exist equilibrium states when consumers competing for $RES$ have asymmetric energy profiles.
\end{remark}

\begin{remark} \label{rem:risk_degrees_relation}
Notice that from the condition of Eq. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}, the existence of NE is possible only if $\epsilon_0<\epsilon_1<\epsilon_2<..<\epsilon_{M-1}$. This is because for every pair of energy demand profiles with $E_{\vartheta_i}<E_{\vartheta_j}$, Eq. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} is possible to hold only if $\epsilon_{\vartheta_i}<\epsilon_{\vartheta_j}$. This means that consumers with lower energy demand levels should be less risk-averse than those with higher energy demand levels.
\end{remark}
\vspace{5pt}
 
\textbf{Sub-case $2(b)$:} 
\emph{The energy demand profiles satisfy $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$  for all $\vartheta_i \in \Theta$.}


In this case, it is dominant strategy for all consumers to defer from competing for $RES$ and engage their loads in the night-zone. As result, the competing probabilities that lead to equilibrium states are equal to $p^{PA,NE}_{RES,\vartheta_i}=0$ for all consumers' types $\vartheta_i\in \Theta$, and the expected aggregate demand for RES at NE is equal to $D^{PA,NE}=0$. Note that a consumer type $\vartheta_i\in \Theta$ will engage in the night-zone a load equal to $\epsilon_{\vartheta_i} E_{\vartheta_i}$, i.e., the risk-averse consumers will engage their maximum demands.

To prove this, we need to show that $\upsilon_{RES, \vartheta_i}(\mathbf{p})>\upsilon_{nonRES, \vartheta_i}(\mathbf{p})$, $\forall \mathbf{p}$ and $\forall i\in \mathcal{N}$. Assume that $\vartheta_i=0$ and that the allocated energy is $E'$. Then, in a large population regime we have $\upsilon_{RES, 0}(\mathbf{p})= E'  ~c_{RES}+(E_0-E')~ \gamma~  c_{RES}$ and 
$\upsilon_{nonRES, 0}(\mathbf{p})= \epsilon_0~ E_0~ \beta~ c_{RES}$. The inequality $\upsilon_{RES,0}(\mathbf{p})>\upsilon_{nonRES, 0}(\mathbf{p})$ is then equivalent to the inequality $E_0 >E' \frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$. The latter inequality is true by assumption, considering that $E'<\mathcal{ER}$. The same can be shown for every $\vartheta_i\in \Theta$.
\vspace{5pt}


\textbf{Sub-case $2(c)$:} %In this Sub-case Eq. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} is not true.
\emph{There exist two distinct subsets of consumers' types $\Sigma_1 , \Sigma_2 \subset \Theta$ s.t. $\{E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}, ~\forall \vartheta_i \in \Sigma_1\}$ and $\{E_{\vartheta_i} \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}, ~ \forall \vartheta_i \in \Sigma_2\}$.} %the resulting interaction of consumers can be approached as a dominance-solvable game. Namely, it is assumed that rationality (as conceptualized by performing the best-response action) among players is common knowledge, that is, each player knows that the rest of the players are rational, and each player knows that the rest of the players know that he knows that the rest of the players are rational, and so on ad infinitum. In particular, 

For the consumers' types in the set $\Sigma_1$, it is dominant strategy to defer from competing for $RES$ and to engage their loads in the night-zone. The explanation is the same with Sub-case $2(b)$, i.e., it is based on comparing the costs of each pure strategy. Similarly with Sub-case $2(b)$, the competing probabilities that lead to equilibrium states are equal to $p^{PA,NE}_{RES,\vartheta_i}=0$ for all consumers' types $\vartheta_i\in \Sigma_1$, and each consumer will engage in the night-zone a load equal to $\epsilon_{\vartheta_i} E_{\vartheta_i}$, i.e., the risk-averse consumers will engage their maximum demands.

For the consumers' types in the set $\Sigma_2$, the mixed strategy NE is determined under the condition of Eq. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} involving only those consumers' types in $\Sigma_2$. Remark \ref{rem:risk_degrees_relation} holds now for all consumers' types in $\Sigma_2$. Additionally, for all consumers' types $\vartheta_i\in \Sigma_2$, the competing probabilities $p^{PA,NE}_{RES,\vartheta_i} $ that lead to equilibrium states lie in the range:%the particular conditions on pricing and energy demand levels and provided by 
%
%
%if their energy demand $E_{\vartheta_j}$ equals the threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$, then the competing probability is 

\vspace{-5pt}
\footnotesize
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{\vartheta_j\in \Sigma_2 \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_j}\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}\right]\frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_pa_bounds_0_extra_demandnew}
\end{align}
\normalsize
This result is obtained similarly to Eq.  \eqref{eq:prop_alloc_pa_bounds_0_extra_demand} but considering only the consumers' types in the set $\Sigma_2$. For consumer types $\vartheta_i\in \Sigma_1$, $p^{PA,NE}_{RES,\vartheta_i}=0$.

As a result, the expected aggregate demand can be expressed as follows, for any $\vartheta_i \in \Sigma_2$:
\vspace{-5pt}
\footnotesize
\begin{align}
&D^{PA,NE}=\nonumber\\ & \min\Biggl \{N  \sum_{\vartheta_l \in \Sigma_2} r_{\vartheta_l }E_{\vartheta_l}, \max\Biggl\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}\right]\frac{N}{(N-1)},0\Biggr\}\Biggr\}.
    \label{eq:demand2}
\end{align}
\normalsize


%In the special case of two risk-seeking consumers, one in $\Sigma_1$ (with index $1$) and the other in $\Sigma_2$ (with index $0$), we obtain $p^{PA,NE}_{RES,0} =min\left\{1,max\left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\beta)}-E_0\right]\frac{1}{r_0(N-1)E_0}\right\}\right\}$. 

\begin{remark}
In the special case of two consumers, one in $\Sigma_1$ (with index $1$) and the other in $\Sigma_2$ (with index $0$), we obtain 
$p^{PA,NE}_{RES,0}  =min\left\{1,max\left\{0, \left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{0}\beta)}-E_{0}\right]\frac{1}{r_{0}(N-1)E_{0}}\right\}\right\}$.
\end{remark}

%Note that based on Eq. \eqref{eq:prop_alloc_eq_j_extra_demand1}, if $E_{\vartheta_j}$ is strictly lower than $thr_d=\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}rse^{PA}_{\vartheta_j}(.)$ then the dominant strategy is to compete for $RES$, else if $E_{\vartheta_j}> th_d$ the dominant strategy is to defer from competing for $RES$.

%Otherwise, if $E_{\vartheta_j}$ is lower than this threshold value, opting for competing is dominant strategy, leveraging the withdrawal of consumers of $\vartheta_i$ energy profile, and, finally, if $E_{\vartheta_j}$ exceeds this threshold value, they are motivated to avoid competition.

\subsubsection*{\textbf{Case $3$}}
\emph{The risk aversion degrees satisfy $\epsilon_{\vartheta_i} \geq \gamma/\beta$, $\forall i\in \mathcal{N}$.}

In this case, it is dominant strategy for all consumers to compete for $RES$. This can be shown by proving that $\upsilon_{RES, \vartheta_i}(\mathbf{p})<\upsilon_{nonRES, \vartheta_i}(\mathbf{p})$, $\forall \mathbf{p},~ \forall i\in \mathcal{N}$. Assume that $\vartheta_i=0$ and that the allocated energy is $E'$. Then, the inequality $\upsilon_{RES,0}(\mathbf{p})<\upsilon_{nonRES, 0}(\mathbf{p})$ is equivalent to the inequality $E_0 >E' \frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$. This is true by assumption, since $(\gamma-\epsilon_0\beta)\leq 0$ in this case. 

Therefore, the competing probabilities that lead to equilibrium states are equal to $p^{PA,NE}_{RES,\vartheta_i}=1$ for all consumers' types $\vartheta_i\in \Theta$, and the expected aggregate demand for RES at NE is equal to $D^{PA,NE}=D^{Total}$.

\subsubsection*{\textbf{Case $4$}} \emph{There exist two distinct subsets of consumers' types $\Sigma_1$, $\Sigma_2 \subset \Theta$ s.t. $\Bigl\{\epsilon_{\vartheta_i} \geq \gamma/\beta, ~ \forall \vartheta_i \in \Sigma_1\Bigr\}$, and $\Bigl\{\epsilon_{\vartheta_i} < \gamma/\beta,~\forall \vartheta_i \in \Sigma_2\Bigr\}$.} 

For the consumers' types in the set $\Sigma_1$, it is dominant strategy to compete for $RES$. Therefore, the competing probabilities that lead to equilibrium states are equal to $p^{PA,NE}_{RES,\vartheta_i}=1$ for all consumers' types $\vartheta_i\in \Sigma_1$. By analogy with Case $3$, this is shown by proving that $\upsilon_{RES, \vartheta_i}(\mathbf{p})<\upsilon_{nonRES, \vartheta_i}(\mathbf{p}),~\forall \mathbf{p}$, $\forall \vartheta_i \in \Sigma_1$.


For the consumers' types in the set $\Sigma_2$, the mixed strategy NE is determined under condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} involving only the those consumers' types in $\Sigma_2$. Remark \ref{rem:risk_degrees_relation} now holds for all consumers in $\Sigma_2$. Besides, for consumers' types $\vartheta_i \in \Sigma_2$, the competing probabilities $p^{PA,NE}_{RES,\vartheta_i}$ that lead to equilibrium states lie in the range:

\footnotesize
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{\vartheta_j\in \Theta \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_j}\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}- \right. \right. \nonumber \\ & \left. \left.
  \sum_{\vartheta_j\in \Sigma_1 \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_j}\right]\frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_pa_bounds_0_extra_demandnew4}
\end{align}
\normalsize
This range is obtained similarly to Eq. \eqref{eq:prop_alloc_pa_bounds_0_extra_demand} considering that the consumers in $\Sigma_1$ compete for $RES$. 

In addition, the expected aggregate demand for RES at NE can be expressed as
\footnotesize
\begin{align}
& D^{PA,NE}= N  \sum_{\vartheta_j \in \Sigma_1} r_{\vartheta_j }E_{\vartheta_j}+\min\Biggl\{N  \sum_{\vartheta_j \in \Sigma_2} r_{\vartheta_j }E_{\vartheta_j}, \max\Biggl\{  \Bigl[\mathcal{ER}\nonumber \\  & \cdot \frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i} -\sum_{\vartheta_j\in \Sigma_1 \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_j}\Bigr]\frac{N}{(N-1)},0\Biggr\}\Biggr\},
    \label{eq:demand3}
\end{align}
\normalsize
for any $\vartheta_i \in \Sigma_2$.

%\vspace{-5pt}
%\footnotesize
%\begin{align}
%&p^{PA,NE}_{RES,\vartheta_j}  =
%   \left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}-[r+(1-2r)\vartheta_i](N-1)E_{\vartheta_i}\right]\notag \\
%   & \times \frac{1}{[r+(1-2r)\vartheta_j](N-1)E_{\vartheta_j}}, \nonumber\\
%&    0\leq p^{PA,NE}_{RES,\vartheta_j} \leq 1.
% \label{eq:prop_alloc_eq_j_extra_demand2}
%\end{align}
%\normalsize
%%This result derives by equalizing the right-hand sides of Eqs. (\ref{eq:prop_alloc_energy}) and (\ref{eq:conditionEQ_extra_demand}) and after replacing $n_0 E_0 +n_1 E_1 $ with the equal quantity $p^{PA,NE}_{RES,\vartheta_j}[r+(1-2r)\vartheta_j](N-1)E_{\vartheta_j} +[r+(1-2r)\vartheta_i](N-1)E_{\vartheta_i}$ (since consumers with energy profile $E_{\vartheta_i}$ compete for $RES$). %As in Case $2$, based on Eq. \eqref{eq:prop_alloc_eq_j_extra_demand2}, if $E_{\vartheta_j}$ is strictly lower than $thr_d$ then the dominant strategy is to compete for $RES$, else if $E_{\vartheta_j}> th_d$ the dominant strategy is to defer from competing for $RES$.


%if $E_{\vartheta_j}$ equals threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$. Otherwise, under lower energy demand $E_{\vartheta_j}$, the dominant strategy amounts to competing and under higher energy demand, they resort to the safer option avoiding competition.

%The mixed strategy equilibrium probabilities for all cases are summarized in Table \ref{table_eq_comp_pro}.
%
%\footnotesize
%\begin{table*}[b]
%\def\arraystretch{1.5}
%\caption{Mixed Strategy Equilibrium Probabilities and Demand for RES, in uncoordinated energy source selection under risk-conservative consumers and proportional allocation of RES; $i,j \in \mathcal{N}$, $\vartheta_i\neq \vartheta_j$, $thr_a=\gamma/\beta$, $thr_b=\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_i\beta)}$, $thr_c=\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_j\beta)}$, $thr_d=\frac{thr_c}{(r+(1-2r)\vartheta_j)(N-1)+1}$, $thr_e= \frac{thr_c- (r+(1-2r)\vartheta_i)(N-1)E_i}{(r+(1-2r)\vartheta_j)(N-1)+1}$, $thr_f=thr_c- (r+(1-2r)\vartheta_i)(N-1)E_i$.}
%%
%\begin{center}
%\begin{tabular}{|c|c|c|c|c||c|c||c|}
%%
%\cline{1-8}
%$\epsilon_i$ & $\epsilon_j$ & $E_{\vartheta_i}$ & \multicolumn{2}{ c|| }{$E_{\vartheta_j}$} & $p^{PA,NE}_{RES,\vartheta_i}$ & $p^{PA,NE}_{RES,\vartheta_j}$ & $D^{PA,NE}$\\  
%\hline \hline 
%%
%$<thr_a$ & $<thr_a$ & $\leq thr_b$ & \multicolumn{2}{ c|| }{$\leq thr_c$} & Ref. (\ref{eq:prop_alloc_eq_bounds_0_extra_demand}) & Ref. (\ref{eq:prop_alloc_eq_bounds_1_extra_demand}) & $\frac{N}{(N-1)}  \left[ \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j} \right]$\\ \cline{1-8}
%%
%%$<thr_a$ & $<thr_a$ & $> thr_b$ & \multicolumn{2}{ c|| }{$> thr_c$} & 0 & 0 & 0\\ \cline{1-8}
%%
%\multicolumn{1}{|c|}{\multirow{3}{*}{$<thr_a$}} & \multicolumn{1}{c|}{\multirow{3}{*}{$<thr_a$}} & \multicolumn{1}{c|}{\multirow{3}{*}{$>thr_b$}} & \multicolumn{2}{ c|| }{\multirow{1}{*}{$\geq thr_d, \leq thr_c$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$0$}} & \multicolumn{1}{ c|| }{\multirow{1}{*}{Ref. (\ref{eq:prop_alloc_eq_j_extra_demand1})}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$\frac{N}{(N-1)}\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}\right]$}}   \\ \cline{4-8}
%%
%\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{2}{ c|| }{\multirow{1}{*}{$< thr_d$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$0$}} & \multicolumn{1}{ c|| }{\multirow{1}{*}{$1$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$[r+(1-2r)\vartheta_j]NE_{\vartheta_j}$}}\\ \cline{4-8}
%%
%\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &\multicolumn{2}{ c|| }{\multirow{1}{*}{$>thr_c$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$0$}} & \multicolumn{1}{ c|| }{\multirow{1}{*}{$0$}} &  \multicolumn{1}{ c| }{\multirow{1}{*}{$0$}} \\ \cline{1-8}
%%
%$\geq thr_a$ & $\geq thr_a$ & $>0$ & \multicolumn{2}{ c|| }{$>0$} & 1 & 1 & $N\left[[r+(1-2r)\vartheta_i]E_{\vartheta_i}+[r+(1-2r)\vartheta_j]E_{\vartheta_j}\right]$\\ \cline{1-8}
%%
%\multicolumn{1}{|c|}{\multirow{3}{*}{$\geq thr_a$}} & \multicolumn{1}{c|}{\multirow{3}{*}{$< thr_a$}} & \multicolumn{1}{c|}{\multirow{3}{*}{$>0$}} & \multicolumn{2}{ c|| }{\multirow{1}{*}{$\geq thr_e, \leq thr_f$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$1$}} & \multicolumn{1}{ c|| }{\multirow{1}{*}{Ref. (\ref{eq:prop_alloc_eq_j_extra_demand2})}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$  \frac{N}{(N-1)}\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}\right]$}}\\ \cline{4-8}
%%%
%\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{2}{ c|| }{\multirow{1}{*}{$<thr_e$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$1$}} & \multicolumn{1}{ c|| }{\multirow{1}{*}{$1$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$N\left[[r+(1-2r)\vartheta_i]E_{\vartheta_i}+[r+(1-2r)\vartheta_j]E_{\vartheta_j}\right]$}} \\ \cline{4-8}
%%%
%\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{2}{ c|| }{\multirow{1}{*}{$>thr_f$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$1$}} & \multicolumn{1}{ c|| }{\multirow{1}{*}{$0$}} & \multicolumn{1}{ c| }{\multirow{1}{*}{$[r+(1-2r)\vartheta_i]NE_{\vartheta_i}$}}\\ \cline{1-8}
%%%%
%\end{tabular}
%\end{center}
%\label{table_eq_comp_pro}
%\end{table*}
%\normalsize



% leverage the absence of competitors of $\vartheta_i$ energy profile and opt for the RES, if $\frac{(\gamma-1)}{(\gamma-\epsilon_j\beta)} \geq \frac{E_{\vartheta_j}}{rse^{PA}_{\vartheta_i}(\cdot)}$, and follow the rest of consumers in the safer option avoiding risking, otherwise.

%If $E_0 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$, it is dominant strategy for all consumers of low-to-moderate energy consumption profile to defer from competing for the renewable energy source, namely $c_{i}^{(\cdot)}(RES,p)>c_{i}^{(\cdot)}(nonRES,p)$, $\forall p$ and $\forall i\in \mathcal{N}: \vartheta_i=0$. Similarly, if $E_1 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$, it is dominant strategy for all consumers of high energy consumption profile to defer from competing for the renewable energy source, namely $c_{i}^{(\cdot)}(RES,p)>c_{i}^{(\cdot)}(nonRES,p)$, $\forall p$ and $\forall i\in \mathcal{N}: \vartheta_i=1$.

%\textbf{Demand:} relations and risk-aversion degree values examined above.

%under equilibrium strategy profiles shaped by the competing probabilities in intervals (\ref{eq:prop_alloc_eq_bounds_0_extra_demand}) and (\ref{eq:prop_alloc_eq_bounds_1_extra_demand}) becomes

%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
% \hspace{-10pt} D^{PA,NE}(p^{PA,NE}) \hspace{-5pt} &=&  \hspace{-5pt} N\left[ r  p^{PA,NE}_{RES,0} E_0+(1-r)  p^{PA,NE}_{RES,1} E_1\right] \nonumber \\
% \hspace{-5pt} &=& \hspace{-5pt} \frac{N}{(N-1)}  \left[ \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{0}\beta)}-E_0 \right]
%\label{eq:demand_pa_ne_extra_demand}
%\end{eqnarray}
%\normalsize


%In Section \ref{sec:coordinated}, we describe conditions on pricing and energy consumption profiles that cause inefficiencies.

%when the renewable energy demand does not match the supply, that is, $D^{PA,NE}(p^{PA,NE}) \neq \mathcal{ER}$.




Finally, in the special case of risk-seeking consumers, the social cost takes an interesting form because it becomes independent of the probability $p^{PA,NE}$. This is independent of the risk aversion degrees and energy demand levels, i.e., it holds for all the four cases above. Specifically,

\small
\begin{align}
&C^{PA,NE}= min(\mathcal{ER}, D^{PA,NE}) c_{RES} +  max(0,D^{PA,NE}-\mathcal{ER})\cdot  \nonumber \\ &c_{nonRES,D} 
+ \left[ D^{Total} -D^{PA,NE} \right] c_{nonRES,N},
 \label{eq:social_cost_pa_sc}
 \end{align}
\normalsize
where $D^{PA,NE} $ is given by Eq. \eqref{eq:demand1} or Eq. \eqref{eq:demand2} with $\epsilon_{\vartheta_i}=1$.





==> old/uncoordinated_ES.tex <==


\subsection{Equal Sharing}\label{sec:eq_sharing_eq_extra_demand}
The analysis of the mixed strategy equilibrium probabilities for the ES policy coincides with the one for the PA policy (Section \ref{sec:prop_alloc_eq_extra_demand}) for all cases, except for Cases $2$ and $4$. For the sake of concision, this analysis is detailed below only for those cases.

\subsubsection*{\textbf{Case $2$}} 
\hspace{10pt}
\vspace{5pt}

\textbf{Sub-case $2(a)$:} A mixed strategy equilibrium exists if and only if, for any consumers' types  $\vartheta_i \in \Theta$ and $ \vartheta_j \in \Theta \setminus \{\vartheta_i\}$, with energy profiles $E_{\vartheta_i} \neq E_{\vartheta_j}$, it holds that
\small
\begin{align}\label{eq:relation_E_0_E_1_es_ne_extra_demand}
(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i} =(\gamma-\epsilon_{\vartheta_j}\beta)E_{\vartheta_j}.
\end{align}
\normalsize
This condition is derived by equalizing the right-hand sides of Eqs. \eqref{eq:eq_sharing_energy} and \eqref{eq:conditionEQ_extra_demand}, for $\vartheta_i \in \Theta$ and $\vartheta_j \in \Theta \setminus \{\vartheta_i\}$ and obtaining:
\begin{small}
\begin{align}
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1= \sum_{ {\vartheta_\ell}\in \Theta} r_{\vartheta_\ell} (N-1) p^{ES,NE}_{RES,\vartheta_\ell},\label{eq:probrelationes1}\\
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)E_{\vartheta_j}}-1= \sum_{ {\vartheta_\ell}\in \Theta} r_{\vartheta_\ell} (N-1) p^{ES,NE}_{RES,\vartheta_\ell}.\label{eq:probrelationes2}
\end{align} 
\end{small}
As the right hand-sides of Eqs. \eqref{eq:probrelationes1}-\eqref{eq:probrelationes2} are equal, it derives that:
\begin{align}
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1= 
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)E_{\vartheta_j}}-1,
\end{align} 
which straightforwardly leads to Eq. \eqref{eq:relation_E_0_E_1_es_ne_extra_demand}. 

 %\emph{The energy demand profiles satisfy  $E_{\vartheta_i } \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i }\beta)}$,  for all $\vartheta_i \in \Theta$.} %or $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gam
As a result, the competing probabilities, $p^{ES,NE}_{RES,{\vartheta_i }}$, for all $ \vartheta_i \in \Theta$ that lead to equilibrium states lie in the following range,
\footnotesize
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1-
  \sum_{{\vartheta_j}\in \Theta \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1\right]\frac{1}{r_{\vartheta_i}(N-1)}\right\}
    \Biggr].
    \label{eq:prop_alloc_eq_bounds_0_extra_demand}
\end{align}
\normalsize
Similarly to the PA policy, this range is derived using Eq. \eqref{eq:probrelationes1}.

\begin{remark}
Note that, similarly to the PA policy, from the condition of Eq. \eqref{eq:relation_E_0_E_1_es_ne_extra_demand}, the existence of NE is possible if and only if $\epsilon_0<\epsilon_1<\epsilon_2<..<\epsilon_{M-1}$. 
\end{remark}
\vspace{5pt}

%Then, we take extreme values of the other probabilities as before. 
%Note that the probabilities $p^{PA,NE}_{RES,\vartheta_i}$ should be chosen in the range \eqref{eq:prop_alloc_eq_bounds_0_extra_demand}, but, also under the constraint of \eqref{eq:probrelationes1}.


\textbf{Sub-case $2(b)$:} In this case, the analysis is identical to the one for the PA policy, in Section \ref{sec:prop_alloc_eq_extra_demand}. 
\vspace{5pt}
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%  p^{PA,NE}_{RES,1}
%  \in
%   \notag\\\Biggl[ max\left(0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{1}\beta)}-E_1-r(N-1)E_0\right]\frac{1}{(1-r)(N-1)E_1}\right),
%   \notag\\
%     min\left(1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{1}\beta)}-E_1\right]\frac{1}{(1-r)(N-1)E_1}\right)
%    \Biggr].
%    \label{eq:prop_alloc_eq_bounds_1_extra_demand}
%\end{align}
%\normalsize


%The rest content of Sub-case (a) remains the same with Section \ref{sec:prop_alloc_eq_extra_demand}. 
%The expected aggregated demand for any $\vartheta_i \in \Theta$ is equal to,
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%& D^{PA,NE}=\nonumber \\ & \min\{N  \sum_{\vartheta_j \in \Theta} r_{\vartheta_j }E_{\vartheta_j}, \max\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1\right]\frac{N}{(N-1)},0\}\}.
%    \label{eq:demand1}
%\end{align}
%\normalsize
%If $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$  for all $\vartheta_i \in \Theta$, it is dominant strategy for all consumers to defer from competing for $RES$, namely, $\upsilon_{RES, \vartheta_i}(p)>\upsilon_{nonRES, \vartheta_i}(p)$, $\forall p$ and $\forall i\in \mathcal{N}$. To show this, assume that $\vartheta_i=0$ and the allocated energy is $E'$. Then, in a large population regime $\upsilon_{RES, 0}(p)= E'  c_{RES}+(E_0-E') \gamma  c_{RES}$ and 
%$\upsilon_{nonRES, 0}(p)= \epsilon_0 E_0 \beta c_{RES}$. The inequality $\upsilon_{RES,0}(p)>\upsilon_{nonRES, 0}(p)$ is then equivalent to the inequality $E_0 >E' \frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ which is true by assumption and by the fact that the allocated energy $E'$ will be less than the available energy $\mathcal{ER}$. The same can be shown for the other $\vartheta_i\in \Theta$. Obviously, in this case, $D^{PA,NE}=0$.

\textbf{Sub-case $2(c)$:} %In this Sub-case Eq. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} is not true.
For consumers' types in the set $\Sigma_1$, the analysis is identical to the one for the PA policy, in Section \ref{sec:prop_alloc_eq_extra_demand}.

For consumers' types in the set $\Sigma_2$, the mixed strategy NE is determined under the condition of Eq. \eqref{eq:relation_E_0_E_1_es_ne_extra_demand} involving only those consumers' types in $\Sigma_2$. 

Therefore, the competing probabilities $p^{ES,NE}_{RES,\vartheta_i}$ for all $\vartheta_i\in \Sigma_2$ that lead to equilibrium states lie in the range:%the particular conditions on pricing and energy demand levels and provided by 
%
%
%if their energy demand $E_{\vartheta_j}$ equals the threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$, then the competing probability is 
\footnotesize
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{\vartheta_j\in \Sigma_2 \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_i}\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}\right]\frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_es_bounds_0_extra_demandnew}
\end{align}
\normalsize
By analogy with the analysis for the PA policy, this range is derived by writing Eq. \eqref{eq:probrelationes1} for consumers in $\Sigma_2$, which gives:
 $$\sum_{\vartheta_l\in \Sigma_2} p^{ES,NE}_{RES,\vartheta_l} r_{\vartheta_l }(N-1)=\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1$$.
 Then, \eqref{eq:prop_alloc_es_bounds_0_extra_demandnew} is derived by multiplying both sides of this equation with $E_{\vartheta_i}$ and taking the upper and lower bounds of the probabilities for all other consumers except $\theta_i \in \Sigma_2$.

\subsubsection*{\textbf{Case $4$}} 
For the consumers' types in the set $\Sigma_1$, the analysis is identical to the one for the PA policy, in Section \ref{sec:prop_alloc_eq_extra_demand}.

For the consumers' types in the set $\Sigma_2$, the mixed strategy NE is determined under condition \eqref{eq:relation_E_0_E_1_es_ne_extra_demand} involving only the those consumers' types in $\Sigma_2$. Besides, for consumers' types $\vartheta_i \in \Sigma_2$, the competing probabilities $p^{ES,NE}_{RES,\vartheta_i}$ that lead to equilibrium states lie in the range:
\small
\begin{align}
&  \Biggl[ \max \left\{0,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{\vartheta_j\in \Theta \setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_i}\right]\cdot  \right. \nonumber \\&  \left. \frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\},
     \min\left\{1,\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}- \right. \right. \nonumber \\ & \left. \left.
  \sum_{\vartheta_j\in \Sigma_1\setminus \{\vartheta_i\}} r_{\vartheta_j} (N-1)E_{\vartheta_i}\right]\frac{1}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_eq_bounds_0_extra_demandnew55}
\end{align}
\normalsize
This result is derived similarly to Eq. \eqref{eq:prop_alloc_es_bounds_0_extra_demandnew}, but considering that all consumers' types $\vartheta_i \in \Sigma_1$ compete for $RES$, i.e., that their competing probabilities that lead to equilibrium states are equal to $p^{ES,NE}_{RES,\vartheta_i}=1$.%, i.e., by equalizing the right-hand sides of Eqs. (\ref{eq:eq_sharing_energy}) and (\ref{eq:conditionEQ_extra_demand}) and considering that consumers with energy profile in $\Sigma_1$ compete for $RES$, i.e., $p^{ES,NE}_{RES,\vartheta_i}=1,~ \forall \vartheta_i \in \Sigma_1 $.% Then, we obtain the equality $\sum_{\vartheta_j\in \Sigma_2} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }(N-1)+\sum_{\vartheta_j\in \Sigma_1} r_{\vartheta_j }(N-1)=\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)E_{\vartheta_i}}-1$, and  Eq. \eqref{eq:prop_alloc_eq_bounds_0_extra_demandnew55} derives if multiplying both sides with $E_{\vartheta_i}$ and taking extreme values of the probabilities. %Note that based on Eq. \eqref{eq:equal_sharing_eq_j_extra_demand2}, if $E_{\vartheta_j}$ is strictly lower than $thr_d=\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}rse^{PA}_{\vartheta_j}(.)$ then the dominant strategy is to compete for $RES$, else if $E_{\vartheta_j}> th_d$ the dominant strategy is to defer from competing for $RES$.




%with $E_0 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$. Otherwise, if $E_0 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$, it is dominant strategy for all consumers to defer from competing for $RES$, namely $c_{i}^{(\cdot)}(RES,p)>c_{i}^{(\cdot)}(nonRES,p)$, $\forall p$ and $\forall i\in \mathcal{N}$. Similarly, if $E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$ and $E_{\vartheta_j} \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}$, with $\vartheta_i\neq \vartheta_j$ and $i,j \in \mathcal{N}$, it is dominant strategy for all consumers of $\vartheta_i$ energy profile not to compete for $RES$. Regarding consumers of $\vartheta_j$ energy profile, they end up competing with probability $p^{ES,NE}_{RES,\vartheta_j}$ that follows (\ref{eq:prop_alloc_eq_j_extra_demand1}). %, if their energy demand $E_{\vartheta_j}$ equals the threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$; otherwise, competing for $RES$ dominates reneging from RES, if $E_{\vartheta_j}$ is lower than this threshold value, and it is dominated by reneging from RES, if $E_{\vartheta_j}$ exceeds this threshold value.
%Furthermore, if $\epsilon_{\vartheta_i} \geq \gamma/\beta$, $\forall i\in \mathcal{N}$, it is dominant strategy for all consumer to compete for $RES$, since it holds that $c_{i}^{(\cdot)}(RES,p) < c_{i}^{(\cdot)}(nonRES,p)$, $\forall p$ and $\forall i\in \mathcal{N}$. Finally, if $\epsilon_{\vartheta_i} \geq \gamma/\beta$ and $\epsilon_{\vartheta_j} < \gamma/\beta$, with $\vartheta_i\neq \vartheta_j$ and $i,j \in \mathcal{N}$, then it is dominant strategy for all consumers of $\vartheta_i$ energy profile to compete, while all consumers of $\vartheta_j$ end up competing with $p^{PA,NE}_{RES,\vartheta_j}, ~0\leq p^{PA,NE}_{RES,\vartheta_j} \leq 1$,
%
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%p^{PA,NE}_{RES,\vartheta_j}  = 
%   \left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}-[r+(1-2r)\vartheta_i](N-1)E_{\vartheta_j}\right] \notag \\
%    \times  \frac{1}{[r+(1-2r)\vartheta_j](N-1)E_{\vartheta_j}} 
% \label{eq:es_eq_j_extra_demand2}
%\end{align}
%\normalsize


%if $E_{\vartheta_j}$ equals threshold $\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$. Otherwise, under lower energy demand $E_{\vartheta_j}$, the dominant strategy amounts to competing and under higher energy demand, they are motivated to resort to the safer option avoiding competition.

%It can be easily observed that the equal sharing and the proportional allocation policies may only cause different equilibrium states under the game variant where consumers risk only part of their maximum possible demand,i.e., with risk-conservative consumers. For instance the conditions of Eqs. \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}, \eqref{eq:relation_E_0_E_1_es_ne_extra_demand} coincide for risk-seeking consumers. %In particular, the equal sharing differentiates from proportional allocation under two cases: (a) if $\epsilon_{\vartheta_i}<\gamma/\beta$, $\forall i\in \mathcal{N}$, $E_0 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 \leq  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$; (b) if $\epsilon_{\vartheta_i} \geq \gamma/\beta$, $\epsilon_{\vartheta_j} < \gamma/\beta$ and $E_{\vartheta_j}=\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)} rse^{PA}_{\vartheta_j}(\cdot)$ with $\vartheta_i\neq \vartheta_j$ and $i,j \in \mathcal{N}$. Thus, 
%The set of mixed strategy equilibrium probabilities under equal sharing is also presented in Table \ref{table_eq_comp_pro}, by (i) replacing the probabilities in the second line, fifth and sixth columns, with the expressions in (\ref{eq:equal_sharing_eq_bounds_0_extra_demand}), (\ref{eq:equal_sharing_eq_bounds_1_extra_demand}), replacing the probability in the seventh line, sixth column with Eq. (\ref{eq:equal_sharing_eq_j_extra_demand2}), and (iii) replacing the thresholds $thr_e$, $thr_f$ with $\frac{thr_c}{( r+(1-2r)\vartheta_i)(N-1)+(r+(1-2r)\vartheta_j)(N-1)+1}$ and $thr_d$, correspondingly.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



In all cases where the PA and ES policies result in the same mixed strategy equilibrium probabilities, the corresponding expected aggregate demand for RES is the same under the two policies. 
Otherwise (i.e., for cases 2 and 4 described above), we can write the expected aggregate demand under the ES policy as follows:

\footnotesize
\begin{align}
& \hspace{-10pt}  D^{ES,NE}(\mathbf{p^{ES,NE}}) =N p^{ES,NE}_{RES,0} r_{0}E_{0}+N \sum_{\vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }E_{\vartheta_j} \nonumber \\
&=\Bigl (\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{0}\beta)E_{0}}-1- \sum_{\vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j } (N-1) \Bigr) \frac{N~E_0}{N-1} \nonumber \\ &+N \sum_{\vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }E_{\vartheta_j} \nonumber \\ &=D^{PA,NE}+N \sum_{ \vartheta_j \in \Theta \setminus \{0\}} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }(E_{\vartheta_j} -E_0).
\label{eq:demand_es_ne_extra_demand}
\end{align}
\normalsize

%given in Table \ref{table_eq_comp_pro}. 
%Otherwise, %under the conditions of the second and seventh line of Table \ref{table_eq_comp_pro}, 
%the expected aggregate demand for renewable energy $D^{ES,NE}(p^{ES,NE})$ is an non-decreasing function of $p^{ES,NE}_{RES,1}$, that is,
%
%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%\hspace{-10pt}  && \hspace{-10pt}  D^{ES,NE}(p^{ES,NE}) =N \sum_{\vartheta_j\in \Theta} p^{ES,NE}_{RES,\vartheta_j} r_{\vartheta_j }E_{\vartheta_j}.
%\label{eq:demand_es_ne_extra_demand}
%\end{eqnarray}
%\normalsize
% \hspace{-10pt} &=& \hspace{-10pt}  \frac{N}{(N-1)} \left[ \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{0}\beta)} -E_0\right] + (1-r)(E_1-E_0)N p^{ES,NE}_{RES,1}\nonumber\\
% \hspace{-10pt} &=& \hspace{-10pt} D^{PA,NE}(p^{PA,NE})+ (1-r)(E_1-E_0)N p^{ES,NE}_{RES,1}.



%The second line in Eq. \eqref{eq:demand_es_ne_extra_demand} derives by replacing in the first line that  $ p^{ES,NE}_{RES,0} =\frac{1}{r(N-1) } \Big[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)E_0}-1- (1-r) (N-1) p^{ES,NE}_{RES,1} \Big]$.
%Likewise, under the conditions of the sixth line of Table \ref{table_eq_comp_pro}, the expected total number of consumers that compete for $RES$ in equilibrium, equals $\frac{N}{(N-1)}  \left[ \frac{\mathcal{ER}}{E_{\vartheta_j}}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-1 \right]$ and the expected aggregate demand for renewable energy $D^{ES,NE}(p^{ES,NE})$ is given by (\ref{eq:demand_es_ne_extra_demand}).

%Conditions under which equilibrium competing probabilities generate inefficiencies, that is, a number of consumers incur the price of the lack of coordination are described in Section \ref{sec:coordinated}.


%\textbf{Social Cost:}  The expected aggregate cost incurred by the entire population is a function of $p^{ES,NE}$ (contrary to the Eq. \eqref{eq:social_cost_pa}) and is given by,
%\vspace{-5pt}
%\footnotesize
%\begin{align}
%& C^{ES,NE}(p^{ES,NE})  \nonumber \\ &=  d(p^{ES,NE}) c_{RES} +(D^{ES,NE}-d(p^{ES,NE}))c_{nonRES,D} \nonumber \\
%&   + N\left[\sum_{\vartheta_j \in \Theta} r_{\vartheta_j }p^{ES,NE}_{nonRES,\vartheta_j}\epsilon_{\vartheta_j }E_{\vartheta_j}\right] c_{nonRES,N},
% \label{eq:social_cost_es_extra_demand}
% \end{align}
%\normalsize 


Finally, similarly to the proportionally-fair allocation, the expected aggregate social cost at NE takes an interesting form in the special case of risk-seeking consumers. Specifically, 
\footnotesize
\begin{align}
&C^{ES,NE}(\mathbf{p^{ES,NE}}) \nonumber\\ &=  d(\mathbf{p^{ES,NE}}) c_{RES} +(D^{ES,NE}(\mathbf{p^{ES,NE}}) -d(\mathbf{p^{ES,NE}}))c_{nonRES,D}\nonumber \\
&+ \hspace{-5pt} \left[ \left[  \sum_{ \vartheta_j=0}^{M-1} r_{\vartheta_j} N E_{\vartheta_j}\right]-D^{ES,NE}(\mathbf{p^{ES,NE}}) \right] c_{nonRES,N}.
 \label{eq:social_cost_es_sc}
 \end{align}
\normalsize
%with \footnotesize$d(p^{ES,NE})=min(sh(p^{ES,NE}), E_0)rNp_{RES,0}^{ES,NE}+min(sh(p^{ES,NE}), E_1)(1-r)Np_{RES,1}^{ES,NE}$ \normalsize the actual aggregate amount of RES  allocated to the consumers and \footnotesize$sh(p^{ES,NE}) =\frac{\mathcal{ER}}{rNp_{RES,0}^{ES,NE}+(1-r)Np_{RES,1}^{ES,NE}}$ \normalsize the fair share of RES disseminated to the consumers. 


%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%sh(p) \hspace{-5pt} &=& \hspace{-5pt} \frac{\mathcal{ER}}{rNp_{RES,0}+(1-r)Np_{RES,1}}
% \label{eq:sharing_es}
% \end{eqnarray}
%\normalsize





%\subsection{Social Cost}\label{sec:social_cost_extra_demand}
%
%In the game variant with risk-conservative consumers, the social cost becomes
%
%
%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%C(p) \hspace{-5pt} &=& \hspace{-5pt} min(\mathcal{ER}, D^{(\cdot)}(p)) c_{RES} +  max(0,D^{(\cdot)}(p)-\mathcal{ER})c_{nonRES,D} \nonumber \\
% \hspace{-42pt}  &&  \hspace{-42pt} + \left[ rNp_{nonRES,0}(\epsilon_{0}E_0) \hspace{-2pt} + \hspace{-2pt} (1-r)Np_{nonRES,1}(\epsilon_{1}E_1)\right] c_{nonRES,N}
% \label{eq:social_cost_pa_es_extra_demand}
% \end{eqnarray}
%\normalsize


%\vspace{-5pt}
%\footnotesize
%\begin{eqnarray}
%C(p) \hspace{-5pt} &=& \hspace{-5pt} min(\mathcal{ER}, D^{(\cdot)}(p)) c_{RES} +  max(0,D^{(\cdot)}(p)-\mathcal{ER})c_{nonRES,D} \nonumber \\
% \hspace{-5pt}   &+& \hspace{-5pt} \left[ rN\epsilon_{0}E_0 + (1-r)N\epsilon_{1}E_1-D^{(\cdot)}(p)\right] c_{nonRES,N}
% \label{eq:social_cost_pa_es_extra_demand}
% \end{eqnarray}
%\normalsize




==> old/uncoordinated_lesia.tex <==
\section{Theoretical Game Analysis} \label{sec:uncoordinated_extra_demand}

Here, we study the conditions on the parameter values for the existence of dominant strategies and mixed-strategy NE under PA, and provide close form formulations of these states, i.e. ranges on the values of the vector of mixed strategies at NE $\mathbf{p^{NE}}$. The proofs of the theoretical results presented below are available in the online appendix \cite{}.

First, we recall that, for a mixed-strategy NE to exist, the expected costs of each consumer for all pure strategies in the support of the mixed-strategy NE must be equal. Using the expressions of the costs in \eqref{eq:RES_cost} and \eqref{eq:nonRES_cost2}, we obtain that the amount of RESs allocated to the type $\ell \in \Theta$ at a NE should satisfy:

%First, we recall that any mixed strategy NE $\mathbf{p^{NE}}$ must fulfill

%\small
%\begin{equation}\label{eq:cost_equality_mixed}
%\upsilon_{RES, \ell}(\mathbf{p^{NE}})= \upsilon_{nonRES, \ell}(\mathbf{p^{NE}}), ~\forall \ell \in \Theta.
%\end{equation}
%\normalsize

%\noindent Namely, the expected costs of each pure strategy in the support of the mixed-strategy equilibrium are equal. By substituting the expressions of \eqref{eq:RES_cost} and \eqref{eq:nonRES_cost2} in \eqref{eq:cost_equality_mixed}, we obtain that the amount of RESs allocated to $\ell \in \Theta$ at a NE should satisfy:

 \vspace{-0.1in} 
\small
\begin{equation}\label{eq:conditionEQ_extra_demand}
rse^{PA, NE}_{\ell}(\mathbf{p^{NE}}) = \frac{\gamma-\epsilon_{\ell}\beta}{\gamma-1}E_{\ell},~ \forall \ell \in \Theta.
\end{equation}
\normalsize 
\vspace{-0.1in}  

\noindent Thus, in the ESSG with the PA policy, a mixed-strategy NE exists under the condition:


 \vspace{-0.1in} 
 \small
\begin{equation}\label{eq:condition_PA_NE}
rse_{\ell}^{PA}(\mathbf{p}^{NE}) =rse_{\ell}^{PA,NE}(\mathbf{p}^{NE}), \forall \ell \in \Theta. \end{equation}
\normalsize 
\vspace{-0.1in}  

\noindent 
Therefore, for all cases, any existing mixed-strategy NE competing probabilities, $\mathbf{p}^{NE}$, are obtained so as to satisfy the condition \eqref{eq:condition_PA_NE}. In the following, we distinguish cases with respect to the RES capacity, as well as the preferences, i.e. the risk aversion degree values and the day-time energy demand, of all consumers. 

\subsection{\textbf{Case $1$: The RES capacity, $\mathcal{ER}$, exceeds the maximum total demand for RES $D^{Total}$ ($\mathcal{ER} \geq D^{Total}$).}}

As the consumers have knowledge of $\mathcal{ER}$ and $D^{Total}$, it is straightforward to show that the dominant-strategy for all consumers is to select the strategy $RES$. As a result, the competing probabilities that lead to equilibrium states are equal to $1$ for all consumer types, and the expected aggregate demand for RES at NE is equal to $D^{Total}$.

In all the remaining cases, we assume that $\mathcal{ER}< D^{Total}$. Three distinct cases are defined with respect to the risk aversion degrees of the consumers and energy prices.

\subsection{\textbf{Case $2$: The risk aversion degrees for all consumer types satisfy $1\leq \epsilon_{\ell}<\gamma/\beta$, $\forall \ell \in \Theta$.}}

We distinguish the following sub-cases with respect to the day-time energy demand levels. 

\subsubsection{\textbf{Sub-case $2(a)$: The day-time energy demand levels satisfy  $E_{\ell } \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell }\beta)}$,  for all $\ell \in \Theta$}}

In this case, a mixed-strategy NE with the PA policy exists if and only if for every pair of consumers, $i,j$ with day-time energy demand levels $E_{\vartheta_i}$, $E_{\vartheta_j}$, respectively, it holds that

 \vspace{-0.1in} 
 \small
\begin{eqnarray}\label{eq:relation_E_0_E_1_pa_ne_extra_demand}
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i }\beta)}-E_{\vartheta_i} &=& \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j }\beta)}-E_{\vartheta_j}.
 \end{eqnarray}
\normalsize 
\vspace{-0.1in}  


\begin{proof}
To derive the condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} we first consider a consumer $i$ with type $\vartheta_i \in \Theta$ that plays $RES$. Then, we can substitute the left-hand side of \eqref{eq:condition_PA_NE} with \eqref{eq:prop_alloc_energy} where the demand for RESs is expressed as $D(\mathbf{p^{NE}}) = E_{\vartheta_i}+ \sum_{ {\ell}\in \Theta} r_{\ell}~ (N-1)~E_{\ell}~p^{NE}_{RES,\ell}$. And, by also substituting the right-hand side of \eqref{eq:condition_PA_NE} with \eqref{eq:conditionEQ_extra_demand} for consumer $i$, we obtain:

\begin{small}
\begin{align}
&  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}= \sum_{ {\ell}\in \Theta} r_{\ell}~ (N-1)~E_{\ell}~p^{NE}_{RES,\ell},
    \label{eq:probrelation1}
\end{align}
\end{small}

\noindent By analogy, we can re-write \eqref{eq:probrelation1} for a consumer $j$ with type $\vartheta_j \in \Theta \setminus \{\vartheta_i\}$ that plays $RES$ as:

\begin{small}
\begin{align}
  &  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}=  \sum_{ {\ell}\in \Theta} r_{\ell} ~(N-1)~E_{\ell}~ p^{NE}_{RES,\ell}.
    \label{eq:probrelation2}  
\end{align}
\end{small}

\noindent Since the right-hand sides of \eqref{eq:probrelation1}-\eqref{eq:probrelation2} are equal, the left-hand sides will be also equal and \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} derives.
\end{proof}


Under condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}, the competing probabilities $p^{NE}_{RES,{\vartheta_i}}$ for each consumer $i$ of type $\vartheta_i \in \Theta$ that lead to equilibrium states lie in the range:


 \vspace{-0.1in} 
 \footnotesize
\begin{align}
&  \Biggl[ \max \Biggl\{0,\frac{\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{ {\ell}\in \Theta \setminus \{{\vartheta_i}\}} r_{\ell} (N-1)E_{\ell}}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\Biggl\}, \nonumber \\
 &      \min\Biggl\{1,\frac{\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\Biggl\}
    \Biggr].
    \label{eq:prop_alloc_pa_bounds_0_extra_demand}
\end{align}
\normalsize 
\vspace{-0.1in}  

Furthermore, at NE, the expected aggregate demand for RES for any consumer type $\ell \in \Theta$ can be expressed as:

 \vspace{-0.1in} 
 \footnotesize
\begin{align}
& D(\mathbf{p}^{NE})= \min\Bigl\{D^{Total}, \max\Bigl\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}-E_{\ell}\right]\frac{N}{(N-1)},0\Bigr\}\Bigr\}.
    \label{eq:demand1}
\end{align}
\normalsize 
\vspace{-0.1in}  

\begin{remark}\label{rem:risk_seeking}If all consumers are risk-seeking (i.e., $\epsilon_{\vartheta_i}= 1, \forall i \in \mathcal{N}$), a NE can exist only if  $E_{0}=E_{1}=...=E_{M-1}$.%for every pair of $\vartheta_i, \vartheta_j \in \Theta$. %On the contrary, if there are risk-conservative consumers, they may need to have asymmetric energy profiles for a NE to exist.
\end{remark}

\begin{remark} \label{rem:risk_degrees_relation}
Note that condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} can hold, and therefore a NE can exist, only if $\epsilon_0\leq \epsilon_1 \leq..\leq \epsilon_{M-1}$. Since by assumption, $E_0\leq E_1 \leq ...\leq E_{M-1}$, this means that consumers with lower day-time energy demand levels should be less risk-averse than those with higher ones.
\end{remark}

 
\subsubsection{\textbf{Sub-case $2(b)$: The day-time energy demand levels satisfy $E_{\ell} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}$  for all $\ell \in \Theta$}} 
In this case, the dominant strategy for all consumers is to play $nonRES$.

As result, the competing probabilities that lead to equilibrium states are equal to $0$ for all consumer types $\vartheta_i\in \Theta$, and the expected aggregate demand for RES at NE is equal to $0$.

\subsubsection{\textbf{Sub-case $2(c)$: There exist two distinct subsets of consumer types, $\Sigma_1 , \Sigma_2 \subset \Theta$, such that $\{E_{\ell} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}, ~\forall \ell \in \Sigma_1\}$ and $\{E_{\ell} \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}, ~ \forall \ell \in \Sigma_2\}$}}

For consumers whose types are in the set $\Sigma_1$, the dominant strategy is to play $nonRES$. 
For consumers whose types are in the set $\Sigma_2$, the mixed strategy NE is determined under the condition of \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}.

Additionally, for consumers whose types are in $\Sigma_1$, the competing probabilities at NE are equal to $0$, whereas, for consumers $i$ of type $\vartheta_i \in \Sigma_2$, the competing probabilities that lead to a NE states lie in the range:

 \vspace{-0.1in} 
 \footnotesize
\begin{align}
&  \Biggl[ \max \biggl\{0,\frac{\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}-
  \sum_{\ell \in \Sigma_2 \setminus \{\vartheta_i\}} r_{\ell} (N-1)E_{\ell}}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\Biggr\}, \nonumber \\
    & \min \Biggl\{1,\frac{\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}}{r_{\vartheta_i}(N-1)E_{\vartheta_i}}\Biggr\}
    \Biggr].
    \label{eq:prop_alloc_pa_bounds_0_extra_demandnew}
\end{align}
\normalsize  
\vspace{-0.1in}  

Finally, the aggregate demand for RESs in $\Sigma_1$ is equal to $0$, and the total aggregate demand for RESs can be expressed as

 \vspace{-0.1in} 
 \footnotesize
\begin{align}
& D(\mathbf{p}^{NE})= \min\Bigl\{ D^{Total}_{\Sigma_2} , \max\Bigl\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}-E_{\ell}\right]\frac{N}{(N-1)},0\Bigr\}\Bigr\},
    \label{eq:demand1_2c}
\end{align}
\normalsize 
\vspace{-0.1in}  

\noindent where $D^{Total}_{\Sigma_2} = N  \sum_{\tilde{\ell } \in \Sigma_2} r_{\tilde{\ell }  }E_{\tilde{\ell } }$ is the maximum demand for RESs of the consumers whose types are in $\Sigma_2$.

\begin{remark}
We note that Remark \ref{rem:risk_degrees_relation} now holds for all consumer types in $\Sigma_2$.
\end{remark}

\subsection{\textbf{Case $3$: The risk aversion degrees satisfy $\epsilon_{\ell} \geq \gamma/\beta$, $\forall \ell \in \Theta$.}}

In this case, the dominant strategy for all consumers is to play $RES$.

Therefore, the competing probabilities that lead to equilibrium states are equal to $1$ for all consumer types, and the aggregate demand for RESs at NE is equal to $D^{Total}$.

\subsection{\textbf{Case $4$: There exist two distinct subsets of consumer types, $\Sigma_1 , \Sigma_2 \subset \Theta$, such that $\Bigl\{\epsilon_{\ell} \geq \gamma/\beta, ~ \forall \ell \in \Sigma_1 \Bigr\}$, and $\Bigl\{\epsilon_{\ell} < \gamma/\beta,~\forall \ell \in \Sigma_2 \Bigr\}$.}} 


By analogy with Case $3$, for the consumers whose type is in the set $\Sigma_1$, the dominant strategy is to compete for RESs.
By analogy with Case $2$, for the consumers whose type is in the set $\Sigma_2$, three sub-cases $4(a)-(c)$ are defined with respect to their day-time energy demand levels. All the conditions derived in Case $2$ can straightforwardly be extended to the consumer types in $\Sigma_2$, considering that all consumers in $\Sigma_1$ play $RES$. To do so, we consider that the available RES capacity for consumers in $\Sigma_2$ is equal to $\mathcal{ER}$ minus the aggregate demand for RESs of consumer types in $\Sigma_1$. For the sake of concision we do not detail these conditions.

